Fast and Useful: Adapting Distilled Generators for Visual Learning

Distilled text-to-image models generate images quickly, but classifiers trained on those images can perform substantially worse than classifiers trained on images from their slower base models. We adapt released distilled generators to produce better training data while retaining fast generation. We fit a low-rank update to the student's first prediction so that it reaches an intermediate state produced by its unguided base, then disable the update and let the unchanged student finish generation. The base supplies training targets and is absent at inference. Guided targets and shorter jumps give classifiers lower accuracy in our ablations, showing why the state used for supervision matters. Across three generator families, the adapted images train better classifiers than images from the released students. With class-name templates at full ImageNet-1k scale, ResNet-50 top-1 rises from 8.4% to 34.2% for FLUX.2-klein and from 12.7% to 32.1% for SD-Turbo, using two and three denoiser evaluations per image, respectively. Fixed adapters also improve results on additional classes, fine-grained datasets, and other learner architectures and training recipes. Template-based adaptation remains useful against richer-prompt alternatives, while the benefit of combining adaptation with LLM generation prompts depends on the generator. Adapting a single generation step makes fast generators substantially more useful for training visual models.

==> numbers-review.tex <==
% Generated by code/scripts/paper_review_details.py; do not edit by hand.
\makeatletter
\expandafter\def\csname nm@in900GainKlein\endcsname{+26.0}
\expandafter\def\csname nm@in900GainKleinCI\endcsname{[+24.8, +27.3]}
\expandafter\def\csname nm@in900GainSD\endcsname{+19.3}
\expandafter\def\csname nm@in900GainSDCI\endcsname{[+18.3, +20.3]}
\expandafter\def\csname nm@equalFamilyDino\endcsname{+0.76}
\expandafter\def\csname nm@equalFamilyDinoCI\endcsname{[+0.55, +0.90]}
\expandafter\def\csname nm@equalFamilyClip\endcsname{+0.75}
\expandafter\def\csname nm@equalFamilyClipCI\endcsname{[+0.54, +0.89]}
\expandafter\def\csname nm@equalFamilyClipFd\endcsname{+0.80}
\expandafter\def\csname nm@equalFamilyClipFdCI\endcsname{[+0.61, +0.91]}
\expandafter\def\csname nm@equalFamilyFid\endcsname{+0.67}
\expandafter\def\csname nm@equalFamilyFidCI\endcsname{[+0.46, +0.80]}
\expandafter\def\csname nm@equalFamilyFdMinusRecall\endcsname{+0.04}
\expandafter\def\csname nm@equalFamilyFdMinusRecallCI\endcsname{[$-$0.10, +0.21]}
\expandafter\def\csname nm@promptTemplateKlein\endcsname{+26.9}
\expandafter\def\csname nm@promptTemplateKleinCI\endcsname{[+23.5, +30.4]}
\expandafter\def\csname nm@promptTemplateSD\endcsname{+25.0}
\expandafter\def\csname nm@promptTemplateSDCI\endcsname{[+21.9, +28.1]}
\expandafter\def\csname nm@promptCaptionKlein\endcsname{+6.4}
\expandafter\def\csname nm@promptCaptionKleinCI\endcsname{[+4.3, +8.6]}
\expandafter\def\csname nm@promptCaptionSD\endcsname{+20.7}
\expandafter\def\csname nm@promptCaptionSDCI\endcsname{[+17.7, +23.8]}
\expandafter\def\csname nm@promptLlmKlein\endcsname{+1.7}
\expandafter\def\csname nm@promptLlmKleinCI\endcsname{[$-$0.4, +4.0]}
\expandafter\def\csname nm@promptLlmSD\endcsname{+16.2}
\expandafter\def\csname nm@promptLlmSDCI\endcsname{[+13.6, +18.9]}
\expandafter\def\csname nm@rhoRecallLofoCI\endcsname{[+0.79, +0.88]}
\expandafter\def\csname nm@prepHoursKlein\endcsname{5.7}
\expandafter\def\csname nm@breakEvenKlein\endcsname{44,000}
\expandafter\def\csname nm@timingBatchKlein\endcsname{8}
\expandafter\def\csname nm@prepHoursSD\endcsname{0.9}
\expandafter\def\csname nm@breakEvenSD\endcsname{38,000}
\expandafter\def\csname nm@timingBatchSD\endcsname{32}
\makeatother


==> numbers.tex <==
% numbers.tex - written by code/scripts/paper_tables.py from results/; do not edit by hand
\makeatletter
\newcommand{\tp}[1]{\@ifundefined{tp@#1}{\textbf{??#1}}{\csname tp@#1\endcsname}}
\newcommand{\tpsd}[1]{\@ifundefined{tpsd@#1}{\textbf{??#1}}{\csname tpsd@#1\endcsname}}
\newcommand{\tpn}[1]{\@ifundefined{tpn@#1}{\textbf{??#1}}{\csname tpn@#1\endcsname}}
\newcommand{\tpsec}[1]{\@ifundefined{tpsec@#1}{\textbf{??#1}}{\csname tpsec@#1\endcsname}}
\newcommand{\tpnfe}[1]{\@ifundefined{tpnfe@#1}{\textbf{??#1}}{\csname tpnfe@#1\endcsname}}
\newcommand{\tpfid}[1]{\@ifundefined{tpfid@#1}{\textbf{??#1}}{\csname tpfid@#1\endcsname}}
\newcommand{\tprec}[1]{\@ifundefined{tprec@#1}{\textbf{??#1}}{\csname tprec@#1\endcsname}}
\newcommand{\gp}[1]{\@ifundefined{gp@#1}{\textbf{??#1}}{\csname gp@#1\endcsname}}
\newcommand{\gpci}[1]{\@ifundefined{gpci@#1}{\textbf{??#1}}{\csname gpci@#1\endcsname}}
\newcommand{\gpa}[1]{\@ifundefined{gpa@#1}{\textbf{??#1}}{\csname gpa@#1\endcsname}}
\newcommand{\gpcia}[1]{\@ifundefined{gpcia@#1}{\textbf{??#1}}{\csname gpcia@#1\endcsname}}
\newcommand{\nm}[1]{\@ifundefined{nm@#1}{\textbf{??#1}}{\csname nm@#1\endcsname}}
\newcommand{\oo}[1]{\@ifundefined{oo@#1}{\textbf{??#1}}{\csname oo@#1\endcsname}}
\expandafter\def\csname tp@bag9_flux_dev\endcsname{12.1}
\expandafter\def\csname tpsd@bag9_flux_dev\endcsname{12.1$\pm$0.1}
\expandafter\def\csname tpn@bag9_flux_dev\endcsname{2}
\expandafter\def\csname tpsec@bag9_flux_dev\endcsname{1.69}
\expandafter\def\csname tpnfe@bag9_flux_dev\endcsname{28}
\expandafter\def\csname tpfid@bag9_flux_dev\endcsname{46.0}
\expandafter\def\csname tprec@bag9_flux_dev\endcsname{0.03}
\expandafter\def\csname tp@bag9_flux_dev_g1\endcsname{19.1}
\expandafter\def\csname tpsd@bag9_flux_dev_g1\endcsname{19.1$\pm$0.4}
\expandafter\def\csname tpn@bag9_flux_dev_g1\endcsname{2}
\expandafter\def\csname tpsec@bag9_flux_dev_g1\endcsname{1.67}
\expandafter\def\csname tpnfe@bag9_flux_dev_g1\endcsname{28}
\expandafter\def\csname tpfid@bag9_flux_dev_g1\endcsname{32.7}
\expandafter\def\csname tprec@bag9_flux_dev_g1\endcsname{0.17}
\expandafter\def\csname tp@bag9_kb_dd2_g1\endcsname{26.1}
\expandafter\def\csname tpsd@bag9_kb_dd2_g1\endcsname{26.1$\pm$0.3}
\expandafter\def\csname tpn@bag9_kb_dd2_g1\endcsname{2}
\expandafter\def\csname tpsec@bag9_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@bag9_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@bag9_kb_dd2_g1\endcsname{29.9}
\expandafter\def\csname tprec@bag9_kb_dd2_g1\endcsname{0.17}
\expandafter\def\csname tp@bag9_kb_g1\endcsname{28.1}
\expandafter\def\csname tpsd@bag9_kb_g1\endcsname{28.1$\pm$0.3}
\expandafter\def\csname tpn@bag9_kb_g1\endcsname{2}
\expandafter\def\csname tpsec@bag9_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@bag9_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@bag9_kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@bag9_kb_g1\endcsname{0.49}
\expandafter\def\csname tp@bag9_kd_ad2\endcsname{28.9}
\expandafter\def\csname tpsd@bag9_kd_ad2\endcsname{28.9$\pm$0.1}
\expandafter\def\csname tpn@bag9_kd_ad2\endcsname{2}
\expandafter\def\csname tpsec@bag9_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@bag9_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@bag9_kd_ad2\endcsname{34.8}
\expandafter\def\csname tprec@bag9_kd_ad2\endcsname{0.28}
\expandafter\def\csname tp@bag9_klein\endcsname{14.6}
\expandafter\def\csname tpsd@bag9_klein\endcsname{14.6$\pm$0.2}
\expandafter\def\csname tpn@bag9_klein\endcsname{2}
\expandafter\def\csname tpsec@bag9_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@bag9_klein\endcsname{4}
\expandafter\def\csname tpfid@bag9_klein\endcsname{47.6}
\expandafter\def\csname tprec@bag9_klein\endcsname{0.01}
\expandafter\def\csname tp@bag9_klein_base\endcsname{18.6}
\expandafter\def\csname tpsd@bag9_klein_base\endcsname{18.6$\pm$0.1}
\expandafter\def\csname tpn@bag9_klein_base\endcsname{2}
\expandafter\def\csname tpsec@bag9_klein_base\endcsname{2.82}
\expandafter\def\csname tpnfe@bag9_klein_base\endcsname{100}
\expandafter\def\csname tpfid@bag9_klein_base\endcsname{42.6}
\expandafter\def\csname tprec@bag9_klein_base\endcsname{0.04}
\expandafter\def\csname tp@bag9_real500\endcsname{51.9}
\expandafter\def\csname tpsd@bag9_real500\endcsname{51.9$\pm$0.4}
\expandafter\def\csname tpn@bag9_real500\endcsname{2}
\expandafter\def\csname tp@bag9_sd15\endcsname{20.1}
\expandafter\def\csname tpsd@bag9_sd15\endcsname{20.1$\pm$0.0}
\expandafter\def\csname tpn@bag9_sd15\endcsname{2}
\expandafter\def\csname tpsec@bag9_sd15\endcsname{0.21}
\expandafter\def\csname tpnfe@bag9_sd15\endcsname{60}
\expandafter\def\csname tpfid@bag9_sd15\endcsname{26.6}
\expandafter\def\csname tprec@bag9_sd15\endcsname{0.06}
\expandafter\def\csname tp@bag9_sd15_g2\endcsname{29.4}
\expandafter\def\csname tpsd@bag9_sd15_g2\endcsname{29.4$\pm$0.0}
\expandafter\def\csname tpn@bag9_sd15_g2\endcsname{2}
\expandafter\def\csname tpsec@bag9_sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@bag9_sd15_g2\endcsname{60}
\expandafter\def\csname tpfid@bag9_sd15_g2\endcsname{25.3}
\expandafter\def\csname tprec@bag9_sd15_g2\endcsname{0.31}
\expandafter\def\csname tp@bag9_sd21\endcsname{21.0}
\expandafter\def\csname tpsd@bag9_sd21\endcsname{21.0$\pm$0.3}
\expandafter\def\csname tpn@bag9_sd21\endcsname{2}
\expandafter\def\csname tpsec@bag9_sd21\endcsname{0.20}
\expandafter\def\csname tpnfe@bag9_sd21\endcsname{60}
\expandafter\def\csname tpfid@bag9_sd21\endcsname{28.0}
\expandafter\def\csname tprec@bag9_sd21\endcsname{0.04}
\expandafter\def\csname tp@bag9_sd21_g1\endcsname{27.3}
\expandafter\def\csname tpsd@bag9_sd21_g1\endcsname{27.3$\pm$0.3}
\expandafter\def\csname tpn@bag9_sd21_g1\endcsname{2}
\expandafter\def\csname tpsec@bag9_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@bag9_sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@bag9_sd21_g1\endcsname{50.2}
\expandafter\def\csname tprec@bag9_sd21_g1\endcsname{0.33}
\expandafter\def\csname tp@bag9_sdt4\endcsname{10.7}
\expandafter\def\csname tpsd@bag9_sdt4\endcsname{10.7$\pm$0.0}
\expandafter\def\csname tpn@bag9_sdt4\endcsname{2}
\expandafter\def\csname tpsec@bag9_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@bag9_sdt4\endcsname{4}
\expandafter\def\csname tpfid@bag9_sdt4\endcsname{37.5}
\expandafter\def\csname tprec@bag9_sdt4\endcsname{0.02}
\expandafter\def\csname tp@bag9_sdt4_dd2_g1\endcsname{14.8}
\expandafter\def\csname tpsd@bag9_sdt4_dd2_g1\endcsname{14.8$\pm$0.0}
\expandafter\def\csname tpn@bag9_sdt4_dd2_g1\endcsname{2}
\expandafter\def\csname tpsec@bag9_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@bag9_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@bag9_sdt4_dd2_g1\endcsname{32.1}
\expandafter\def\csname tprec@bag9_sdt4_dd2_g1\endcsname{0.12}
\expandafter\def\csname tp@bag9_sdt_ad1\endcsname{19.5}
\expandafter\def\csname tpsd@bag9_sdt_ad1\endcsname{19.5$\pm$1.4}
\expandafter\def\csname tpn@bag9_sdt_ad1\endcsname{2}
\expandafter\def\csname tpsec@bag9_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@bag9_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@bag9_sdt_ad1\endcsname{30.2}
\expandafter\def\csname tprec@bag9_sdt_ad1\endcsname{0.16}
\expandafter\def\csname tp@bag9_zimage\endcsname{14.6}
\expandafter\def\csname tpsd@bag9_zimage\endcsname{14.6$\pm$0.5}
\expandafter\def\csname tpn@bag9_zimage\endcsname{2}
\expandafter\def\csname tpsec@bag9_zimage\endcsname{3.78}
\expandafter\def\csname tpnfe@bag9_zimage\endcsname{100}
\expandafter\def\csname tpfid@bag9_zimage\endcsname{34.6}
\expandafter\def\csname tprec@bag9_zimage\endcsname{0.03}
\expandafter\def\csname tp@bag9_zimage_g1\endcsname{24.8}
\expandafter\def\csname tpsd@bag9_zimage_g1\endcsname{24.8$\pm$0.2}
\expandafter\def\csname tpn@bag9_zimage_g1\endcsname{2}
\expandafter\def\csname tpsec@bag9_zimage_g1\endcsname{1.92}
\expandafter\def\csname tpnfe@bag9_zimage_g1\endcsname{50}
\expandafter\def\csname tpfid@bag9_zimage_g1\endcsname{29.4}
\expandafter\def\csname tprec@bag9_zimage_g1\endcsname{0.39}
\expandafter\def\csname tp@bag9_zimage_turbo\endcsname{13.1}
\expandafter\def\csname tpsd@bag9_zimage_turbo\endcsname{13.1$\pm$0.1}
\expandafter\def\csname tpn@bag9_zimage_turbo\endcsname{2}
\expandafter\def\csname tpsec@bag9_zimage_turbo\endcsname{0.37}
\expandafter\def\csname tpnfe@bag9_zimage_turbo\endcsname{9}
\expandafter\def\csname tpfid@bag9_zimage_turbo\endcsname{56.2}
\expandafter\def\csname tprec@bag9_zimage_turbo\endcsname{0.00}
\expandafter\def\csname tp@bag9_zt_dd3_g1\endcsname{19.4}
\expandafter\def\csname tpsd@bag9_zt_dd3_g1\endcsname{19.4$\pm$1.3}
\expandafter\def\csname tpn@bag9_zt_dd3_g1\endcsname{2}
\expandafter\def\csname tpsec@bag9_zt_dd3_g1\endcsname{0.37}
\expandafter\def\csname tpnfe@bag9_zt_dd3_g1\endcsname{9}
\expandafter\def\csname tpfid@bag9_zt_dd3_g1\endcsname{26.4}
\expandafter\def\csname tprec@bag9_zt_dd3_g1\endcsname{0.08}
\expandafter\def\csname tp@cap_kb_dd2_g1\endcsname{60.8}
\expandafter\def\csname tpsd@cap_kb_dd2_g1\endcsname{60.8$\pm$0.2}
\expandafter\def\csname tpn@cap_kb_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@cap_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@cap_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@cap_kb_dd2_g1\endcsname{16.0}
\expandafter\def\csname tprec@cap_kb_dd2_g1\endcsname{0.58}
\expandafter\def\csname tp@cap_kb_g1\endcsname{63.0}
\expandafter\def\csname tpsd@cap_kb_g1\endcsname{63.0$\pm$1.3}
\expandafter\def\csname tpn@cap_kb_g1\endcsname{3}
\expandafter\def\csname tpsec@cap_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@cap_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@cap_kb_g1\endcsname{22.9}
\expandafter\def\csname tprec@cap_kb_g1\endcsname{0.84}
\expandafter\def\csname tp@cap_kd_ad2\endcsname{61.5}
\expandafter\def\csname tpsd@cap_kd_ad2\endcsname{61.5$\pm$0.4}
\expandafter\def\csname tpn@cap_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@cap_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@cap_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@cap_kd_ad2\endcsname{20.6}
\expandafter\def\csname tprec@cap_kd_ad2\endcsname{0.70}
\expandafter\def\csname tp@cap_kd_coco\endcsname{61.7}
\expandafter\def\csname tpsd@cap_kd_coco\endcsname{61.7$\pm$0.5}
\expandafter\def\csname tpn@cap_kd_coco\endcsname{3}
\expandafter\def\csname tpsec@cap_kd_coco\endcsname{0.10}
\expandafter\def\csname tpnfe@cap_kd_coco\endcsname{2}
\expandafter\def\csname tpfid@cap_kd_coco\endcsname{21.3}
\expandafter\def\csname tprec@cap_kd_coco\endcsname{0.68}
\expandafter\def\csname tp@cap_klein\endcsname{55.0}
\expandafter\def\csname tpsd@cap_klein\endcsname{55.0$\pm$0.8}
\expandafter\def\csname tpn@cap_klein\endcsname{3}
\expandafter\def\csname tpsec@cap_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@cap_klein\endcsname{4}
\expandafter\def\csname tpfid@cap_klein\endcsname{14.4}
\expandafter\def\csname tprec@cap_klein\endcsname{0.41}
\expandafter\def\csname tp@cap_klein_base\endcsname{55.1}
\expandafter\def\csname tpsd@cap_klein_base\endcsname{55.1$\pm$1.7}
\expandafter\def\csname tpn@cap_klein_base\endcsname{3}
\expandafter\def\csname tpsec@cap_klein_base\endcsname{2.76}
\expandafter\def\csname tpnfe@cap_klein_base\endcsname{100}
\expandafter\def\csname tpfid@cap_klein_base\endcsname{14.8}
\expandafter\def\csname tprec@cap_klein_base\endcsname{0.47}
\expandafter\def\csname tp@cap_klein_base_g2\endcsname{61.6}
\expandafter\def\csname tpsd@cap_klein_base_g2\endcsname{61.6$\pm$1.2}
\expandafter\def\csname tpn@cap_klein_base_g2\endcsname{3}
\expandafter\def\csname tpsec@cap_klein_base_g2\endcsname{2.75}
\expandafter\def\csname tpnfe@cap_klein_base_g2\endcsname{100}
\expandafter\def\csname tpfid@cap_klein_base_g2\endcsname{13.4}
\expandafter\def\csname tprec@cap_klein_base_g2\endcsname{0.68}
\expandafter\def\csname tp@cap_sd15\endcsname{42.2}
\expandafter\def\csname tpsd@cap_sd15\endcsname{42.2$\pm$0.7}
\expandafter\def\csname tpn@cap_sd15\endcsname{3}
\expandafter\def\csname tpsec@cap_sd15\endcsname{0.21}
\expandafter\def\csname tpnfe@cap_sd15\endcsname{60}
\expandafter\def\csname tpfid@cap_sd15\endcsname{19.0}
\expandafter\def\csname tprec@cap_sd15\endcsname{0.24}
\expandafter\def\csname tp@cap_sd15_g2\endcsname{57.3}
\expandafter\def\csname tpsd@cap_sd15_g2\endcsname{57.3$\pm$0.8}
\expandafter\def\csname tpn@cap_sd15_g2\endcsname{3}
\expandafter\def\csname tpsec@cap_sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@cap_sd15_g2\endcsname{60}
\expandafter\def\csname tpfid@cap_sd15_g2\endcsname{26.1}
\expandafter\def\csname tprec@cap_sd15_g2\endcsname{0.48}
\expandafter\def\csname tp@cap_sd21\endcsname{43.5}
\expandafter\def\csname tpsd@cap_sd21\endcsname{43.5$\pm$1.6}
\expandafter\def\csname tpn@cap_sd21\endcsname{3}
\expandafter\def\csname tpsec@cap_sd21\endcsname{0.20}
\expandafter\def\csname tpnfe@cap_sd21\endcsname{60}
\expandafter\def\csname tpfid@cap_sd21\endcsname{20.5}
\expandafter\def\csname tprec@cap_sd21\endcsname{0.19}
\expandafter\def\csname tp@cap_sd21_cfg_late\endcsname{58.4}
\expandafter\def\csname tpsd@cap_sd21_cfg_late\endcsname{58.4$\pm$0.5}
\expandafter\def\csname tpn@cap_sd21_cfg_late\endcsname{3}
\expandafter\def\csname tpsec@cap_sd21_cfg_late\endcsname{0.15}
\expandafter\def\csname tpnfe@cap_sd21_cfg_late\endcsname{45}
\expandafter\def\csname tpfid@cap_sd21_cfg_late\endcsname{42.7}
\expandafter\def\csname tprec@cap_sd21_cfg_late\endcsname{0.43}
\expandafter\def\csname tp@cap_sd21_g1\endcsname{53.5}
\expandafter\def\csname tpsd@cap_sd21_g1\endcsname{53.5$\pm$0.4}
\expandafter\def\csname tpn@cap_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@cap_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@cap_sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@cap_sd21_g1\endcsname{57.2}
\expandafter\def\csname tprec@cap_sd21_g1\endcsname{0.43}
\expandafter\def\csname tp@cap_sd21_g2\endcsname{57.2}
\expandafter\def\csname tpsd@cap_sd21_g2\endcsname{57.2$\pm$0.3}
\expandafter\def\csname tpn@cap_sd21_g2\endcsname{3}
\expandafter\def\csname tpsec@cap_sd21_g2\endcsname{0.20}
\expandafter\def\csname tpnfe@cap_sd21_g2\endcsname{60}
\expandafter\def\csname tpfid@cap_sd21_g2\endcsname{26.0}
\expandafter\def\csname tprec@cap_sd21_g2\endcsname{0.42}
\expandafter\def\csname tp@cap_sd_turbo\endcsname{38.3}
\expandafter\def\csname tpsd@cap_sd_turbo\endcsname{38.3$\pm$0.4}
\expandafter\def\csname tpn@cap_sd_turbo\endcsname{3}
\expandafter\def\csname tpsec@cap_sd_turbo\endcsname{0.02}
\expandafter\def\csname tpnfe@cap_sd_turbo\endcsname{1}
\expandafter\def\csname tpfid@cap_sd_turbo\endcsname{19.1}
\expandafter\def\csname tprec@cap_sd_turbo\endcsname{0.17}
\expandafter\def\csname tp@cap_sdt4\endcsname{32.4}
\expandafter\def\csname tpsd@cap_sdt4\endcsname{32.4$\pm$0.2}
\expandafter\def\csname tpn@cap_sdt4\endcsname{3}
\expandafter\def\csname tpsec@cap_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@cap_sdt4\endcsname{4}
\expandafter\def\csname tpfid@cap_sdt4\endcsname{28.7}
\expandafter\def\csname tprec@cap_sdt4\endcsname{0.15}
\expandafter\def\csname tp@cap_sdt4_dd2_g1\endcsname{42.8}
\expandafter\def\csname tpsd@cap_sdt4_dd2_g1\endcsname{42.8$\pm$0.5}
\expandafter\def\csname tpn@cap_sdt4_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@cap_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@cap_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@cap_sdt4_dd2_g1\endcsname{28.9}
\expandafter\def\csname tprec@cap_sdt4_dd2_g1\endcsname{0.32}
\expandafter\def\csname tp@cap_sdt_ad1\endcsname{53.2}
\expandafter\def\csname tpsd@cap_sdt_ad1\endcsname{53.2$\pm$0.3}
\expandafter\def\csname tpn@cap_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@cap_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@cap_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@cap_sdt_ad1\endcsname{25.6}
\expandafter\def\csname tprec@cap_sdt_ad1\endcsname{0.38}
\expandafter\def\csname tp@cap_sdt_coco\endcsname{52.4}
\expandafter\def\csname tpsd@cap_sdt_coco\endcsname{52.4$\pm$0.7}
\expandafter\def\csname tpn@cap_sdt_coco\endcsname{3}
\expandafter\def\csname tpsec@cap_sdt_coco\endcsname{0.03}
\expandafter\def\csname tpnfe@cap_sdt_coco\endcsname{3}
\expandafter\def\csname tpfid@cap_sdt_coco\endcsname{27.4}
\expandafter\def\csname tprec@cap_sdt_coco\endcsname{0.36}
\expandafter\def\csname tp@cap_sdxl\endcsname{41.8}
\expandafter\def\csname tpsd@cap_sdxl\endcsname{41.8$\pm$0.6}
\expandafter\def\csname tpn@cap_sdxl\endcsname{3}
\expandafter\def\csname tpsec@cap_sdxl\endcsname{1.30}
\expandafter\def\csname tpnfe@cap_sdxl\endcsname{60}
\expandafter\def\csname tpfid@cap_sdxl\endcsname{17.2}
\expandafter\def\csname tprec@cap_sdxl\endcsname{0.14}
\expandafter\def\csname tp@cap_sdxl_g5\endcsname{42.7}
\expandafter\def\csname tpsd@cap_sdxl_g5\endcsname{42.7$\pm$0.5}
\expandafter\def\csname tpn@cap_sdxl_g5\endcsname{3}
\expandafter\def\csname tpsec@cap_sdxl_g5\endcsname{1.26}
\expandafter\def\csname tpnfe@cap_sdxl_g5\endcsname{60}
\expandafter\def\csname tpfid@cap_sdxl_g5\endcsname{16.2}
\expandafter\def\csname tprec@cap_sdxl_g5\endcsname{0.17}
\expandafter\def\csname tp@cap_sdxl_turbo\endcsname{40.5}
\expandafter\def\csname tpsd@cap_sdxl_turbo\endcsname{40.5$\pm$1.0}
\expandafter\def\csname tpn@cap_sdxl_turbo\endcsname{3}
\expandafter\def\csname tpsec@cap_sdxl_turbo\endcsname{0.03}
\expandafter\def\csname tpnfe@cap_sdxl_turbo\endcsname{1}
\expandafter\def\csname tpfid@cap_sdxl_turbo\endcsname{17.2}
\expandafter\def\csname tprec@cap_sdxl_turbo\endcsname{0.19}
\expandafter\def\csname tp@cars_kb_dd2_g1\endcsname{38.8}
\expandafter\def\csname tpsd@cars_kb_dd2_g1\endcsname{38.8$\pm$0.3}
\expandafter\def\csname tpn@cars_kb_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@cars_kb_dd2_g1\endcsname{0.16}
\expandafter\def\csname tpnfe@cars_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tp@cars_kb_g1_s20\endcsname{33.7}
\expandafter\def\csname tpsd@cars_kb_g1_s20\endcsname{33.7$\pm$0.9}
\expandafter\def\csname tpn@cars_kb_g1_s20\endcsname{3}
\expandafter\def\csname tpsec@cars_kb_g1_s20\endcsname{0.57}
\expandafter\def\csname tpnfe@cars_kb_g1_s20\endcsname{20}
\expandafter\def\csname tp@cars_kd_ad2\endcsname{36.2}
\expandafter\def\csname tpsd@cars_kd_ad2\endcsname{36.2$\pm$0.2}
\expandafter\def\csname tpn@cars_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@cars_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@cars_kd_ad2\endcsname{2}
\expandafter\def\csname tp@cars_kd_coco\endcsname{33.0}
\expandafter\def\csname tpsd@cars_kd_coco\endcsname{33.0$\pm$0.5}
\expandafter\def\csname tpn@cars_kd_coco\endcsname{3}
\expandafter\def\csname tpsec@cars_kd_coco\endcsname{0.10}
\expandafter\def\csname tpnfe@cars_kd_coco\endcsname{2}
\expandafter\def\csname tp@cars_klein\endcsname{18.9}
\expandafter\def\csname tpsd@cars_klein\endcsname{18.9$\pm$0.4}
\expandafter\def\csname tpn@cars_klein\endcsname{3}
\expandafter\def\csname tpsec@cars_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@cars_klein\endcsname{4}
\expandafter\def\csname tp@cars_real\endcsname{87.0}
\expandafter\def\csname tpsd@cars_real\endcsname{87.0$\pm$0.2}
\expandafter\def\csname tpn@cars_real\endcsname{3}
\expandafter\def\csname tp@cars_sd21_g1\endcsname{69.6}
\expandafter\def\csname tpsd@cars_sd21_g1\endcsname{69.6$\pm$0.0}
\expandafter\def\csname tpn@cars_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@cars_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@cars_sd21_g1\endcsname{30}
\expandafter\def\csname tp@cars_sdt4\endcsname{46.9}
\expandafter\def\csname tpsd@cars_sdt4\endcsname{46.9$\pm$0.4}
\expandafter\def\csname tpn@cars_sdt4\endcsname{3}
\expandafter\def\csname tpsec@cars_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@cars_sdt4\endcsname{4}
\expandafter\def\csname tp@cars_sdt4_dd2_g1\endcsname{64.8}
\expandafter\def\csname tpsd@cars_sdt4_dd2_g1\endcsname{64.8$\pm$0.5}
\expandafter\def\csname tpn@cars_sdt4_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@cars_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@cars_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tp@cars_sdt_ad1\endcsname{68.3}
\expandafter\def\csname tpsd@cars_sdt_ad1\endcsname{68.3$\pm$0.2}
\expandafter\def\csname tpn@cars_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@cars_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@cars_sdt_ad1\endcsname{3}
\expandafter\def\csname tp@cars_sdt_coco\endcsname{67.8}
\expandafter\def\csname tpsd@cars_sdt_coco\endcsname{67.8$\pm$0.6}
\expandafter\def\csname tpn@cars_sdt_coco\endcsname{3}
\expandafter\def\csname tpsec@cars_sdt_coco\endcsname{0.03}
\expandafter\def\csname tpnfe@cars_sdt_coco\endcsname{3}
\expandafter\def\csname tp@cnx_kb_g1\endcsname{39.1}
\expandafter\def\csname tpsd@cnx_kb_g1\endcsname{39.1$\pm$0.8}
\expandafter\def\csname tpn@cnx_kb_g1\endcsname{3}
\expandafter\def\csname tpsec@cnx_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@cnx_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@cnx_kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@cnx_kb_g1\endcsname{0.49}
\expandafter\def\csname tp@cnx_kd_ad2\endcsname{39.0}
\expandafter\def\csname tpsd@cnx_kd_ad2\endcsname{39.0$\pm$0.2}
\expandafter\def\csname tpn@cnx_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@cnx_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@cnx_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@cnx_kd_ad2\endcsname{34.8}
\expandafter\def\csname tprec@cnx_kd_ad2\endcsname{0.28}
\expandafter\def\csname tp@cnx_klein\endcsname{19.9}
\expandafter\def\csname tpsd@cnx_klein\endcsname{19.9$\pm$0.2}
\expandafter\def\csname tpn@cnx_klein\endcsname{3}
\expandafter\def\csname tpsec@cnx_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@cnx_klein\endcsname{4}
\expandafter\def\csname tpfid@cnx_klein\endcsname{47.6}
\expandafter\def\csname tprec@cnx_klein\endcsname{0.01}
\expandafter\def\csname tp@cnx_real500\endcsname{72.3}
\expandafter\def\csname tpsd@cnx_real500\endcsname{72.3$\pm$0.3}
\expandafter\def\csname tpn@cnx_real500\endcsname{3}
\expandafter\def\csname tp@cnx_sd21_g1\endcsname{42.4}
\expandafter\def\csname tpsd@cnx_sd21_g1\endcsname{42.4$\pm$2.4}
\expandafter\def\csname tpn@cnx_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@cnx_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@cnx_sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@cnx_sd21_g1\endcsname{50.2}
\expandafter\def\csname tprec@cnx_sd21_g1\endcsname{0.33}
\expandafter\def\csname tp@cnx_sdt4\endcsname{20.7}
\expandafter\def\csname tpsd@cnx_sdt4\endcsname{20.7$\pm$0.5}
\expandafter\def\csname tpn@cnx_sdt4\endcsname{3}
\expandafter\def\csname tpsec@cnx_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@cnx_sdt4\endcsname{4}
\expandafter\def\csname tpfid@cnx_sdt4\endcsname{37.5}
\expandafter\def\csname tprec@cnx_sdt4\endcsname{0.02}
\expandafter\def\csname tp@cnx_sdt_ad1\endcsname{41.8}
\expandafter\def\csname tpsd@cnx_sdt_ad1\endcsname{41.8$\pm$1.4}
\expandafter\def\csname tpn@cnx_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@cnx_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@cnx_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@cnx_sdt_ad1\endcsname{30.2}
\expandafter\def\csname tprec@cnx_sdt_ad1\endcsname{0.16}
\expandafter\def\csname tp@cpucal_klein\endcsname{17.2}
\expandafter\def\csname tpsd@cpucal_klein\endcsname{17.2}
\expandafter\def\csname tpn@cpucal_klein\endcsname{1}
\expandafter\def\csname tpsec@cpucal_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@cpucal_klein\endcsname{4}
\expandafter\def\csname tpfid@cpucal_klein\endcsname{47.6}
\expandafter\def\csname tprec@cpucal_klein\endcsname{0.01}
\expandafter\def\csname tp@cpucal_vits_klein\endcsname{15.9}
\expandafter\def\csname tpsd@cpucal_vits_klein\endcsname{15.9}
\expandafter\def\csname tpn@cpucal_vits_klein\endcsname{1}
\expandafter\def\csname tpsec@cpucal_vits_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@cpucal_vits_klein\endcsname{4}
\expandafter\def\csname tpfid@cpucal_vits_klein\endcsname{47.6}
\expandafter\def\csname tprec@cpucal_vits_klein\endcsname{0.01}
\expandafter\def\csname tp@cpucal_wp_tin200_sdxl\endcsname{33.6}
\expandafter\def\csname tpsd@cpucal_wp_tin200_sdxl\endcsname{33.6}
\expandafter\def\csname tpn@cpucal_wp_tin200_sdxl\endcsname{1}
\expandafter\def\csname tpsec@cpucal_wp_tin200_sdxl\endcsname{1.27}
\expandafter\def\csname tpnfe@cpucal_wp_tin200_sdxl\endcsname{60}
\expandafter\def\csname tp@dpdmd\endcsname{13.9}
\expandafter\def\csname tpsd@dpdmd\endcsname{13.9$\pm$0.2}
\expandafter\def\csname tpn@dpdmd\endcsname{3}
\expandafter\def\csname tpsec@dpdmd\endcsname{0.07}
\expandafter\def\csname tpnfe@dpdmd\endcsname{4}
\expandafter\def\csname tpfid@dpdmd\endcsname{44.4}
\expandafter\def\csname tprec@dpdmd\endcsname{0.02}
\expandafter\def\csname tp@dpdmd_ad0\endcsname{21.7}
\expandafter\def\csname tpsd@dpdmd_ad0\endcsname{21.7$\pm$0.1}
\expandafter\def\csname tpn@dpdmd_ad0\endcsname{3}
\expandafter\def\csname tpsec@dpdmd_ad0\endcsname{0.08}
\expandafter\def\csname tpnfe@dpdmd_ad0\endcsname{4}
\expandafter\def\csname tpfid@dpdmd_ad0\endcsname{36.7}
\expandafter\def\csname tprec@dpdmd_ad0\endcsname{0.04}
\expandafter\def\csname tp@dpdmd_ad0_s1\endcsname{21.9}
\expandafter\def\csname tpsd@dpdmd_ad0_s1\endcsname{21.9$\pm$0.3}
\expandafter\def\csname tpn@dpdmd_ad0_s1\endcsname{3}
\expandafter\def\csname tpsec@dpdmd_ad0_s1\endcsname{0.08}
\expandafter\def\csname tpnfe@dpdmd_ad0_s1\endcsname{4}
\expandafter\def\csname tpfid@dpdmd_ad0_s1\endcsname{36.6}
\expandafter\def\csname tprec@dpdmd_ad0_s1\endcsname{0.04}
\expandafter\def\csname tp@dpdmd_ad0_s2\endcsname{21.3}
\expandafter\def\csname tpsd@dpdmd_ad0_s2\endcsname{21.3$\pm$0.2}
\expandafter\def\csname tpn@dpdmd_ad0_s2\endcsname{3}
\expandafter\def\csname tpsec@dpdmd_ad0_s2\endcsname{0.08}
\expandafter\def\csname tpnfe@dpdmd_ad0_s2\endcsname{4}
\expandafter\def\csname tpfid@dpdmd_ad0_s2\endcsname{36.6}
\expandafter\def\csname tprec@dpdmd_ad0_s2\endcsname{0.04}
\expandafter\def\csname tp@dpdmd_ad0_x3\endcsname{21.6}
\expandafter\def\csname tpsd@dpdmd_ad0_x3\endcsname{21.6$\pm$0.3}
\expandafter\def\csname tpn@dpdmd_ad0_x3\endcsname{9}
\expandafter\def\csname tpsec@dpdmd_ad0_x3\endcsname{0.08}
\expandafter\def\csname tpnfe@dpdmd_ad0_x3\endcsname{4}
\expandafter\def\csname tp@dpdmd_ad1\endcsname{27.3}
\expandafter\def\csname tpsd@dpdmd_ad1\endcsname{27.3$\pm$0.2}
\expandafter\def\csname tpn@dpdmd_ad1\endcsname{3}
\expandafter\def\csname tpsec@dpdmd_ad1\endcsname{0.07}
\expandafter\def\csname tpnfe@dpdmd_ad1\endcsname{3}
\expandafter\def\csname tpfid@dpdmd_ad1\endcsname{32.0}
\expandafter\def\csname tprec@dpdmd_ad1\endcsname{0.05}
\expandafter\def\csname tp@dpdmd_dd1_g1\endcsname{15.8}
\expandafter\def\csname tpsd@dpdmd_dd1_g1\endcsname{15.8$\pm$0.1}
\expandafter\def\csname tpn@dpdmd_dd1_g1\endcsname{3}
\expandafter\def\csname tpsec@dpdmd_dd1_g1\endcsname{0.09}
\expandafter\def\csname tpnfe@dpdmd_dd1_g1\endcsname{4}
\expandafter\def\csname tpfid@dpdmd_dd1_g1\endcsname{43.4}
\expandafter\def\csname tprec@dpdmd_dd1_g1\endcsname{0.02}
\expandafter\def\csname tp@flux_dev\endcsname{12.6}
\expandafter\def\csname tpsd@flux_dev\endcsname{12.6$\pm$0.3}
\expandafter\def\csname tpn@flux_dev\endcsname{3}
\expandafter\def\csname tpsec@flux_dev\endcsname{1.69}
\expandafter\def\csname tpnfe@flux_dev\endcsname{28}
\expandafter\def\csname tpfid@flux_dev\endcsname{46.0}
\expandafter\def\csname tprec@flux_dev\endcsname{0.03}
\expandafter\def\csname tp@flux_dev_g1\endcsname{30.6}
\expandafter\def\csname tpsd@flux_dev_g1\endcsname{30.6$\pm$0.5}
\expandafter\def\csname tpn@flux_dev_g1\endcsname{3}
\expandafter\def\csname tpsec@flux_dev_g1\endcsname{1.67}
\expandafter\def\csname tpnfe@flux_dev_g1\endcsname{28}
\expandafter\def\csname tpfid@flux_dev_g1\endcsname{32.7}
\expandafter\def\csname tprec@flux_dev_g1\endcsname{0.17}
\expandafter\def\csname tp@flux_dev_g2\endcsname{17.1}
\expandafter\def\csname tpsd@flux_dev_g2\endcsname{17.1$\pm$0.3}
\expandafter\def\csname tpn@flux_dev_g2\endcsname{3}
\expandafter\def\csname tpsec@flux_dev_g2\endcsname{1.65}
\expandafter\def\csname tpnfe@flux_dev_g2\endcsname{28}
\expandafter\def\csname tpfid@flux_dev_g2\endcsname{38.6}
\expandafter\def\csname tprec@flux_dev_g2\endcsname{0.05}
\expandafter\def\csname tp@flux_schnell\endcsname{20.4}
\expandafter\def\csname tpsd@flux_schnell\endcsname{20.4$\pm$0.1}
\expandafter\def\csname tpn@flux_schnell\endcsname{3}
\expandafter\def\csname tpsec@flux_schnell\endcsname{0.22}
\expandafter\def\csname tpnfe@flux_schnell\endcsname{4}
\expandafter\def\csname tpfid@flux_schnell\endcsname{39.8}
\expandafter\def\csname tprec@flux_schnell\endcsname{0.01}
\expandafter\def\csname tp@food101_kb_dd2_g1\endcsname{25.9}
\expandafter\def\csname tpsd@food101_kb_dd2_g1\endcsname{25.9$\pm$0.1}
\expandafter\def\csname tpn@food101_kb_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@food101_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@food101_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tprec@food101_kb_dd2_g1\endcsname{0.24}
\expandafter\def\csname tp@food101_kb_g1_s20\endcsname{29.8}
\expandafter\def\csname tpsd@food101_kb_g1_s20\endcsname{29.8$\pm$0.2}
\expandafter\def\csname tpn@food101_kb_g1_s20\endcsname{3}
\expandafter\def\csname tpsec@food101_kb_g1_s20\endcsname{0.57}
\expandafter\def\csname tpnfe@food101_kb_g1_s20\endcsname{20}
\expandafter\def\csname tprec@food101_kb_g1_s20\endcsname{0.67}
\expandafter\def\csname tp@food101_kd_ad2\endcsname{30.9}
\expandafter\def\csname tpsd@food101_kd_ad2\endcsname{30.9$\pm$0.2}
\expandafter\def\csname tpn@food101_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@food101_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@food101_kd_ad2\endcsname{2}
\expandafter\def\csname tprec@food101_kd_ad2\endcsname{0.29}
\expandafter\def\csname tp@food101_kd_coco\endcsname{31.8}
\expandafter\def\csname tpsd@food101_kd_coco\endcsname{31.8$\pm$0.6}
\expandafter\def\csname tpn@food101_kd_coco\endcsname{3}
\expandafter\def\csname tpsec@food101_kd_coco\endcsname{0.10}
\expandafter\def\csname tpnfe@food101_kd_coco\endcsname{2}
\expandafter\def\csname tp@food101_klein\endcsname{10.5}
\expandafter\def\csname tpsd@food101_klein\endcsname{10.5$\pm$0.3}
\expandafter\def\csname tpn@food101_klein\endcsname{3}
\expandafter\def\csname tpsec@food101_klein\endcsname{0.21}
\expandafter\def\csname tpnfe@food101_klein\endcsname{4}
\expandafter\def\csname tprec@food101_klein\endcsname{0.01}
\expandafter\def\csname tp@food101_real500\endcsname{79.3}
\expandafter\def\csname tpsd@food101_real500\endcsname{79.3$\pm$0.3}
\expandafter\def\csname tpn@food101_real500\endcsname{3}
\expandafter\def\csname tp@food101_sd21_g1\endcsname{37.3}
\expandafter\def\csname tpsd@food101_sd21_g1\endcsname{37.3$\pm$0.2}
\expandafter\def\csname tpn@food101_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@food101_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@food101_sd21_g1\endcsname{30}
\expandafter\def\csname tprec@food101_sd21_g1\endcsname{0.53}
\expandafter\def\csname tp@food101_sdt4\endcsname{10.0}
\expandafter\def\csname tpsd@food101_sdt4\endcsname{10.0$\pm$0.3}
\expandafter\def\csname tpn@food101_sdt4\endcsname{3}
\expandafter\def\csname tpsec@food101_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@food101_sdt4\endcsname{4}
\expandafter\def\csname tprec@food101_sdt4\endcsname{0.01}
\expandafter\def\csname tp@food101_sdt4_dd2_g1\endcsname{27.3}
\expandafter\def\csname tpsd@food101_sdt4_dd2_g1\endcsname{27.3$\pm$0.2}
\expandafter\def\csname tpn@food101_sdt4_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@food101_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@food101_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tprec@food101_sdt4_dd2_g1\endcsname{0.11}
\expandafter\def\csname tp@food101_sdt_ad1\endcsname{31.8}
\expandafter\def\csname tpsd@food101_sdt_ad1\endcsname{31.8$\pm$0.2}
\expandafter\def\csname tpn@food101_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@food101_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@food101_sdt_ad1\endcsname{3}
\expandafter\def\csname tprec@food101_sdt_ad1\endcsname{0.14}
\expandafter\def\csname tp@food101_sdt_coco\endcsname{31.3}
\expandafter\def\csname tpsd@food101_sdt_coco\endcsname{31.3$\pm$0.7}
\expandafter\def\csname tpn@food101_sdt_coco\endcsname{3}
\expandafter\def\csname tpsec@food101_sdt_coco\endcsname{0.03}
\expandafter\def\csname tpnfe@food101_sdt_coco\endcsname{3}
\expandafter\def\csname tp@ft_kb_dd2_g1\endcsname{84.8}
\expandafter\def\csname tpsd@ft_kb_dd2_g1\endcsname{84.8$\pm$0.1}
\expandafter\def\csname tpn@ft_kb_dd2_g1\endcsname{2}
\expandafter\def\csname tpsec@ft_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@ft_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@ft_kb_dd2_g1\endcsname{29.9}
\expandafter\def\csname tprec@ft_kb_dd2_g1\endcsname{0.17}
\expandafter\def\csname tp@ft_kb_g1\endcsname{84.7}
\expandafter\def\csname tpsd@ft_kb_g1\endcsname{84.7$\pm$0.3}
\expandafter\def\csname tpn@ft_kb_g1\endcsname{2}
\expandafter\def\csname tpsec@ft_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@ft_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@ft_kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@ft_kb_g1\endcsname{0.49}
\expandafter\def\csname tp@ft_klein\endcsname{83.1}
\expandafter\def\csname tpsd@ft_klein\endcsname{83.1$\pm$0.1}
\expandafter\def\csname tpn@ft_klein\endcsname{2}
\expandafter\def\csname tpsec@ft_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@ft_klein\endcsname{4}
\expandafter\def\csname tpfid@ft_klein\endcsname{47.6}
\expandafter\def\csname tprec@ft_klein\endcsname{0.01}
\expandafter\def\csname tp@ft_klein_base\endcsname{84.2}
\expandafter\def\csname tpsd@ft_klein_base\endcsname{84.2$\pm$0.4}
\expandafter\def\csname tpn@ft_klein_base\endcsname{2}
\expandafter\def\csname tpsec@ft_klein_base\endcsname{2.82}
\expandafter\def\csname tpnfe@ft_klein_base\endcsname{100}
\expandafter\def\csname tpfid@ft_klein_base\endcsname{42.6}
\expandafter\def\csname tprec@ft_klein_base\endcsname{0.04}
\expandafter\def\csname tp@ft_real500\endcsname{97.1}
\expandafter\def\csname tpsd@ft_real500\endcsname{97.1$\pm$0.0}
\expandafter\def\csname tpn@ft_real500\endcsname{2}
\expandafter\def\csname tp@ft_sd15\endcsname{90.5}
\expandafter\def\csname tpsd@ft_sd15\endcsname{90.5$\pm$0.2}
\expandafter\def\csname tpn@ft_sd15\endcsname{2}
\expandafter\def\csname tpsec@ft_sd15\endcsname{0.21}
\expandafter\def\csname tpnfe@ft_sd15\endcsname{60}
\expandafter\def\csname tpfid@ft_sd15\endcsname{26.6}
\expandafter\def\csname tprec@ft_sd15\endcsname{0.06}
\expandafter\def\csname tp@ft_sd15_g2\endcsname{91.7}
\expandafter\def\csname tpsd@ft_sd15_g2\endcsname{91.7$\pm$0.1}
\expandafter\def\csname tpn@ft_sd15_g2\endcsname{2}
\expandafter\def\csname tpsec@ft_sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@ft_sd15_g2\endcsname{60}
\expandafter\def\csname tpfid@ft_sd15_g2\endcsname{25.3}
\expandafter\def\csname tprec@ft_sd15_g2\endcsname{0.31}
\expandafter\def\csname tp@hp_flux_dev\endcsname{9.0}
\expandafter\def\csname tpsd@hp_flux_dev\endcsname{9.0$\pm$0.2}
\expandafter\def\csname tpn@hp_flux_dev\endcsname{2}
\expandafter\def\csname tpsec@hp_flux_dev\endcsname{1.69}
\expandafter\def\csname tpnfe@hp_flux_dev\endcsname{28}
\expandafter\def\csname tpfid@hp_flux_dev\endcsname{46.0}
\expandafter\def\csname tprec@hp_flux_dev\endcsname{0.03}
\expandafter\def\csname tp@hp_flux_dev_g1\endcsname{14.4}
\expandafter\def\csname tpsd@hp_flux_dev_g1\endcsname{14.4$\pm$0.0}
\expandafter\def\csname tpn@hp_flux_dev_g1\endcsname{2}
\expandafter\def\csname tpsec@hp_flux_dev_g1\endcsname{1.67}
\expandafter\def\csname tpnfe@hp_flux_dev_g1\endcsname{28}
\expandafter\def\csname tpfid@hp_flux_dev_g1\endcsname{32.7}
\expandafter\def\csname tprec@hp_flux_dev_g1\endcsname{0.17}
\expandafter\def\csname tp@hp_kb_dd2_g1\endcsname{19.7}
\expandafter\def\csname tpsd@hp_kb_dd2_g1\endcsname{19.7$\pm$0.2}
\expandafter\def\csname tpn@hp_kb_dd2_g1\endcsname{2}
\expandafter\def\csname tpsec@hp_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@hp_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@hp_kb_dd2_g1\endcsname{29.9}
\expandafter\def\csname tprec@hp_kb_dd2_g1\endcsname{0.17}
\expandafter\def\csname tp@hp_kb_g1\endcsname{20.7}
\expandafter\def\csname tpsd@hp_kb_g1\endcsname{20.7$\pm$0.5}
\expandafter\def\csname tpn@hp_kb_g1\endcsname{2}
\expandafter\def\csname tpsec@hp_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@hp_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@hp_kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@hp_kb_g1\endcsname{0.49}
\expandafter\def\csname tp@hp_kd_ad2\endcsname{21.4}
\expandafter\def\csname tpsd@hp_kd_ad2\endcsname{21.4$\pm$0.7}
\expandafter\def\csname tpn@hp_kd_ad2\endcsname{2}
\expandafter\def\csname tpsec@hp_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@hp_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@hp_kd_ad2\endcsname{34.8}
\expandafter\def\csname tprec@hp_kd_ad2\endcsname{0.28}
\expandafter\def\csname tp@hp_klein\endcsname{13.6}
\expandafter\def\csname tpsd@hp_klein\endcsname{13.6$\pm$1.8}
\expandafter\def\csname tpn@hp_klein\endcsname{2}
\expandafter\def\csname tpsec@hp_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@hp_klein\endcsname{4}
\expandafter\def\csname tpfid@hp_klein\endcsname{47.6}
\expandafter\def\csname tprec@hp_klein\endcsname{0.01}
\expandafter\def\csname tp@hp_klein_base\endcsname{16.4}
\expandafter\def\csname tpsd@hp_klein_base\endcsname{16.4$\pm$0.9}
\expandafter\def\csname tpn@hp_klein_base\endcsname{2}
\expandafter\def\csname tpsec@hp_klein_base\endcsname{2.82}
\expandafter\def\csname tpnfe@hp_klein_base\endcsname{100}
\expandafter\def\csname tpfid@hp_klein_base\endcsname{42.6}
\expandafter\def\csname tprec@hp_klein_base\endcsname{0.04}
\expandafter\def\csname tp@hp_real500\endcsname{34.7}
\expandafter\def\csname tpsd@hp_real500\endcsname{34.7$\pm$1.0}
\expandafter\def\csname tpn@hp_real500\endcsname{2}
\expandafter\def\csname tp@hp_sd15\endcsname{18.9}
\expandafter\def\csname tpsd@hp_sd15\endcsname{18.9$\pm$0.0}
\expandafter\def\csname tpn@hp_sd15\endcsname{2}
\expandafter\def\csname tpsec@hp_sd15\endcsname{0.21}
\expandafter\def\csname tpnfe@hp_sd15\endcsname{60}
\expandafter\def\csname tpfid@hp_sd15\endcsname{26.6}
\expandafter\def\csname tprec@hp_sd15\endcsname{0.06}
\expandafter\def\csname tp@hp_sd15_g2\endcsname{26.4}
\expandafter\def\csname tpsd@hp_sd15_g2\endcsname{26.4$\pm$2.8}
\expandafter\def\csname tpn@hp_sd15_g2\endcsname{2}
\expandafter\def\csname tpsec@hp_sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@hp_sd15_g2\endcsname{60}
\expandafter\def\csname tpfid@hp_sd15_g2\endcsname{25.3}
\expandafter\def\csname tprec@hp_sd15_g2\endcsname{0.31}
\expandafter\def\csname tp@hp_sd21\endcsname{16.9}
\expandafter\def\csname tpsd@hp_sd21\endcsname{16.9$\pm$0.4}
\expandafter\def\csname tpn@hp_sd21\endcsname{2}
\expandafter\def\csname tpsec@hp_sd21\endcsname{0.20}
\expandafter\def\csname tpnfe@hp_sd21\endcsname{60}
\expandafter\def\csname tpfid@hp_sd21\endcsname{28.0}
\expandafter\def\csname tprec@hp_sd21\endcsname{0.04}
\expandafter\def\csname tp@hp_sd21_g1\endcsname{21.7}
\expandafter\def\csname tpsd@hp_sd21_g1\endcsname{21.7$\pm$1.6}
\expandafter\def\csname tpn@hp_sd21_g1\endcsname{2}
\expandafter\def\csname tpsec@hp_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@hp_sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@hp_sd21_g1\endcsname{50.2}
\expandafter\def\csname tprec@hp_sd21_g1\endcsname{0.33}
\expandafter\def\csname tp@hp_sdt4\endcsname{11.1}
\expandafter\def\csname tpsd@hp_sdt4\endcsname{11.1$\pm$0.3}
\expandafter\def\csname tpn@hp_sdt4\endcsname{2}
\expandafter\def\csname tpsec@hp_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@hp_sdt4\endcsname{4}
\expandafter\def\csname tpfid@hp_sdt4\endcsname{37.5}
\expandafter\def\csname tprec@hp_sdt4\endcsname{0.02}
\expandafter\def\csname tp@hp_sdt4_dd2_g1\endcsname{16.9}
\expandafter\def\csname tpsd@hp_sdt4_dd2_g1\endcsname{16.9$\pm$0.0}
\expandafter\def\csname tpn@hp_sdt4_dd2_g1\endcsname{2}
\expandafter\def\csname tpsec@hp_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@hp_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@hp_sdt4_dd2_g1\endcsname{32.1}
\expandafter\def\csname tprec@hp_sdt4_dd2_g1\endcsname{0.12}
\expandafter\def\csname tp@hp_sdt_ad1\endcsname{20.1}
\expandafter\def\csname tpsd@hp_sdt_ad1\endcsname{20.1$\pm$0.3}
\expandafter\def\csname tpn@hp_sdt_ad1\endcsname{2}
\expandafter\def\csname tpsec@hp_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@hp_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@hp_sdt_ad1\endcsname{30.2}
\expandafter\def\csname tprec@hp_sdt_ad1\endcsname{0.16}
\expandafter\def\csname tp@hp_zimage\endcsname{13.3}
\expandafter\def\csname tpsd@hp_zimage\endcsname{13.3$\pm$0.2}
\expandafter\def\csname tpn@hp_zimage\endcsname{2}
\expandafter\def\csname tpsec@hp_zimage\endcsname{3.78}
\expandafter\def\csname tpnfe@hp_zimage\endcsname{100}
\expandafter\def\csname tpfid@hp_zimage\endcsname{34.6}
\expandafter\def\csname tprec@hp_zimage\endcsname{0.03}
\expandafter\def\csname tp@hp_zimage_g1\endcsname{19.4}
\expandafter\def\csname tpsd@hp_zimage_g1\endcsname{19.4$\pm$0.1}
\expandafter\def\csname tpn@hp_zimage_g1\endcsname{2}
\expandafter\def\csname tpsec@hp_zimage_g1\endcsname{1.92}
\expandafter\def\csname tpnfe@hp_zimage_g1\endcsname{50}
\expandafter\def\csname tpfid@hp_zimage_g1\endcsname{29.4}
\expandafter\def\csname tprec@hp_zimage_g1\endcsname{0.39}
\expandafter\def\csname tp@hp_zimage_turbo\endcsname{7.7}
\expandafter\def\csname tpsd@hp_zimage_turbo\endcsname{7.7$\pm$0.3}
\expandafter\def\csname tpn@hp_zimage_turbo\endcsname{2}
\expandafter\def\csname tpsec@hp_zimage_turbo\endcsname{0.37}
\expandafter\def\csname tpnfe@hp_zimage_turbo\endcsname{9}
\expandafter\def\csname tpfid@hp_zimage_turbo\endcsname{56.2}
\expandafter\def\csname tprec@hp_zimage_turbo\endcsname{0.00}
\expandafter\def\csname tp@hp_zt_dd3_g1\endcsname{17.9}
\expandafter\def\csname tpsd@hp_zt_dd3_g1\endcsname{17.9$\pm$4.7}
\expandafter\def\csname tpn@hp_zt_dd3_g1\endcsname{2}
\expandafter\def\csname tpsec@hp_zt_dd3_g1\endcsname{0.37}
\expandafter\def\csname tpnfe@hp_zt_dd3_g1\endcsname{9}
\expandafter\def\csname tpfid@hp_zt_dd3_g1\endcsname{26.4}
\expandafter\def\csname tprec@hp_zt_dd3_g1\endcsname{0.08}
\expandafter\def\csname tp@in1k_kb_dd2_g1\endcsname{17.7}
\expandafter\def\csname tpsd@in1k_kb_dd2_g1\endcsname{17.7$\pm$0.2}
\expandafter\def\csname tpn@in1k_kb_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@in1k_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@in1k_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tp@in1k_kb_g1_s20\endcsname{17.6}
\expandafter\def\csname tpsd@in1k_kb_g1_s20\endcsname{17.6$\pm$0.2}
\expandafter\def\csname tpn@in1k_kb_g1_s20\endcsname{3}
\expandafter\def\csname tpsec@in1k_kb_g1_s20\endcsname{0.57}
\expandafter\def\csname tpnfe@in1k_kb_g1_s20\endcsname{20}
\expandafter\def\csname tp@in1k_kb_g1_s20_full\endcsname{37.2}
\expandafter\def\csname tpsd@in1k_kb_g1_s20_full\endcsname{37.2$\pm$0.1}
\expandafter\def\csname tpn@in1k_kb_g1_s20_full\endcsname{3}
\expandafter\def\csname tpsec@in1k_kb_g1_s20_full\endcsname{0.57}
\expandafter\def\csname tpnfe@in1k_kb_g1_s20_full\endcsname{20}
\expandafter\def\csname tp@in1k_kb_g4_s20\endcsname{10.3}
\expandafter\def\csname tpsd@in1k_kb_g4_s20\endcsname{10.3$\pm$0.2}
\expandafter\def\csname tpn@in1k_kb_g4_s20\endcsname{3}
\expandafter\def\csname tpsec@in1k_kb_g4_s20\endcsname{1.13}
\expandafter\def\csname tpnfe@in1k_kb_g4_s20\endcsname{40}
\expandafter\def\csname tp@in1k_kd_ad2\endcsname{18.6}
\expandafter\def\csname tpsd@in1k_kd_ad2\endcsname{18.6$\pm$0.0}
\expandafter\def\csname tpn@in1k_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@in1k_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@in1k_kd_ad2\endcsname{2}
\expandafter\def\csname tp@in1k_kd_ad2_full\endcsname{34.2}
\expandafter\def\csname tpsd@in1k_kd_ad2_full\endcsname{34.2$\pm$0.1}
\expandafter\def\csname tpn@in1k_kd_ad2_full\endcsname{3}
\expandafter\def\csname tpsec@in1k_kd_ad2_full\endcsname{0.10}
\expandafter\def\csname tpnfe@in1k_kd_ad2_full\endcsname{2}
\expandafter\def\csname tp@in1k_klein\endcsname{8.4}
\expandafter\def\csname tpsd@in1k_klein\endcsname{8.4$\pm$0.1}
\expandafter\def\csname tpn@in1k_klein\endcsname{3}
\expandafter\def\csname tpsec@in1k_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@in1k_klein\endcsname{4}
\expandafter\def\csname tp@in1k_klein_full\endcsname{8.4}
\expandafter\def\csname tpsd@in1k_klein_full\endcsname{8.4$\pm$0.1}
\expandafter\def\csname tpn@in1k_klein_full\endcsname{3}
\expandafter\def\csname tpsec@in1k_klein_full\endcsname{0.14}
\expandafter\def\csname tpnfe@in1k_klein_full\endcsname{4}
\expandafter\def\csname tp@in1k_mix_kd_ad2\endcsname{76.5}
\expandafter\def\csname tpsd@in1k_mix_kd_ad2\endcsname{76.5$\pm$0.2}
\expandafter\def\csname tpn@in1k_mix_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@in1k_mix_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@in1k_mix_kd_ad2\endcsname{2}
\expandafter\def\csname tp@in1k_mix_klein\endcsname{76.0}
\expandafter\def\csname tpsd@in1k_mix_klein\endcsname{76.0$\pm$0.0}
\expandafter\def\csname tpn@in1k_mix_klein\endcsname{3}
\expandafter\def\csname tpsec@in1k_mix_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@in1k_mix_klein\endcsname{4}
\expandafter\def\csname tp@in1k_real100\endcsname{48.5}
\expandafter\def\csname tpsd@in1k_real100\endcsname{48.5$\pm$0.2}
\expandafter\def\csname tpn@in1k_real100\endcsname{3}
\expandafter\def\csname tp@in1k_real_e200\endcsname{76.7}
\expandafter\def\csname tpsd@in1k_real_e200\endcsname{76.7$\pm$0.2}
\expandafter\def\csname tpn@in1k_real_e200\endcsname{3}
\expandafter\def\csname tp@in1k_sd15\endcsname{15.3}
\expandafter\def\csname tpsd@in1k_sd15\endcsname{15.3$\pm$0.1}
\expandafter\def\csname tpn@in1k_sd15\endcsname{3}
\expandafter\def\csname tpsec@in1k_sd15\endcsname{0.21}
\expandafter\def\csname tpnfe@in1k_sd15\endcsname{60}
\expandafter\def\csname tp@in1k_sd15_g2\endcsname{24.5}
\expandafter\def\csname tpsd@in1k_sd15_g2\endcsname{24.5$\pm$0.1}
\expandafter\def\csname tpn@in1k_sd15_g2\endcsname{3}
\expandafter\def\csname tpsec@in1k_sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@in1k_sd15_g2\endcsname{60}
\expandafter\def\csname tp@in1k_sd21_g1\endcsname{18.8}
\expandafter\def\csname tpsd@in1k_sd21_g1\endcsname{18.8$\pm$0.4}
\expandafter\def\csname tpn@in1k_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@in1k_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@in1k_sd21_g1\endcsname{30}
\expandafter\def\csname tp@in1k_sdt4\endcsname{8.8}
\expandafter\def\csname tpsd@in1k_sdt4\endcsname{8.8$\pm$0.1}
\expandafter\def\csname tpn@in1k_sdt4\endcsname{3}
\expandafter\def\csname tpsec@in1k_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@in1k_sdt4\endcsname{4}
\expandafter\def\csname tp@in1k_sdt4_dd2_g1\endcsname{15.2}
\expandafter\def\csname tpsd@in1k_sdt4_dd2_g1\endcsname{15.2$\pm$0.5}
\expandafter\def\csname tpn@in1k_sdt4_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@in1k_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@in1k_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tp@in1k_sdt4_full\endcsname{12.7}
\expandafter\def\csname tpsd@in1k_sdt4_full\endcsname{12.7$\pm$0.2}
\expandafter\def\csname tpn@in1k_sdt4_full\endcsname{3}
\expandafter\def\csname tpsec@in1k_sdt4_full\endcsname{0.03}
\expandafter\def\csname tpnfe@in1k_sdt4_full\endcsname{4}
\expandafter\def\csname tp@in1k_sdt_ad1\endcsname{19.1}
\expandafter\def\csname tpsd@in1k_sdt_ad1\endcsname{19.1$\pm$0.1}
\expandafter\def\csname tpn@in1k_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@in1k_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@in1k_sdt_ad1\endcsname{3}
\expandafter\def\csname tp@in1k_sdt_ad1_full\endcsname{32.1}
\expandafter\def\csname tpsd@in1k_sdt_ad1_full\endcsname{32.1$\pm$0.3}
\expandafter\def\csname tpn@in1k_sdt_ad1_full\endcsname{3}
\expandafter\def\csname tpsec@in1k_sdt_ad1_full\endcsname{0.03}
\expandafter\def\csname tpnfe@in1k_sdt_ad1_full\endcsname{3}
\expandafter\def\csname tp@kb_b2d25_g1\endcsname{43.5}
\expandafter\def\csname tpsd@kb_b2d25_g1\endcsname{43.5$\pm$0.3}
\expandafter\def\csname tpn@kb_b2d25_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_b2d25_g1\endcsname{1.39}
\expandafter\def\csname tpnfe@kb_b2d25_g1\endcsname{50}
\expandafter\def\csname tpfid@kb_b2d25_g1\endcsname{31.4}
\expandafter\def\csname tprec@kb_b2d25_g1\endcsname{0.33}
\expandafter\def\csname tp@kb_b2d25_g2\endcsname{32.3}
\expandafter\def\csname tpsd@kb_b2d25_g2\endcsname{32.3$\pm$0.6}
\expandafter\def\csname tpn@kb_b2d25_g2\endcsname{3}
\expandafter\def\csname tpsec@kb_b2d25_g2\endcsname{2.06}
\expandafter\def\csname tpnfe@kb_b2d25_g2\endcsname{75}
\expandafter\def\csname tpfid@kb_b2d25_g2\endcsname{32.4}
\expandafter\def\csname tprec@kb_b2d25_g2\endcsname{0.11}
\expandafter\def\csname tp@kb_b2d40_g1\endcsname{44.0}
\expandafter\def\csname tpsd@kb_b2d40_g1\endcsname{44.0$\pm$0.2}
\expandafter\def\csname tpn@kb_b2d40_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_b2d40_g1\endcsname{1.39}
\expandafter\def\csname tpnfe@kb_b2d40_g1\endcsname{50}
\expandafter\def\csname tpfid@kb_b2d40_g1\endcsname{34.4}
\expandafter\def\csname tprec@kb_b2d40_g1\endcsname{0.43}
\expandafter\def\csname tp@kb_cads_g4\endcsname{11.3}
\expandafter\def\csname tpsd@kb_cads_g4\endcsname{11.3$\pm$0.9}
\expandafter\def\csname tpn@kb_cads_g4\endcsname{3}
\expandafter\def\csname tpsec@kb_cads_g4\endcsname{2.74}
\expandafter\def\csname tpnfe@kb_cads_g4\endcsname{100}
\expandafter\def\csname tpfid@kb_cads_g4\endcsname{283.8}
\expandafter\def\csname tprec@kb_cads_g4\endcsname{0.00}
\expandafter\def\csname tp@kb_cfg_early\endcsname{24.4}
\expandafter\def\csname tpsd@kb_cfg_early\endcsname{24.4$\pm$0.3}
\expandafter\def\csname tpn@kb_cfg_early\endcsname{3}
\expandafter\def\csname tpsec@kb_cfg_early\endcsname{2.06}
\expandafter\def\csname tpnfe@kb_cfg_early\endcsname{75}
\expandafter\def\csname tpfid@kb_cfg_early\endcsname{41.2}
\expandafter\def\csname tprec@kb_cfg_early\endcsname{0.05}
\expandafter\def\csname tp@kb_cfg_gt51\endcsname{22.8}
\expandafter\def\csname tpsd@kb_cfg_gt51\endcsname{22.8$\pm$0.3}
\expandafter\def\csname tpn@kb_cfg_gt51\endcsname{3}
\expandafter\def\csname tpsec@kb_cfg_gt51\endcsname{2.52}
\expandafter\def\csname tpnfe@kb_cfg_gt51\endcsname{92}
\expandafter\def\csname tpfid@kb_cfg_gt51\endcsname{42.3}
\expandafter\def\csname tprec@kb_cfg_gt51\endcsname{0.04}
\expandafter\def\csname tp@kb_cfg_late\endcsname{45.9}
\expandafter\def\csname tpsd@kb_cfg_late\endcsname{45.9$\pm$0.8}
\expandafter\def\csname tpn@kb_cfg_late\endcsname{3}
\expandafter\def\csname tpsec@kb_cfg_late\endcsname{2.07}
\expandafter\def\csname tpnfe@kb_cfg_late\endcsname{75}
\expandafter\def\csname tpfid@kb_cfg_late\endcsname{28.5}
\expandafter\def\csname tprec@kb_cfg_late\endcsname{0.45}
\expandafter\def\csname tp@kb_cfg_lt51\endcsname{45.2}
\expandafter\def\csname tpsd@kb_cfg_lt51\endcsname{45.2$\pm$0.4}
\expandafter\def\csname tpn@kb_cfg_lt51\endcsname{3}
\expandafter\def\csname tpsec@kb_cfg_lt51\endcsname{1.61}
\expandafter\def\csname tpnfe@kb_cfg_lt51\endcsname{58}
\expandafter\def\csname tpfid@kb_cfg_lt51\endcsname{32.4}
\expandafter\def\csname tprec@kb_cfg_lt51\endcsname{0.51}
\expandafter\def\csname tp@kb_d2b10_g2\endcsname{26.3}
\expandafter\def\csname tpsd@kb_d2b10_g2\endcsname{26.3$\pm$0.3}
\expandafter\def\csname tpn@kb_d2b10_g2\endcsname{3}
\expandafter\def\csname tpsec@kb_d2b10_g2\endcsname{2.47}
\expandafter\def\csname tpnfe@kb_d2b10_g2\endcsname{90}
\expandafter\def\csname tpfid@kb_d2b10_g2\endcsname{41.1}
\expandafter\def\csname tprec@kb_d2b10_g2\endcsname{0.04}
\expandafter\def\csname tp@kb_d2b25_g1\endcsname{26.1}
\expandafter\def\csname tpsd@kb_d2b25_g1\endcsname{26.1$\pm$0.4}
\expandafter\def\csname tpn@kb_d2b25_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_d2b25_g1\endcsname{1.40}
\expandafter\def\csname tpnfe@kb_d2b25_g1\endcsname{50}
\expandafter\def\csname tpfid@kb_d2b25_g1\endcsname{39.4}
\expandafter\def\csname tprec@kb_d2b25_g1\endcsname{0.03}
\expandafter\def\csname tp@kb_d2b25_g2\endcsname{24.9}
\expandafter\def\csname tpsd@kb_d2b25_g2\endcsname{24.9$\pm$0.2}
\expandafter\def\csname tpn@kb_d2b25_g2\endcsname{3}
\expandafter\def\csname tpsec@kb_d2b25_g2\endcsname{2.07}
\expandafter\def\csname tpnfe@kb_d2b25_g2\endcsname{75}
\expandafter\def\csname tpfid@kb_d2b25_g2\endcsname{40.6}
\expandafter\def\csname tprec@kb_d2b25_g2\endcsname{0.02}
\expandafter\def\csname tp@kb_d2b40_g1\endcsname{23.2}
\expandafter\def\csname tpsd@kb_d2b40_g1\endcsname{23.2$\pm$0.1}
\expandafter\def\csname tpn@kb_d2b40_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_d2b40_g1\endcsname{1.39}
\expandafter\def\csname tpnfe@kb_d2b40_g1\endcsname{50}
\expandafter\def\csname tpfid@kb_d2b40_g1\endcsname{39.8}
\expandafter\def\csname tprec@kb_d2b40_g1\endcsname{0.02}
\expandafter\def\csname tp@kb_d2b40_g2\endcsname{22.9}
\expandafter\def\csname tpsd@kb_d2b40_g2\endcsname{22.9$\pm$0.3}
\expandafter\def\csname tpn@kb_d2b40_g2\endcsname{3}
\expandafter\def\csname tpsec@kb_d2b40_g2\endcsname{1.67}
\expandafter\def\csname tpnfe@kb_d2b40_g2\endcsname{60}
\expandafter\def\csname tpfid@kb_d2b40_g2\endcsname{40.0}
\expandafter\def\csname tprec@kb_d2b40_g2\endcsname{0.02}
\expandafter\def\csname tp@kb_d2b45_g2\endcsname{22.2}
\expandafter\def\csname tpsd@kb_d2b45_g2\endcsname{22.2$\pm$0.4}
\expandafter\def\csname tpn@kb_d2b45_g2\endcsname{3}
\expandafter\def\csname tpsec@kb_d2b45_g2\endcsname{1.54}
\expandafter\def\csname tpnfe@kb_d2b45_g2\endcsname{55}
\expandafter\def\csname tpfid@kb_d2b45_g2\endcsname{39.7}
\expandafter\def\csname tprec@kb_d2b45_g2\endcsname{0.02}
\expandafter\def\csname tp@kb_dd1_g1\endcsname{28.6}
\expandafter\def\csname tpsd@kb_dd1_g1\endcsname{28.6$\pm$0.1}
\expandafter\def\csname tpn@kb_dd1_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_dd1_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@kb_dd1_g1\endcsname{4}
\expandafter\def\csname tpfid@kb_dd1_g1\endcsname{34.2}
\expandafter\def\csname tprec@kb_dd1_g1\endcsname{0.05}
\expandafter\def\csname tp@kb_dd2_g1\endcsname{39.9}
\expandafter\def\csname tpsd@kb_dd2_g1\endcsname{39.9$\pm$0.3}
\expandafter\def\csname tpn@kb_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@kb_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@kb_dd2_g1\endcsname{29.9}
\expandafter\def\csname tprec@kb_dd2_g1\endcsname{0.17}
\expandafter\def\csname tp@kb_dd2_g1_x2\endcsname{45.9}
\expandafter\def\csname tpsd@kb_dd2_g1_x2\endcsname{45.9$\pm$0.1}
\expandafter\def\csname tpn@kb_dd2_g1_x2\endcsname{3}
\expandafter\def\csname tpsec@kb_dd2_g1_x2\endcsname{0.16}
\expandafter\def\csname tpnfe@kb_dd2_g1_x2\endcsname{4}
\expandafter\def\csname tpfid@kb_dd2_g1_x2\endcsname{29.6}
\expandafter\def\csname tprec@kb_dd2_g1_x2\endcsname{0.16}
\expandafter\def\csname tp@kb_dd2_sel_dpp\endcsname{40.8}
\expandafter\def\csname tpsd@kb_dd2_sel_dpp\endcsname{40.8$\pm$0.4}
\expandafter\def\csname tpn@kb_dd2_sel_dpp\endcsname{3}
\expandafter\def\csname tpsec@kb_dd2_sel_dpp\endcsname{0.16}
\expandafter\def\csname tpnfe@kb_dd2_sel_dpp\endcsname{4}
\expandafter\def\csname tpfid@kb_dd2_sel_dpp\endcsname{29.6}
\expandafter\def\csname tprec@kb_dd2_sel_dpp\endcsname{0.16}
\expandafter\def\csname tp@kb_dd2_sel_fps\endcsname{40.4}
\expandafter\def\csname tpsd@kb_dd2_sel_fps\endcsname{40.4$\pm$1.5}
\expandafter\def\csname tpn@kb_dd2_sel_fps\endcsname{3}
\expandafter\def\csname tpsec@kb_dd2_sel_fps\endcsname{0.16}
\expandafter\def\csname tpnfe@kb_dd2_sel_fps\endcsname{4}
\expandafter\def\csname tpfid@kb_dd2_sel_fps\endcsname{29.6}
\expandafter\def\csname tprec@kb_dd2_sel_fps\endcsname{0.16}
\expandafter\def\csname tp@kb_dd2_sel_random\endcsname{40.2}
\expandafter\def\csname tpsd@kb_dd2_sel_random\endcsname{40.2$\pm$0.2}
\expandafter\def\csname tpn@kb_dd2_sel_random\endcsname{3}
\expandafter\def\csname tpsec@kb_dd2_sel_random\endcsname{0.16}
\expandafter\def\csname tpnfe@kb_dd2_sel_random\endcsname{4}
\expandafter\def\csname tpfid@kb_dd2_sel_random\endcsname{29.6}
\expandafter\def\csname tprec@kb_dd2_sel_random\endcsname{0.16}
\expandafter\def\csname tp@kb_dd3_g1\endcsname{39.6}
\expandafter\def\csname tpsd@kb_dd3_g1\endcsname{39.6$\pm$0.1}
\expandafter\def\csname tpn@kb_dd3_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_dd3_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@kb_dd3_g1\endcsname{4}
\expandafter\def\csname tpfid@kb_dd3_g1\endcsname{37.8}
\expandafter\def\csname tprec@kb_dd3_g1\endcsname{0.27}
\expandafter\def\csname tp@kb_df58_g1\endcsname{16.7}
\expandafter\def\csname tpsd@kb_df58_g1\endcsname{16.7$\pm$0.1}
\expandafter\def\csname tpn@kb_df58_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_df58_g1\endcsname{0.40}
\expandafter\def\csname tpnfe@kb_df58_g1\endcsname{13}
\expandafter\def\csname tpfid@kb_df58_g1\endcsname{46.7}
\expandafter\def\csname tprec@kb_df58_g1\endcsname{0.01}
\expandafter\def\csname tp@kb_df58_g2\endcsname{17.0}
\expandafter\def\csname tpsd@kb_df58_g2\endcsname{17.0$\pm$0.1}
\expandafter\def\csname tpn@kb_df58_g2\endcsname{3}
\expandafter\def\csname tpsec@kb_df58_g2\endcsname{0.66}
\expandafter\def\csname tpnfe@kb_df58_g2\endcsname{23}
\expandafter\def\csname tpfid@kb_df58_g2\endcsname{46.9}
\expandafter\def\csname tprec@kb_df58_g2\endcsname{0.01}
\expandafter\def\csname tp@kb_df70_g1\endcsname{17.0}
\expandafter\def\csname tpsd@kb_df70_g1\endcsname{17.0$\pm$0.4}
\expandafter\def\csname tpn@kb_df70_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_df70_g1\endcsname{0.53}
\expandafter\def\csname tpnfe@kb_df70_g1\endcsname{18}
\expandafter\def\csname tpfid@kb_df70_g1\endcsname{46.1}
\expandafter\def\csname tprec@kb_df70_g1\endcsname{0.01}
\expandafter\def\csname tp@kb_df70_g15\endcsname{17.0}
\expandafter\def\csname tpsd@kb_df70_g15\endcsname{17.0$\pm$0.2}
\expandafter\def\csname tpn@kb_df70_g15\endcsname{3}
\expandafter\def\csname tpsec@kb_df70_g15\endcsname{0.93}
\expandafter\def\csname tpnfe@kb_df70_g15\endcsname{33}
\expandafter\def\csname tpfid@kb_df70_g15\endcsname{46.3}
\expandafter\def\csname tprec@kb_df70_g15\endcsname{0.01}
\expandafter\def\csname tp@kb_df70_g2\endcsname{17.2}
\expandafter\def\csname tpsd@kb_df70_g2\endcsname{17.2$\pm$0.4}
\expandafter\def\csname tpn@kb_df70_g2\endcsname{3}
\expandafter\def\csname tpsec@kb_df70_g2\endcsname{0.93}
\expandafter\def\csname tpnfe@kb_df70_g2\endcsname{33}
\expandafter\def\csname tpfid@kb_df70_g2\endcsname{46.5}
\expandafter\def\csname tprec@kb_df70_g2\endcsname{0.01}
\expandafter\def\csname tp@kb_g1\endcsname{45.1}
\expandafter\def\csname tpsd@kb_g1\endcsname{45.1$\pm$0.0}
\expandafter\def\csname tpn@kb_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@kb_g1\endcsname{50}
\expandafter\def\csname tpfid@kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@kb_g1\endcsname{0.49}
\expandafter\def\csname tp@kb_g15\endcsname{40.8}
\expandafter\def\csname tpsd@kb_g15\endcsname{40.8$\pm$0.3}
\expandafter\def\csname tpn@kb_g15\endcsname{3}
\expandafter\def\csname tpsec@kb_g15\endcsname{2.74}
\expandafter\def\csname tpnfe@kb_g15\endcsname{100}
\expandafter\def\csname tpfid@kb_g15\endcsname{28.5}
\expandafter\def\csname tprec@kb_g15\endcsname{0.32}
\expandafter\def\csname tp@kb_g1_s10\endcsname{41.4}
\expandafter\def\csname tpsd@kb_g1_s10\endcsname{41.4$\pm$0.9}
\expandafter\def\csname tpn@kb_g1_s10\endcsname{3}
\expandafter\def\csname tpsec@kb_g1_s10\endcsname{0.30}
\expandafter\def\csname tpnfe@kb_g1_s10\endcsname{10}
\expandafter\def\csname tpfid@kb_g1_s10\endcsname{40.2}
\expandafter\def\csname tprec@kb_g1_s10\endcsname{0.33}
\expandafter\def\csname tp@kb_g1_s20\endcsname{44.7}
\expandafter\def\csname tpsd@kb_g1_s20\endcsname{44.7$\pm$0.9}
\expandafter\def\csname tpn@kb_g1_s20\endcsname{3}
\expandafter\def\csname tpsec@kb_g1_s20\endcsname{0.57}
\expandafter\def\csname tpnfe@kb_g1_s20\endcsname{20}
\expandafter\def\csname tpfid@kb_g1_s20\endcsname{34.8}
\expandafter\def\csname tprec@kb_g1_s20\endcsname{0.46}
\expandafter\def\csname tp@kb_g2_s10\endcsname{31.2}
\expandafter\def\csname tpsd@kb_g2_s10\endcsname{31.2$\pm$0.2}
\expandafter\def\csname tpn@kb_g2_s10\endcsname{3}
\expandafter\def\csname tpsec@kb_g2_s10\endcsname{0.58}
\expandafter\def\csname tpnfe@kb_g2_s10\endcsname{20}
\expandafter\def\csname tpfid@kb_g2_s10\endcsname{33.6}
\expandafter\def\csname tprec@kb_g2_s10\endcsname{0.14}
\expandafter\def\csname tp@kb_g2_s20\endcsname{34.7}
\expandafter\def\csname tpsd@kb_g2_s20\endcsname{34.7$\pm$0.4}
\expandafter\def\csname tpn@kb_g2_s20\endcsname{3}
\expandafter\def\csname tpsec@kb_g2_s20\endcsname{1.13}
\expandafter\def\csname tpnfe@kb_g2_s20\endcsname{40}
\expandafter\def\csname tpfid@kb_g2_s20\endcsname{32.4}
\expandafter\def\csname tprec@kb_g2_s20\endcsname{0.18}
\expandafter\def\csname tp@kb_g3\endcsname{27.2}
\expandafter\def\csname tpsd@kb_g3\endcsname{27.2$\pm$0.3}
\expandafter\def\csname tpn@kb_g3\endcsname{3}
\expandafter\def\csname tpsec@kb_g3\endcsname{2.74}
\expandafter\def\csname tpnfe@kb_g3\endcsname{100}
\expandafter\def\csname tpfid@kb_g3\endcsname{38.9}
\expandafter\def\csname tprec@kb_g3\endcsname{0.07}
\expandafter\def\csname tp@kb_hi10\endcsname{27.6}
\expandafter\def\csname tpsd@kb_hi10\endcsname{27.6$\pm$0.3}
\expandafter\def\csname tpn@kb_hi10\endcsname{3}
\expandafter\def\csname tpsec@kb_hi10\endcsname{1.68}
\expandafter\def\csname tpnfe@kb_hi10\endcsname{60}
\expandafter\def\csname tpfid@kb_hi10\endcsname{36.6}
\expandafter\def\csname tprec@kb_hi10\endcsname{0.11}
\expandafter\def\csname tp@kb_hi20\endcsname{25.1}
\expandafter\def\csname tpsd@kb_hi20\endcsname{25.1$\pm$0.2}
\expandafter\def\csname tpn@kb_hi20\endcsname{3}
\expandafter\def\csname tpsec@kb_hi20\endcsname{1.93}
\expandafter\def\csname tpnfe@kb_hi20\endcsname{70}
\expandafter\def\csname tpfid@kb_hi20\endcsname{40.5}
\expandafter\def\csname tprec@kb_hi20\endcsname{0.06}
\expandafter\def\csname tp@kb_interval_g4\endcsname{45.9}
\expandafter\def\csname tpsd@kb_interval_g4\endcsname{45.9$\pm$0.5}
\expandafter\def\csname tpn@kb_interval_g4\endcsname{3}
\expandafter\def\csname tpsec@kb_interval_g4\endcsname{2.02}
\expandafter\def\csname tpnfe@kb_interval_g4\endcsname{72}
\expandafter\def\csname tpfid@kb_interval_g4\endcsname{28.6}
\expandafter\def\csname tprec@kb_interval_g4\endcsname{0.46}
\expandafter\def\csname tp@kb_jump70_g2\endcsname{4.5}
\expandafter\def\csname tpsd@kb_jump70_g2\endcsname{4.5$\pm$0.1}
\expandafter\def\csname tpn@kb_jump70_g2\endcsname{3}
\expandafter\def\csname tpsec@kb_jump70_g2\endcsname{0.91}
\expandafter\def\csname tpnfe@kb_jump70_g2\endcsname{32}
\expandafter\def\csname tpfid@kb_jump70_g2\endcsname{150.7}
\expandafter\def\csname tprec@kb_jump70_g2\endcsname{0.00}
\expandafter\def\csname tp@kb_lo10\endcsname{37.2}
\expandafter\def\csname tpsd@kb_lo10\endcsname{37.2$\pm$0.4}
\expandafter\def\csname tpn@kb_lo10\endcsname{3}
\expandafter\def\csname tpsec@kb_lo10\endcsname{2.48}
\expandafter\def\csname tpnfe@kb_lo10\endcsname{90}
\expandafter\def\csname tpfid@kb_lo10\endcsname{31.0}
\expandafter\def\csname tprec@kb_lo10\endcsname{0.17}
\expandafter\def\csname tp@kb_lo20\endcsname{45.3}
\expandafter\def\csname tpsd@kb_lo20\endcsname{45.3$\pm$0.3}
\expandafter\def\csname tpn@kb_lo20\endcsname{3}
\expandafter\def\csname tpsec@kb_lo20\endcsname{2.20}
\expandafter\def\csname tpnfe@kb_lo20\endcsname{80}
\expandafter\def\csname tpfid@kb_lo20\endcsname{27.5}
\expandafter\def\csname tprec@kb_lo20\endcsname{0.38}
\expandafter\def\csname tp@kb_or10_d3\endcsname{32.8}
\expandafter\def\csname tpsd@kb_or10_d3\endcsname{32.8$\pm$0.1}
\expandafter\def\csname tpn@kb_or10_d3\endcsname{3}
\expandafter\def\csname tpsec@kb_or10_d3\endcsname{0.40}
\expandafter\def\csname tpnfe@kb_or10_d3\endcsname{13}
\expandafter\def\csname tpfid@kb_or10_d3\endcsname{31.8}
\expandafter\def\csname tprec@kb_or10_d3\endcsname{0.07}
\expandafter\def\csname tp@kb_or21_d2\endcsname{43.5}
\expandafter\def\csname tpsd@kb_or21_d2\endcsname{43.5$\pm$0.5}
\expandafter\def\csname tpn@kb_or21_d2\endcsname{3}
\expandafter\def\csname tpsec@kb_or21_d2\endcsname{0.67}
\expandafter\def\csname tpnfe@kb_or21_d2\endcsname{23}
\expandafter\def\csname tpfid@kb_or21_d2\endcsname{27.7}
\expandafter\def\csname tprec@kb_or21_d2\endcsname{0.28}
\expandafter\def\csname tp@kb_or34_d1\endcsname{46.0}
\expandafter\def\csname tpsd@kb_or34_d1\endcsname{46.0$\pm$0.4}
\expandafter\def\csname tpn@kb_or34_d1\endcsname{3}
\expandafter\def\csname tpsec@kb_or34_d1\endcsname{0.99}
\expandafter\def\csname tpnfe@kb_or34_d1\endcsname{35}
\expandafter\def\csname tpfid@kb_or34_d1\endcsname{30.2}
\expandafter\def\csname tprec@kb_or34_d1\endcsname{0.44}
\expandafter\def\csname tp@kb_or35_d1_g2\endcsname{34.2}
\expandafter\def\csname tpsd@kb_or35_d1_g2\endcsname{34.2$\pm$0.3}
\expandafter\def\csname tpn@kb_or35_d1_g2\endcsname{3}
\expandafter\def\csname tpsec@kb_or35_d1_g2\endcsname{1.97}
\expandafter\def\csname tpnfe@kb_or35_d1_g2\endcsname{71}
\expandafter\def\csname tpfid@kb_or35_d1_g2\endcsname{33.9}
\expandafter\def\csname tprec@kb_or35_d1_g2\endcsname{0.13}
\expandafter\def\csname tp@kb_or35_d1_g4\endcsname{23.6}
\expandafter\def\csname tpsd@kb_or35_d1_g4\endcsname{23.6$\pm$0.2}
\expandafter\def\csname tpn@kb_or35_d1_g4\endcsname{3}
\expandafter\def\csname tpsec@kb_or35_d1_g4\endcsname{1.96}
\expandafter\def\csname tpnfe@kb_or35_d1_g4\endcsname{71}
\expandafter\def\csname tpfid@kb_or35_d1_g4\endcsname{43.1}
\expandafter\def\csname tprec@kb_or35_d1_g4\endcsname{0.03}
\expandafter\def\csname tp@kb_or43_d1\endcsname{45.8}
\expandafter\def\csname tpsd@kb_or43_d1\endcsname{45.8$\pm$0.6}
\expandafter\def\csname tpn@kb_or43_d1\endcsname{3}
\expandafter\def\csname tpsec@kb_or43_d1\endcsname{1.23}
\expandafter\def\csname tpnfe@kb_or43_d1\endcsname{44}
\expandafter\def\csname tpfid@kb_or43_d1\endcsname{31.1}
\expandafter\def\csname tprec@kb_or43_d1\endcsname{0.49}
\expandafter\def\csname tp@kb_sw58_g1\endcsname{28.4}
\expandafter\def\csname tpsd@kb_sw58_g1\endcsname{28.4$\pm$0.5}
\expandafter\def\csname tpn@kb_sw58_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_sw58_g1\endcsname{0.40}
\expandafter\def\csname tpnfe@kb_sw58_g1\endcsname{13}
\expandafter\def\csname tpfid@kb_sw58_g1\endcsname{32.9}
\expandafter\def\csname tprec@kb_sw58_g1\endcsname{0.07}
\expandafter\def\csname tp@kb_sw70_g1\endcsname{29.9}
\expandafter\def\csname tpsd@kb_sw70_g1\endcsname{29.9$\pm$0.3}
\expandafter\def\csname tpn@kb_sw70_g1\endcsname{3}
\expandafter\def\csname tpsec@kb_sw70_g1\endcsname{0.53}
\expandafter\def\csname tpnfe@kb_sw70_g1\endcsname{18}
\expandafter\def\csname tpfid@kb_sw70_g1\endcsname{32.4}
\expandafter\def\csname tprec@kb_sw70_g1\endcsname{0.07}
\expandafter\def\csname tp@kd_ad0\endcsname{32.1}
\expandafter\def\csname tpsd@kd_ad0\endcsname{32.1$\pm$0.6}
\expandafter\def\csname tpn@kd_ad0\endcsname{3}
\expandafter\def\csname tpsec@kd_ad0\endcsname{0.15}
\expandafter\def\csname tpnfe@kd_ad0\endcsname{4}
\expandafter\def\csname tpfid@kd_ad0\endcsname{32.5}
\expandafter\def\csname tprec@kd_ad0\endcsname{0.07}
\expandafter\def\csname tp@kd_ad1\endcsname{43.9}
\expandafter\def\csname tpsd@kd_ad1\endcsname{43.9$\pm$0.9}
\expandafter\def\csname tpn@kd_ad1\endcsname{3}
\expandafter\def\csname tpsec@kd_ad1\endcsname{0.12}
\expandafter\def\csname tpnfe@kd_ad1\endcsname{3}
\expandafter\def\csname tpfid@kd_ad1\endcsname{28.7}
\expandafter\def\csname tprec@kd_ad1\endcsname{0.21}
\expandafter\def\csname tp@kd_ad1_s1\endcsname{43.2}
\expandafter\def\csname tpsd@kd_ad1_s1\endcsname{43.2$\pm$0.4}
\expandafter\def\csname tpn@kd_ad1_s1\endcsname{3}
\expandafter\def\csname tpsec@kd_ad1_s1\endcsname{0.13}
\expandafter\def\csname tpnfe@kd_ad1_s1\endcsname{3}
\expandafter\def\csname tpfid@kd_ad1_s1\endcsname{28.9}
\expandafter\def\csname tprec@kd_ad1_s1\endcsname{0.21}
\expandafter\def\csname tp@kd_ad1_s2\endcsname{43.2}
\expandafter\def\csname tpsd@kd_ad1_s2\endcsname{43.2$\pm$0.3}
\expandafter\def\csname tpn@kd_ad1_s2\endcsname{3}
\expandafter\def\csname tpsec@kd_ad1_s2\endcsname{0.13}
\expandafter\def\csname tpnfe@kd_ad1_s2\endcsname{3}
\expandafter\def\csname tpfid@kd_ad1_s2\endcsname{28.9}
\expandafter\def\csname tprec@kd_ad1_s2\endcsname{0.22}
\expandafter\def\csname tp@kd_ad1_tg4\endcsname{21.5}
\expandafter\def\csname tpsd@kd_ad1_tg4\endcsname{21.5$\pm$0.1}
\expandafter\def\csname tpn@kd_ad1_tg4\endcsname{3}
\expandafter\def\csname tpsec@kd_ad1_tg4\endcsname{0.13}
\expandafter\def\csname tpnfe@kd_ad1_tg4\endcsname{3}
\expandafter\def\csname tpfid@kd_ad1_tg4\endcsname{44.6}
\expandafter\def\csname tprec@kd_ad1_tg4\endcsname{0.02}
\expandafter\def\csname tp@kd_ad1x\endcsname{43.0}
\expandafter\def\csname tpsd@kd_ad1x\endcsname{43.0$\pm$0.6}
\expandafter\def\csname tpn@kd_ad1x\endcsname{3}
\expandafter\def\csname tpsec@kd_ad1x\endcsname{0.13}
\expandafter\def\csname tpnfe@kd_ad1x\endcsname{3}
\expandafter\def\csname tpfid@kd_ad1x\endcsname{28.7}
\expandafter\def\csname tprec@kd_ad1x\endcsname{0.21}
\expandafter\def\csname tp@kd_ad2\endcsname{44.1}
\expandafter\def\csname tpsd@kd_ad2\endcsname{44.1$\pm$0.5}
\expandafter\def\csname tpn@kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2\endcsname{34.8}
\expandafter\def\csname tprec@kd_ad2\endcsname{0.28}
\expandafter\def\csname tp@kd_ad2_all\endcsname{41.4}
\expandafter\def\csname tpsd@kd_ad2_all\endcsname{41.4$\pm$0.3}
\expandafter\def\csname tpn@kd_ad2_all\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2_all\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2_all\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2_all\endcsname{45.0}
\expandafter\def\csname tprec@kd_ad2_all\endcsname{0.12}
\expandafter\def\csname tp@kd_ad2_full_lr1e5\endcsname{42.7}
\expandafter\def\csname tpsd@kd_ad2_full_lr1e5\endcsname{42.7$\pm$0.5}
\expandafter\def\csname tpn@kd_ad2_full_lr1e5\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2_full_lr1e5\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2_full_lr1e5\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2_full_lr1e5\endcsname{36.5}
\expandafter\def\csname tprec@kd_ad2_full_lr1e5\endcsname{0.25}
\expandafter\def\csname tp@kd_ad2_full_lr3e6\endcsname{43.2}
\expandafter\def\csname tpsd@kd_ad2_full_lr3e6\endcsname{43.2$\pm$1.0}
\expandafter\def\csname tpn@kd_ad2_full_lr3e6\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2_full_lr3e6\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2_full_lr3e6\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2_full_lr3e6\endcsname{34.8}
\expandafter\def\csname tprec@kd_ad2_full_lr3e6\endcsname{0.28}
\expandafter\def\csname tp@kd_ad2_ns1\endcsname{44.4}
\expandafter\def\csname tpsd@kd_ad2_ns1\endcsname{44.4$\pm$0.5}
\expandafter\def\csname tpn@kd_ad2_ns1\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2_ns1\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2_ns1\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2_ns1\endcsname{34.7}
\expandafter\def\csname tprec@kd_ad2_ns1\endcsname{0.28}
\expandafter\def\csname tp@kd_ad2_r128\endcsname{44.1}
\expandafter\def\csname tpsd@kd_ad2_r128\endcsname{44.1$\pm$0.4}
\expandafter\def\csname tpn@kd_ad2_r128\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2_r128\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2_r128\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2_r128\endcsname{34.9}
\expandafter\def\csname tprec@kd_ad2_r128\endcsname{0.28}
\expandafter\def\csname tp@kd_ad2_r8\endcsname{43.4}
\expandafter\def\csname tpsd@kd_ad2_r8\endcsname{43.4$\pm$0.3}
\expandafter\def\csname tpn@kd_ad2_r8\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2_r8\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2_r8\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2_r8\endcsname{34.9}
\expandafter\def\csname tprec@kd_ad2_r8\endcsname{0.26}
\expandafter\def\csname tp@kd_ad2_s2\endcsname{43.6}
\expandafter\def\csname tpsd@kd_ad2_s2\endcsname{43.6$\pm$0.1}
\expandafter\def\csname tpn@kd_ad2_s2\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2_s2\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2_s2\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2_s2\endcsname{34.8}
\expandafter\def\csname tprec@kd_ad2_s2\endcsname{0.27}
\expandafter\def\csname tp@kd_ad2_tg2\endcsname{31.5}
\expandafter\def\csname tpsd@kd_ad2_tg2\endcsname{31.5$\pm$0.7}
\expandafter\def\csname tpn@kd_ad2_tg2\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2_tg2\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2_tg2\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2_tg2\endcsname{35.3}
\expandafter\def\csname tprec@kd_ad2_tg2\endcsname{0.07}
\expandafter\def\csname tp@kd_ad2_tg4\endcsname{20.1}
\expandafter\def\csname tpsd@kd_ad2_tg4\endcsname{20.1$\pm$0.4}
\expandafter\def\csname tpn@kd_ad2_tg4\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2_tg4\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2_tg4\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2_tg4\endcsname{44.5}
\expandafter\def\csname tprec@kd_ad2_tg4\endcsname{0.01}
\expandafter\def\csname tp@kd_ad2_x3\endcsname{43.8}
\expandafter\def\csname tpsd@kd_ad2_x3\endcsname{43.8$\pm$0.4}
\expandafter\def\csname tpn@kd_ad2_x3\endcsname{9}
\expandafter\def\csname tpsec@kd_ad2_x3\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2_x3\endcsname{2}
\expandafter\def\csname tp@kd_ad2b\endcsname{43.8}
\expandafter\def\csname tpsd@kd_ad2b\endcsname{43.8$\pm$0.5}
\expandafter\def\csname tpn@kd_ad2b\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2b\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2b\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2b\endcsname{34.8}
\expandafter\def\csname tprec@kd_ad2b\endcsname{0.27}
\expandafter\def\csname tp@kd_ad2x\endcsname{43.2}
\expandafter\def\csname tpsd@kd_ad2x\endcsname{43.2$\pm$0.7}
\expandafter\def\csname tpn@kd_ad2x\endcsname{3}
\expandafter\def\csname tpsec@kd_ad2x\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad2x\endcsname{2}
\expandafter\def\csname tpfid@kd_ad2x\endcsname{34.5}
\expandafter\def\csname tprec@kd_ad2x\endcsname{0.27}
\expandafter\def\csname tp@kd_ad3\endcsname{40.0}
\expandafter\def\csname tpsd@kd_ad3\endcsname{40.0$\pm$0.5}
\expandafter\def\csname tpn@kd_ad3\endcsname{3}
\expandafter\def\csname tpsec@kd_ad3\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_ad3\endcsname{2}
\expandafter\def\csname tpfid@kd_ad3\endcsname{41.9}
\expandafter\def\csname tprec@kd_ad3\endcsname{0.18}
\expandafter\def\csname tp@kd_cads_s01\endcsname{18.3}
\expandafter\def\csname tpsd@kd_cads_s01\endcsname{18.3$\pm$0.7}
\expandafter\def\csname tpn@kd_cads_s01\endcsname{3}
\expandafter\def\csname tpsec@kd_cads_s01\endcsname{0.15}
\expandafter\def\csname tpnfe@kd_cads_s01\endcsname{4}
\expandafter\def\csname tpfid@kd_cads_s01\endcsname{166.5}
\expandafter\def\csname tprec@kd_cads_s01\endcsname{0.08}
\expandafter\def\csname tp@kd_cads_s025\endcsname{17.7}
\expandafter\def\csname tpsd@kd_cads_s025\endcsname{17.7$\pm$0.3}
\expandafter\def\csname tpn@kd_cads_s025\endcsname{3}
\expandafter\def\csname tpsec@kd_cads_s025\endcsname{0.15}
\expandafter\def\csname tpnfe@kd_cads_s025\endcsname{4}
\expandafter\def\csname tpfid@kd_cads_s025\endcsname{169.0}
\expandafter\def\csname tprec@kd_cads_s025\endcsname{0.08}
\expandafter\def\csname tp@kd_coco\endcsname{45.0}
\expandafter\def\csname tpsd@kd_coco\endcsname{45.0$\pm$0.5}
\expandafter\def\csname tpn@kd_coco\endcsname{3}
\expandafter\def\csname tpsec@kd_coco\endcsname{0.10}
\expandafter\def\csname tpnfe@kd_coco\endcsname{2}
\expandafter\def\csname tpfid@kd_coco\endcsname{34.9}
\expandafter\def\csname tprec@kd_coco\endcsname{0.23}
\expandafter\def\csname tp@kd_fsg\endcsname{20.7}
\expandafter\def\csname tpsd@kd_fsg\endcsname{20.7$\pm$0.7}
\expandafter\def\csname tpn@kd_fsg\endcsname{3}
\expandafter\def\csname tpsec@kd_fsg\endcsname{0.16}
\expandafter\def\csname tpnfe@kd_fsg\endcsname{4}
\expandafter\def\csname tpfid@kd_fsg\endcsname{41.7}
\expandafter\def\csname tprec@kd_fsg\endcsname{0.02}
\expandafter\def\csname tp@kd_mono1\endcsname{24.5}
\expandafter\def\csname tpsd@kd_mono1\endcsname{24.5$\pm$0.7}
\expandafter\def\csname tpn@kd_mono1\endcsname{3}
\expandafter\def\csname tpsec@kd_mono1\endcsname{0.25}
\expandafter\def\csname tpnfe@kd_mono1\endcsname{4.74}
\expandafter\def\csname tpfid@kd_mono1\endcsname{36.9}
\expandafter\def\csname tprec@kd_mono1\endcsname{0.03}
\expandafter\def\csname tp@kd_mono4\endcsname{26.8}
\expandafter\def\csname tpsd@kd_mono4\endcsname{26.8$\pm$0.3}
\expandafter\def\csname tpn@kd_mono4\endcsname{3}
\expandafter\def\csname tpsec@kd_mono4\endcsname{0.52}
\expandafter\def\csname tpnfe@kd_mono4\endcsname{6.98}
\expandafter\def\csname tpfid@kd_mono4\endcsname{31.5}
\expandafter\def\csname tprec@kd_mono4\endcsname{0.08}
\expandafter\def\csname tp@kd_mono4_g32\endcsname{29.9}
\expandafter\def\csname tpsd@kd_mono4_g32\endcsname{29.9$\pm$0.3}
\expandafter\def\csname tpn@kd_mono4_g32\endcsname{3}
\expandafter\def\csname tpsec@kd_mono4_g32\endcsname{0.63}
\expandafter\def\csname tpnfe@kd_mono4_g32\endcsname{7.87}
\expandafter\def\csname tpfid@kd_mono4_g32\endcsname{30.5}
\expandafter\def\csname tprec@kd_mono4_g32\endcsname{0.12}
\expandafter\def\csname tp@kd_mono4_rand\endcsname{16.8}
\expandafter\def\csname tpsd@kd_mono4_rand\endcsname{16.8$\pm$0.1}
\expandafter\def\csname tpn@kd_mono4_rand\endcsname{3}
\expandafter\def\csname tpsec@kd_mono4_rand\endcsname{0.15}
\expandafter\def\csname tpnfe@kd_mono4_rand\endcsname{4}
\expandafter\def\csname tpfid@kd_mono4_rand\endcsname{47.5}
\expandafter\def\csname tprec@kd_mono4_rand\endcsname{0.01}
\expandafter\def\csname tp@kd_rep05\endcsname{18.0}
\expandafter\def\csname tpsd@kd_rep05\endcsname{18.0$\pm$0.2}
\expandafter\def\csname tpn@kd_rep05\endcsname{3}
\expandafter\def\csname tpsec@kd_rep05\endcsname{0.15}
\expandafter\def\csname tpnfe@kd_rep05\endcsname{4}
\expandafter\def\csname tpfid@kd_rep05\endcsname{46.3}
\expandafter\def\csname tprec@kd_rep05\endcsname{0.01}
\expandafter\def\csname tp@kd_rep1\endcsname{19.4}
\expandafter\def\csname tpsd@kd_rep1\endcsname{19.4$\pm$0.5}
\expandafter\def\csname tpn@kd_rep1\endcsname{3}
\expandafter\def\csname tpsec@kd_rep1\endcsname{0.15}
\expandafter\def\csname tpnfe@kd_rep1\endcsname{4}
\expandafter\def\csname tpfid@kd_rep1\endcsname{45.1}
\expandafter\def\csname tprec@kd_rep1\endcsname{0.01}
\expandafter\def\csname tp@kd_rep1_01\endcsname{21.6}
\expandafter\def\csname tpsd@kd_rep1_01\endcsname{21.6$\pm$0.3}
\expandafter\def\csname tpn@kd_rep1_01\endcsname{3}
\expandafter\def\csname tpsec@kd_rep1_01\endcsname{0.15}
\expandafter\def\csname tpnfe@kd_rep1_01\endcsname{4}
\expandafter\def\csname tpfid@kd_rep1_01\endcsname{42.3}
\expandafter\def\csname tprec@kd_rep1_01\endcsname{0.02}
\expandafter\def\csname tp@kd_rep2\endcsname{20.9}
\expandafter\def\csname tpsd@kd_rep2\endcsname{20.9$\pm$0.4}
\expandafter\def\csname tpn@kd_rep2\endcsname{3}
\expandafter\def\csname tpsec@kd_rep2\endcsname{0.15}
\expandafter\def\csname tpnfe@kd_rep2\endcsname{4}
\expandafter\def\csname tpfid@kd_rep2\endcsname{42.7}
\expandafter\def\csname tprec@kd_rep2\endcsname{0.02}
\expandafter\def\csname tp@kd_rep2_01\endcsname{24.8}
\expandafter\def\csname tpsd@kd_rep2_01\endcsname{24.8$\pm$0.2}
\expandafter\def\csname tpn@kd_rep2_01\endcsname{3}
\expandafter\def\csname tpsec@kd_rep2_01\endcsname{0.15}
\expandafter\def\csname tpnfe@kd_rep2_01\endcsname{4}
\expandafter\def\csname tpfid@kd_rep2_01\endcsname{37.1}
\expandafter\def\csname tprec@kd_rep2_01\endcsname{0.03}
\expandafter\def\csname tp@kd_rep4_01\endcsname{24.2}
\expandafter\def\csname tpsd@kd_rep4_01\endcsname{24.2$\pm$0.3}
\expandafter\def\csname tpn@kd_rep4_01\endcsname{3}
\expandafter\def\csname tpsec@kd_rep4_01\endcsname{0.15}
\expandafter\def\csname tpnfe@kd_rep4_01\endcsname{4}
\expandafter\def\csname tpfid@kd_rep4_01\endcsname{39.7}
\expandafter\def\csname tprec@kd_rep4_01\endcsname{0.05}
\expandafter\def\csname tp@kd_self70\endcsname{14.7}
\expandafter\def\csname tpsd@kd_self70\endcsname{14.7$\pm$0.1}
\expandafter\def\csname tpn@kd_self70\endcsname{3}
\expandafter\def\csname tpsec@kd_self70\endcsname{0.53}
\expandafter\def\csname tpnfe@kd_self70\endcsname{18}
\expandafter\def\csname tpfid@kd_self70\endcsname{46.0}
\expandafter\def\csname tprec@kd_self70\endcsname{0.01}
\expandafter\def\csname tp@kd_sft\endcsname{31.8}
\expandafter\def\csname tpsd@kd_sft\endcsname{31.8$\pm$0.3}
\expandafter\def\csname tpn@kd_sft\endcsname{3}
\expandafter\def\csname tpsec@kd_sft\endcsname{0.11}
\expandafter\def\csname tpnfe@kd_sft\endcsname{3}
\expandafter\def\csname tpfid@kd_sft\endcsname{30.2}
\expandafter\def\csname tprec@kd_sft\endcsname{0.09}
\expandafter\def\csname tp@kd_skip3\endcsname{12.8}
\expandafter\def\csname tpsd@kd_skip3\endcsname{12.8$\pm$0.2}
\expandafter\def\csname tpn@kd_skip3\endcsname{3}
\expandafter\def\csname tpsec@kd_skip3\endcsname{0.11}
\expandafter\def\csname tpnfe@kd_skip3\endcsname{3}
\expandafter\def\csname tpfid@kd_skip3\endcsname{51.3}
\expandafter\def\csname tprec@kd_skip3\endcsname{0.00}
\expandafter\def\csname tp@kd_skip51\endcsname{7.0}
\expandafter\def\csname tpsd@kd_skip51\endcsname{7.0$\pm$0.1}
\expandafter\def\csname tpn@kd_skip51\endcsname{3}
\expandafter\def\csname tpsec@kd_skip51\endcsname{0.09}
\expandafter\def\csname tpnfe@kd_skip51\endcsname{2}
\expandafter\def\csname tpfid@kd_skip51\endcsname{60.3}
\expandafter\def\csname tprec@kd_skip51\endcsname{0.00}
\expandafter\def\csname tp@klein\endcsname{17.1}
\expandafter\def\csname tpsd@klein\endcsname{17.1$\pm$0.4}
\expandafter\def\csname tpn@klein\endcsname{3}
\expandafter\def\csname tpsec@klein\endcsname{0.14}
\expandafter\def\csname tpnfe@klein\endcsname{4}
\expandafter\def\csname tpfid@klein\endcsname{47.6}
\expandafter\def\csname tprec@klein\endcsname{0.01}
\expandafter\def\csname tp@klein_all50\endcsname{21.2}
\expandafter\def\csname tpsd@klein_all50\endcsname{21.2$\pm$0.2}
\expandafter\def\csname tpn@klein_all50\endcsname{3}
\expandafter\def\csname tpfid@klein_all50\endcsname{39.5}
\expandafter\def\csname tprec@klein_all50\endcsname{0.02}
\expandafter\def\csname tp@klein_b2d10\endcsname{21.1}
\expandafter\def\csname tpsd@klein_b2d10\endcsname{21.1$\pm$0.2}
\expandafter\def\csname tpn@klein_b2d10\endcsname{3}
\expandafter\def\csname tpfid@klein_b2d10\endcsname{38.8}
\expandafter\def\csname tprec@klein_b2d10\endcsname{0.03}
\expandafter\def\csname tp@klein_b2d25\endcsname{23.2}
\expandafter\def\csname tpsd@klein_b2d25\endcsname{23.2$\pm$0.7}
\expandafter\def\csname tpn@klein_b2d25\endcsname{3}
\expandafter\def\csname tpfid@klein_b2d25\endcsname{40.6}
\expandafter\def\csname tprec@klein_b2d25\endcsname{0.03}
\expandafter\def\csname tp@klein_b2d5\endcsname{22.1}
\expandafter\def\csname tpsd@klein_b2d5\endcsname{22.1$\pm$0.2}
\expandafter\def\csname tpn@klein_b2d5\endcsname{3}
\expandafter\def\csname tpfid@klein_b2d5\endcsname{38.0}
\expandafter\def\csname tprec@klein_b2d5\endcsname{0.02}
\expandafter\def\csname tp@klein_base\endcsname{23.6}
\expandafter\def\csname tpsd@klein_base\endcsname{23.6$\pm$0.5}
\expandafter\def\csname tpn@klein_base\endcsname{3}
\expandafter\def\csname tpsec@klein_base\endcsname{2.82}
\expandafter\def\csname tpnfe@klein_base\endcsname{100}
\expandafter\def\csname tpfid@klein_base\endcsname{42.6}
\expandafter\def\csname tprec@klein_base\endcsname{0.04}
\expandafter\def\csname tp@klein_base_g2\endcsname{34.8}
\expandafter\def\csname tpsd@klein_base_g2\endcsname{34.8$\pm$0.7}
\expandafter\def\csname tpn@klein_base_g2\endcsname{3}
\expandafter\def\csname tpsec@klein_base_g2\endcsname{2.82}
\expandafter\def\csname tpnfe@klein_base_g2\endcsname{100}
\expandafter\def\csname tpfid@klein_base_g2\endcsname{32.5}
\expandafter\def\csname tprec@klein_base_g2\endcsname{0.18}
\expandafter\def\csname tp@klein_d2b10\endcsname{24.2}
\expandafter\def\csname tpsd@klein_d2b10\endcsname{24.2$\pm$0.3}
\expandafter\def\csname tpn@klein_d2b10\endcsname{3}
\expandafter\def\csname tpfid@klein_d2b10\endcsname{44.1}
\expandafter\def\csname tprec@klein_d2b10\endcsname{0.02}
\expandafter\def\csname tp@klein_d2b25\endcsname{24.4}
\expandafter\def\csname tpsd@klein_d2b25\endcsname{24.4$\pm$0.4}
\expandafter\def\csname tpn@klein_d2b25\endcsname{3}
\expandafter\def\csname tpfid@klein_d2b25\endcsname{41.6}
\expandafter\def\csname tprec@klein_d2b25\endcsname{0.02}
\expandafter\def\csname tp@klein_d2b5\endcsname{22.4}
\expandafter\def\csname tpsd@klein_d2b5\endcsname{22.4$\pm$0.6}
\expandafter\def\csname tpn@klein_d2b5\endcsname{3}
\expandafter\def\csname tpfid@klein_d2b5\endcsname{44.9}
\expandafter\def\csname tprec@klein_d2b5\endcsname{0.02}
\expandafter\def\csname tp@klein_ns1\endcsname{17.2}
\expandafter\def\csname tpsd@klein_ns1\endcsname{17.2$\pm$0.4}
\expandafter\def\csname tpn@klein_ns1\endcsname{3}
\expandafter\def\csname tpsec@klein_ns1\endcsname{0.14}
\expandafter\def\csname tpnfe@klein_ns1\endcsname{4}
\expandafter\def\csname tpfid@klein_ns1\endcsname{47.8}
\expandafter\def\csname tprec@klein_ns1\endcsname{0.01}
\expandafter\def\csname tp@llm_kb_dd2_g1\endcsname{43.1}
\expandafter\def\csname tpsd@llm_kb_dd2_g1\endcsname{43.1$\pm$0.6}
\expandafter\def\csname tpn@llm_kb_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@llm_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@llm_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@llm_kb_dd2_g1\endcsname{46.1}
\expandafter\def\csname tprec@llm_kb_dd2_g1\endcsname{0.23}
\expandafter\def\csname tp@llm_kb_g1\endcsname{42.9}
\expandafter\def\csname tpsd@llm_kb_g1\endcsname{42.9$\pm$0.7}
\expandafter\def\csname tpn@llm_kb_g1\endcsname{3}
\expandafter\def\csname tpsec@llm_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@llm_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@llm_kb_g1\endcsname{57.9}
\expandafter\def\csname tprec@llm_kb_g1\endcsname{0.51}
\expandafter\def\csname tp@llm_kd_ad2\endcsname{39.6}
\expandafter\def\csname tpsd@llm_kd_ad2\endcsname{39.6$\pm$0.3}
\expandafter\def\csname tpn@llm_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@llm_kd_ad2\endcsname{0.11}
\expandafter\def\csname tpnfe@llm_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@llm_kd_ad2\endcsname{61.6}
\expandafter\def\csname tprec@llm_kd_ad2\endcsname{0.35}
\expandafter\def\csname tp@llm_klein\endcsname{37.9}
\expandafter\def\csname tpsd@llm_klein\endcsname{37.9$\pm$0.2}
\expandafter\def\csname tpn@llm_klein\endcsname{3}
\expandafter\def\csname tpsec@llm_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@llm_klein\endcsname{4}
\expandafter\def\csname tpfid@llm_klein\endcsname{37.8}
\expandafter\def\csname tprec@llm_klein\endcsname{0.13}
\expandafter\def\csname tp@llm_sd15_g2\endcsname{50.2}
\expandafter\def\csname tpsd@llm_sd15_g2\endcsname{50.2$\pm$0.4}
\expandafter\def\csname tpn@llm_sd15_g2\endcsname{3}
\expandafter\def\csname tpsec@llm_sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@llm_sd15_g2\endcsname{60}
\expandafter\def\csname tpfid@llm_sd15_g2\endcsname{38.0}
\expandafter\def\csname tprec@llm_sd15_g2\endcsname{0.33}
\expandafter\def\csname tp@llm_sd21_g2\endcsname{50.3}
\expandafter\def\csname tpsd@llm_sd21_g2\endcsname{50.3$\pm$0.1}
\expandafter\def\csname tpn@llm_sd21_g2\endcsname{3}
\expandafter\def\csname tpsec@llm_sd21_g2\endcsname{0.20}
\expandafter\def\csname tpnfe@llm_sd21_g2\endcsname{60}
\expandafter\def\csname tpfid@llm_sd21_g2\endcsname{37.2}
\expandafter\def\csname tprec@llm_sd21_g2\endcsname{0.29}
\expandafter\def\csname tp@llm_sd_turbo\endcsname{31.4}
\expandafter\def\csname tpsd@llm_sd_turbo\endcsname{31.4$\pm$0.5}
\expandafter\def\csname tpn@llm_sd_turbo\endcsname{3}
\expandafter\def\csname tpsec@llm_sd_turbo\endcsname{0.02}
\expandafter\def\csname tpnfe@llm_sd_turbo\endcsname{1}
\expandafter\def\csname tpfid@llm_sd_turbo\endcsname{28.7}
\expandafter\def\csname tprec@llm_sd_turbo\endcsname{0.05}
\expandafter\def\csname tp@llm_sdt4\endcsname{29.6}
\expandafter\def\csname tpsd@llm_sdt4\endcsname{29.6$\pm$0.7}
\expandafter\def\csname tpn@llm_sdt4\endcsname{3}
\expandafter\def\csname tpsec@llm_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@llm_sdt4\endcsname{4}
\expandafter\def\csname tpfid@llm_sdt4\endcsname{41.1}
\expandafter\def\csname tprec@llm_sdt4\endcsname{0.07}
\expandafter\def\csname tp@llm_sdt4_dd2_g1\endcsname{37.6}
\expandafter\def\csname tpsd@llm_sdt4_dd2_g1\endcsname{37.6$\pm$0.6}
\expandafter\def\csname tpn@llm_sdt4_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@llm_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@llm_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@llm_sdt4_dd2_g1\endcsname{44.3}
\expandafter\def\csname tprec@llm_sdt4_dd2_g1\endcsname{0.18}
\expandafter\def\csname tp@llm_sdt_ad1\endcsname{45.8}
\expandafter\def\csname tpsd@llm_sdt_ad1\endcsname{45.8$\pm$0.5}
\expandafter\def\csname tpn@llm_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@llm_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@llm_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@llm_sdt_ad1\endcsname{40.3}
\expandafter\def\csname tprec@llm_sdt_ad1\endcsname{0.25}
\expandafter\def\csname tp@low_kb_g1\endcsname{58.3}
\expandafter\def\csname tpsd@low_kb_g1\endcsname{58.3$\pm$0.7}
\expandafter\def\csname tpn@low_kb_g1\endcsname{3}
\expandafter\def\csname tpsec@low_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@low_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@low_kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@low_kb_g1\endcsname{0.49}
\expandafter\def\csname tp@low_kd_ad2\endcsname{60.2}
\expandafter\def\csname tpsd@low_kd_ad2\endcsname{60.2$\pm$0.3}
\expandafter\def\csname tpn@low_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@low_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@low_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@low_kd_ad2\endcsname{34.8}
\expandafter\def\csname tprec@low_kd_ad2\endcsname{0.28}
\expandafter\def\csname tp@low_klein\endcsname{48.1}
\expandafter\def\csname tpsd@low_klein\endcsname{48.1$\pm$0.4}
\expandafter\def\csname tpn@low_klein\endcsname{3}
\expandafter\def\csname tpsec@low_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@low_klein\endcsname{4}
\expandafter\def\csname tpfid@low_klein\endcsname{47.6}
\expandafter\def\csname tprec@low_klein\endcsname{0.01}
\expandafter\def\csname tp@low_real50\endcsname{34.0}
\expandafter\def\csname tpsd@low_real50\endcsname{34.0$\pm$0.7}
\expandafter\def\csname tpn@low_real50\endcsname{3}
\expandafter\def\csname tp@low_sd21_g1\endcsname{61.8}
\expandafter\def\csname tpsd@low_sd21_g1\endcsname{61.8$\pm$0.5}
\expandafter\def\csname tpn@low_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@low_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@low_sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@low_sd21_g1\endcsname{50.2}
\expandafter\def\csname tprec@low_sd21_g1\endcsname{0.33}
\expandafter\def\csname tp@low_sdt4\endcsname{51.6}
\expandafter\def\csname tpsd@low_sdt4\endcsname{51.6$\pm$0.5}
\expandafter\def\csname tpn@low_sdt4\endcsname{3}
\expandafter\def\csname tpsec@low_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@low_sdt4\endcsname{4}
\expandafter\def\csname tpfid@low_sdt4\endcsname{37.5}
\expandafter\def\csname tprec@low_sdt4\endcsname{0.02}
\expandafter\def\csname tp@low_sdt_ad1\endcsname{64.8}
\expandafter\def\csname tpsd@low_sdt_ad1\endcsname{64.8$\pm$0.1}
\expandafter\def\csname tpn@low_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@low_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@low_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@low_sdt_ad1\endcsname{30.2}
\expandafter\def\csname tprec@low_sdt_ad1\endcsname{0.16}
\expandafter\def\csname tp@lp_flux_dev\endcsname{14.6}
\expandafter\def\csname tpsd@lp_flux_dev\endcsname{14.6$\pm$0.6}
\expandafter\def\csname tpn@lp_flux_dev\endcsname{2}
\expandafter\def\csname tpsec@lp_flux_dev\endcsname{1.69}
\expandafter\def\csname tpnfe@lp_flux_dev\endcsname{28}
\expandafter\def\csname tpfid@lp_flux_dev\endcsname{46.0}
\expandafter\def\csname tprec@lp_flux_dev\endcsname{0.03}
\expandafter\def\csname tp@lp_flux_dev_g1\endcsname{30.1}
\expandafter\def\csname tpsd@lp_flux_dev_g1\endcsname{30.1$\pm$0.1}
\expandafter\def\csname tpn@lp_flux_dev_g1\endcsname{2}
\expandafter\def\csname tpsec@lp_flux_dev_g1\endcsname{1.67}
\expandafter\def\csname tpnfe@lp_flux_dev_g1\endcsname{28}
\expandafter\def\csname tpfid@lp_flux_dev_g1\endcsname{32.7}
\expandafter\def\csname tprec@lp_flux_dev_g1\endcsname{0.17}
\expandafter\def\csname tp@lp_kb_dd2_g1\endcsname{33.7}
\expandafter\def\csname tpsd@lp_kb_dd2_g1\endcsname{33.7$\pm$0.7}
\expandafter\def\csname tpn@lp_kb_dd2_g1\endcsname{2}
\expandafter\def\csname tpsec@lp_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@lp_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@lp_kb_dd2_g1\endcsname{29.9}
\expandafter\def\csname tprec@lp_kb_dd2_g1\endcsname{0.17}
\expandafter\def\csname tp@lp_kb_g1\endcsname{37.8}
\expandafter\def\csname tpsd@lp_kb_g1\endcsname{37.8$\pm$0.2}
\expandafter\def\csname tpn@lp_kb_g1\endcsname{2}
\expandafter\def\csname tpsec@lp_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@lp_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@lp_kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@lp_kb_g1\endcsname{0.49}
\expandafter\def\csname tp@lp_kd_ad2\endcsname{36.6}
\expandafter\def\csname tpsd@lp_kd_ad2\endcsname{36.6$\pm$1.3}
\expandafter\def\csname tpn@lp_kd_ad2\endcsname{2}
\expandafter\def\csname tpsec@lp_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@lp_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@lp_kd_ad2\endcsname{34.8}
\expandafter\def\csname tprec@lp_kd_ad2\endcsname{0.28}
\expandafter\def\csname tp@lp_klein\endcsname{16.3}
\expandafter\def\csname tpsd@lp_klein\endcsname{16.3$\pm$0.1}
\expandafter\def\csname tpn@lp_klein\endcsname{2}
\expandafter\def\csname tpsec@lp_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@lp_klein\endcsname{4}
\expandafter\def\csname tpfid@lp_klein\endcsname{47.6}
\expandafter\def\csname tprec@lp_klein\endcsname{0.01}
\expandafter\def\csname tp@lp_klein_base\endcsname{22.8}
\expandafter\def\csname tpsd@lp_klein_base\endcsname{22.8$\pm$0.3}
\expandafter\def\csname tpn@lp_klein_base\endcsname{2}
\expandafter\def\csname tpsec@lp_klein_base\endcsname{2.82}
\expandafter\def\csname tpnfe@lp_klein_base\endcsname{100}
\expandafter\def\csname tpfid@lp_klein_base\endcsname{42.6}
\expandafter\def\csname tprec@lp_klein_base\endcsname{0.04}
\expandafter\def\csname tp@lp_real500\endcsname{70.2}
\expandafter\def\csname tpsd@lp_real500\endcsname{70.2$\pm$0.3}
\expandafter\def\csname tpn@lp_real500\endcsname{2}
\expandafter\def\csname tp@lp_sd15\endcsname{30.7}
\expandafter\def\csname tpsd@lp_sd15\endcsname{30.7$\pm$0.4}
\expandafter\def\csname tpn@lp_sd15\endcsname{2}
\expandafter\def\csname tpsec@lp_sd15\endcsname{0.21}
\expandafter\def\csname tpnfe@lp_sd15\endcsname{60}
\expandafter\def\csname tpfid@lp_sd15\endcsname{26.6}
\expandafter\def\csname tprec@lp_sd15\endcsname{0.06}
\expandafter\def\csname tp@lp_sd15_g2\endcsname{43.9}
\expandafter\def\csname tpsd@lp_sd15_g2\endcsname{43.9$\pm$0.2}
\expandafter\def\csname tpn@lp_sd15_g2\endcsname{2}
\expandafter\def\csname tpsec@lp_sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@lp_sd15_g2\endcsname{60}
\expandafter\def\csname tpfid@lp_sd15_g2\endcsname{25.3}
\expandafter\def\csname tprec@lp_sd15_g2\endcsname{0.31}
\expandafter\def\csname tp@lp_sd21\endcsname{28.7}
\expandafter\def\csname tpsd@lp_sd21\endcsname{28.7$\pm$1.0}
\expandafter\def\csname tpn@lp_sd21\endcsname{2}
\expandafter\def\csname tpsec@lp_sd21\endcsname{0.20}
\expandafter\def\csname tpnfe@lp_sd21\endcsname{60}
\expandafter\def\csname tpfid@lp_sd21\endcsname{28.0}
\expandafter\def\csname tprec@lp_sd21\endcsname{0.04}
\expandafter\def\csname tp@lp_sd21_g1\endcsname{39.7}
\expandafter\def\csname tpsd@lp_sd21_g1\endcsname{39.7$\pm$0.2}
\expandafter\def\csname tpn@lp_sd21_g1\endcsname{2}
\expandafter\def\csname tpsec@lp_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@lp_sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@lp_sd21_g1\endcsname{50.2}
\expandafter\def\csname tprec@lp_sd21_g1\endcsname{0.33}
\expandafter\def\csname tp@lp_sdt4\endcsname{19.9}
\expandafter\def\csname tpsd@lp_sdt4\endcsname{19.9$\pm$0.2}
\expandafter\def\csname tpn@lp_sdt4\endcsname{2}
\expandafter\def\csname tpsec@lp_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@lp_sdt4\endcsname{4}
\expandafter\def\csname tpfid@lp_sdt4\endcsname{37.5}
\expandafter\def\csname tprec@lp_sdt4\endcsname{0.02}
\expandafter\def\csname tp@lp_sdt4_dd2_g1\endcsname{34.9}
\expandafter\def\csname tpsd@lp_sdt4_dd2_g1\endcsname{34.9$\pm$0.4}
\expandafter\def\csname tpn@lp_sdt4_dd2_g1\endcsname{2}
\expandafter\def\csname tpsec@lp_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@lp_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@lp_sdt4_dd2_g1\endcsname{32.1}
\expandafter\def\csname tprec@lp_sdt4_dd2_g1\endcsname{0.12}
\expandafter\def\csname tp@lp_sdt_ad1\endcsname{37.6}
\expandafter\def\csname tpsd@lp_sdt_ad1\endcsname{37.6$\pm$0.5}
\expandafter\def\csname tpn@lp_sdt_ad1\endcsname{2}
\expandafter\def\csname tpsec@lp_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@lp_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@lp_sdt_ad1\endcsname{30.2}
\expandafter\def\csname tprec@lp_sdt_ad1\endcsname{0.16}
\expandafter\def\csname tp@lp_zimage\endcsname{19.0}
\expandafter\def\csname tpsd@lp_zimage\endcsname{19.0$\pm$0.4}
\expandafter\def\csname tpn@lp_zimage\endcsname{2}
\expandafter\def\csname tpsec@lp_zimage\endcsname{3.78}
\expandafter\def\csname tpnfe@lp_zimage\endcsname{100}
\expandafter\def\csname tpfid@lp_zimage\endcsname{34.6}
\expandafter\def\csname tprec@lp_zimage\endcsname{0.03}
\expandafter\def\csname tp@lp_zimage_g1\endcsname{39.4}
\expandafter\def\csname tpsd@lp_zimage_g1\endcsname{39.4$\pm$0.7}
\expandafter\def\csname tpn@lp_zimage_g1\endcsname{2}
\expandafter\def\csname tpsec@lp_zimage_g1\endcsname{1.92}
\expandafter\def\csname tpnfe@lp_zimage_g1\endcsname{50}
\expandafter\def\csname tpfid@lp_zimage_g1\endcsname{29.4}
\expandafter\def\csname tprec@lp_zimage_g1\endcsname{0.39}
\expandafter\def\csname tp@lp_zimage_turbo\endcsname{13.8}
\expandafter\def\csname tpsd@lp_zimage_turbo\endcsname{13.8$\pm$0.5}
\expandafter\def\csname tpn@lp_zimage_turbo\endcsname{2}
\expandafter\def\csname tpsec@lp_zimage_turbo\endcsname{0.37}
\expandafter\def\csname tpnfe@lp_zimage_turbo\endcsname{9}
\expandafter\def\csname tpfid@lp_zimage_turbo\endcsname{56.2}
\expandafter\def\csname tprec@lp_zimage_turbo\endcsname{0.00}
\expandafter\def\csname tp@lp_zt_dd3_g1\endcsname{28.9}
\expandafter\def\csname tpsd@lp_zt_dd3_g1\endcsname{28.9$\pm$0.7}
\expandafter\def\csname tpn@lp_zt_dd3_g1\endcsname{2}
\expandafter\def\csname tpsec@lp_zt_dd3_g1\endcsname{0.37}
\expandafter\def\csname tpnfe@lp_zt_dd3_g1\endcsname{9}
\expandafter\def\csname tpfid@lp_zt_dd3_g1\endcsname{26.4}
\expandafter\def\csname tprec@lp_zt_dd3_g1\endcsname{0.08}
\expandafter\def\csname tp@mix_kb_dd2_g1\endcsname{80.7}
\expandafter\def\csname tpsd@mix_kb_dd2_g1\endcsname{80.7$\pm$0.3}
\expandafter\def\csname tpn@mix_kb_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@mix_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@mix_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@mix_kb_dd2_g1\endcsname{29.9}
\expandafter\def\csname tprec@mix_kb_dd2_g1\endcsname{0.17}
\expandafter\def\csname tp@mix_kb_g1\endcsname{79.6}
\expandafter\def\csname tpsd@mix_kb_g1\endcsname{79.6$\pm$0.3}
\expandafter\def\csname tpn@mix_kb_g1\endcsname{3}
\expandafter\def\csname tpsec@mix_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@mix_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@mix_kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@mix_kb_g1\endcsname{0.49}
\expandafter\def\csname tp@mix_kd_ad2\endcsname{80.4}
\expandafter\def\csname tpsd@mix_kd_ad2\endcsname{80.4$\pm$0.1}
\expandafter\def\csname tpn@mix_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@mix_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@mix_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@mix_kd_ad2\endcsname{34.8}
\expandafter\def\csname tprec@mix_kd_ad2\endcsname{0.28}
\expandafter\def\csname tp@mix_klein\endcsname{78.7}
\expandafter\def\csname tpsd@mix_klein\endcsname{78.7$\pm$0.4}
\expandafter\def\csname tpn@mix_klein\endcsname{3}
\expandafter\def\csname tpsec@mix_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@mix_klein\endcsname{4}
\expandafter\def\csname tpfid@mix_klein\endcsname{47.6}
\expandafter\def\csname tprec@mix_klein\endcsname{0.01}
\expandafter\def\csname tp@mix_klein_base\endcsname{78.8}
\expandafter\def\csname tpsd@mix_klein_base\endcsname{78.8$\pm$0.7}
\expandafter\def\csname tpn@mix_klein_base\endcsname{3}
\expandafter\def\csname tpsec@mix_klein_base\endcsname{2.82}
\expandafter\def\csname tpnfe@mix_klein_base\endcsname{100}
\expandafter\def\csname tpfid@mix_klein_base\endcsname{42.6}
\expandafter\def\csname tprec@mix_klein_base\endcsname{0.04}
\expandafter\def\csname tp@mix_sd15\endcsname{80.4}
\expandafter\def\csname tpsd@mix_sd15\endcsname{80.4$\pm$0.2}
\expandafter\def\csname tpn@mix_sd15\endcsname{3}
\expandafter\def\csname tpsec@mix_sd15\endcsname{0.21}
\expandafter\def\csname tpnfe@mix_sd15\endcsname{60}
\expandafter\def\csname tpfid@mix_sd15\endcsname{26.6}
\expandafter\def\csname tprec@mix_sd15\endcsname{0.06}
\expandafter\def\csname tp@mix_sd15_g2\endcsname{81.0}
\expandafter\def\csname tpsd@mix_sd15_g2\endcsname{81.0$\pm$0.1}
\expandafter\def\csname tpn@mix_sd15_g2\endcsname{3}
\expandafter\def\csname tpsec@mix_sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@mix_sd15_g2\endcsname{60}
\expandafter\def\csname tpfid@mix_sd15_g2\endcsname{25.3}
\expandafter\def\csname tprec@mix_sd15_g2\endcsname{0.31}
\expandafter\def\csname tp@mix_sd21_g1\endcsname{80.5}
\expandafter\def\csname tpsd@mix_sd21_g1\endcsname{80.5$\pm$0.4}
\expandafter\def\csname tpn@mix_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@mix_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@mix_sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@mix_sd21_g1\endcsname{50.2}
\expandafter\def\csname tprec@mix_sd21_g1\endcsname{0.33}
\expandafter\def\csname tp@mix_sdt4\endcsname{79.3}
\expandafter\def\csname tpsd@mix_sdt4\endcsname{79.3$\pm$0.2}
\expandafter\def\csname tpn@mix_sdt4\endcsname{3}
\expandafter\def\csname tpsec@mix_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@mix_sdt4\endcsname{4}
\expandafter\def\csname tpfid@mix_sdt4\endcsname{37.5}
\expandafter\def\csname tprec@mix_sdt4\endcsname{0.02}
\expandafter\def\csname tp@mix_sdt_ad1\endcsname{82.2}
\expandafter\def\csname tpsd@mix_sdt_ad1\endcsname{82.2$\pm$0.3}
\expandafter\def\csname tpn@mix_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@mix_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@mix_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@mix_sdt_ad1\endcsname{30.2}
\expandafter\def\csname tprec@mix_sdt_ad1\endcsname{0.16}
\expandafter\def\csname tp@pets_kb_dd2_g1\endcsname{45.3}
\expandafter\def\csname tpsd@pets_kb_dd2_g1\endcsname{45.3$\pm$0.5}
\expandafter\def\csname tpn@pets_kb_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@pets_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@pets_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tp@pets_kb_g1_s20\endcsname{47.4}
\expandafter\def\csname tpsd@pets_kb_g1_s20\endcsname{47.4$\pm$0.3}
\expandafter\def\csname tpn@pets_kb_g1_s20\endcsname{3}
\expandafter\def\csname tpsec@pets_kb_g1_s20\endcsname{0.57}
\expandafter\def\csname tpnfe@pets_kb_g1_s20\endcsname{20}
\expandafter\def\csname tp@pets_kd_ad2\endcsname{46.2}
\expandafter\def\csname tpsd@pets_kd_ad2\endcsname{46.2$\pm$0.8}
\expandafter\def\csname tpn@pets_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@pets_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@pets_kd_ad2\endcsname{2}
\expandafter\def\csname tp@pets_klein\endcsname{20.5}
\expandafter\def\csname tpsd@pets_klein\endcsname{20.5$\pm$1.0}
\expandafter\def\csname tpn@pets_klein\endcsname{3}
\expandafter\def\csname tpsec@pets_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@pets_klein\endcsname{4}
\expandafter\def\csname tp@pets_real\endcsname{64.1}
\expandafter\def\csname tpsd@pets_real\endcsname{64.1$\pm$0.7}
\expandafter\def\csname tpn@pets_real\endcsname{3}
\expandafter\def\csname tp@pets_sd21_g1\endcsname{65.5}
\expandafter\def\csname tpsd@pets_sd21_g1\endcsname{65.5$\pm$0.6}
\expandafter\def\csname tpn@pets_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@pets_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@pets_sd21_g1\endcsname{30}
\expandafter\def\csname tp@pets_sdt4\endcsname{19.5}
\expandafter\def\csname tpsd@pets_sdt4\endcsname{19.5$\pm$1.4}
\expandafter\def\csname tpn@pets_sdt4\endcsname{3}
\expandafter\def\csname tpsec@pets_sdt4\endcsname{0.06}
\expandafter\def\csname tpnfe@pets_sdt4\endcsname{4}
\expandafter\def\csname tp@pets_sdt4_dd2_g1\endcsname{50.6}
\expandafter\def\csname tpsd@pets_sdt4_dd2_g1\endcsname{50.6$\pm$0.9}
\expandafter\def\csname tpn@pets_sdt4_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@pets_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@pets_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tp@pets_sdt_ad1\endcsname{54.5}
\expandafter\def\csname tpsd@pets_sdt_ad1\endcsname{54.5$\pm$0.9}
\expandafter\def\csname tpn@pets_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@pets_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@pets_sdt_ad1\endcsname{3}
\expandafter\def\csname tp@ra_kb_g1\endcsname{47.8}
\expandafter\def\csname tpsd@ra_kb_g1\endcsname{47.8$\pm$0.2}
\expandafter\def\csname tpn@ra_kb_g1\endcsname{3}
\expandafter\def\csname tpsec@ra_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@ra_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@ra_kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@ra_kb_g1\endcsname{0.49}
\expandafter\def\csname tp@ra_kd_ad2\endcsname{46.7}
\expandafter\def\csname tpsd@ra_kd_ad2\endcsname{46.7$\pm$0.4}
\expandafter\def\csname tpn@ra_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@ra_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@ra_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@ra_kd_ad2\endcsname{34.8}
\expandafter\def\csname tprec@ra_kd_ad2\endcsname{0.28}
\expandafter\def\csname tp@ra_klein\endcsname{22.0}
\expandafter\def\csname tpsd@ra_klein\endcsname{22.0$\pm$0.3}
\expandafter\def\csname tpn@ra_klein\endcsname{3}
\expandafter\def\csname tpsec@ra_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@ra_klein\endcsname{4}
\expandafter\def\csname tpfid@ra_klein\endcsname{47.6}
\expandafter\def\csname tprec@ra_klein\endcsname{0.01}
\expandafter\def\csname tp@ra_real500\endcsname{80.3}
\expandafter\def\csname tpsd@ra_real500\endcsname{80.3$\pm$0.2}
\expandafter\def\csname tpn@ra_real500\endcsname{3}
\expandafter\def\csname tp@ra_sd21_g1\endcsname{52.8}
\expandafter\def\csname tpsd@ra_sd21_g1\endcsname{52.8$\pm$0.8}
\expandafter\def\csname tpn@ra_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@ra_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@ra_sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@ra_sd21_g1\endcsname{50.2}
\expandafter\def\csname tprec@ra_sd21_g1\endcsname{0.33}
\expandafter\def\csname tp@ra_sdt4\endcsname{23.4}
\expandafter\def\csname tpsd@ra_sdt4\endcsname{23.4$\pm$0.7}
\expandafter\def\csname tpn@ra_sdt4\endcsname{3}
\expandafter\def\csname tpsec@ra_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@ra_sdt4\endcsname{4}
\expandafter\def\csname tpfid@ra_sdt4\endcsname{37.5}
\expandafter\def\csname tprec@ra_sdt4\endcsname{0.02}
\expandafter\def\csname tp@ra_sdt_ad1\endcsname{48.0}
\expandafter\def\csname tpsd@ra_sdt_ad1\endcsname{48.0$\pm$0.6}
\expandafter\def\csname tpn@ra_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@ra_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@ra_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@ra_sdt_ad1\endcsname{30.2}
\expandafter\def\csname tprec@ra_sdt_ad1\endcsname{0.16}
\expandafter\def\csname tp@real500\endcsname{77.1}
\expandafter\def\csname tpsd@real500\endcsname{77.1$\pm$0.2}
\expandafter\def\csname tpn@real500\endcsname{3}
\expandafter\def\csname tp@real500_e200\endcsname{78.8}
\expandafter\def\csname tpsd@real500_e200\endcsname{78.8$\pm$0.0}
\expandafter\def\csname tpn@real500_e200\endcsname{3}
\expandafter\def\csname tp@scale_kd_ad2_100\endcsname{24.4}
\expandafter\def\csname tpsd@scale_kd_ad2_100\endcsname{24.4$\pm$0.9}
\expandafter\def\csname tpn@scale_kd_ad2_100\endcsname{2}
\expandafter\def\csname tpsec@scale_kd_ad2_100\endcsname{0.10}
\expandafter\def\csname tpnfe@scale_kd_ad2_100\endcsname{2}
\expandafter\def\csname tpfid@scale_kd_ad2_100\endcsname{34.8}
\expandafter\def\csname tprec@scale_kd_ad2_100\endcsname{0.28}
\expandafter\def\csname tp@scale_kd_ad2_1300\endcsname{51.7}
\expandafter\def\csname tpsd@scale_kd_ad2_1300\endcsname{51.7$\pm$0.6}
\expandafter\def\csname tpn@scale_kd_ad2_1300\endcsname{2}
\expandafter\def\csname tpsec@scale_kd_ad2_1300\endcsname{0.10}
\expandafter\def\csname tpnfe@scale_kd_ad2_1300\endcsname{2}
\expandafter\def\csname tpfid@scale_kd_ad2_1300\endcsname{34.8}
\expandafter\def\csname tprec@scale_kd_ad2_1300\endcsname{0.28}
\expandafter\def\csname tp@scale_kd_ad2_300\endcsname{38.8}
\expandafter\def\csname tpsd@scale_kd_ad2_300\endcsname{38.8$\pm$0.1}
\expandafter\def\csname tpn@scale_kd_ad2_300\endcsname{2}
\expandafter\def\csname tpsec@scale_kd_ad2_300\endcsname{0.10}
\expandafter\def\csname tpnfe@scale_kd_ad2_300\endcsname{2}
\expandafter\def\csname tpfid@scale_kd_ad2_300\endcsname{34.8}
\expandafter\def\csname tprec@scale_kd_ad2_300\endcsname{0.28}
\expandafter\def\csname tp@scale_kd_ad2_3000\endcsname{57.0}
\expandafter\def\csname tpsd@scale_kd_ad2_3000\endcsname{57.0$\pm$0.5}
\expandafter\def\csname tpn@scale_kd_ad2_3000\endcsname{2}
\expandafter\def\csname tpsec@scale_kd_ad2_3000\endcsname{0.10}
\expandafter\def\csname tpnfe@scale_kd_ad2_3000\endcsname{2}
\expandafter\def\csname tpfid@scale_kd_ad2_3000\endcsname{34.8}
\expandafter\def\csname tprec@scale_kd_ad2_3000\endcsname{0.28}
\expandafter\def\csname tp@scale_klein_100\endcsname{12.6}
\expandafter\def\csname tpsd@scale_klein_100\endcsname{12.6$\pm$0.2}
\expandafter\def\csname tpn@scale_klein_100\endcsname{2}
\expandafter\def\csname tpsec@scale_klein_100\endcsname{0.14}
\expandafter\def\csname tpnfe@scale_klein_100\endcsname{4}
\expandafter\def\csname tp@scale_klein_1300\endcsname{18.7}
\expandafter\def\csname tpsd@scale_klein_1300\endcsname{18.7$\pm$0.5}
\expandafter\def\csname tpn@scale_klein_1300\endcsname{2}
\expandafter\def\csname tpsec@scale_klein_1300\endcsname{0.14}
\expandafter\def\csname tpnfe@scale_klein_1300\endcsname{4}
\expandafter\def\csname tp@scale_klein_300\endcsname{15.8}
\expandafter\def\csname tpsd@scale_klein_300\endcsname{15.8$\pm$0.0}
\expandafter\def\csname tpn@scale_klein_300\endcsname{2}
\expandafter\def\csname tpsec@scale_klein_300\endcsname{0.14}
\expandafter\def\csname tpnfe@scale_klein_300\endcsname{4}
\expandafter\def\csname tp@scale_klein_3000\endcsname{19.5}
\expandafter\def\csname tpsd@scale_klein_3000\endcsname{19.5$\pm$0.0}
\expandafter\def\csname tpn@scale_klein_3000\endcsname{2}
\expandafter\def\csname tpsec@scale_klein_3000\endcsname{0.14}
\expandafter\def\csname tpnfe@scale_klein_3000\endcsname{4}
\expandafter\def\csname tp@scale_klein_500\endcsname{16.8}
\expandafter\def\csname tpsd@scale_klein_500\endcsname{16.8$\pm$0.4}
\expandafter\def\csname tpn@scale_klein_500\endcsname{2}
\expandafter\def\csname tpsec@scale_klein_500\endcsname{0.14}
\expandafter\def\csname tpnfe@scale_klein_500\endcsname{4}
\expandafter\def\csname tp@sd15\endcsname{32.9}
\expandafter\def\csname tpsd@sd15\endcsname{32.9$\pm$0.5}
\expandafter\def\csname tpn@sd15\endcsname{3}
\expandafter\def\csname tpsec@sd15\endcsname{0.21}
\expandafter\def\csname tpnfe@sd15\endcsname{60}
\expandafter\def\csname tpfid@sd15\endcsname{26.6}
\expandafter\def\csname tprec@sd15\endcsname{0.06}
\expandafter\def\csname tp@sd15_g2\endcsname{52.1}
\expandafter\def\csname tpsd@sd15_g2\endcsname{52.1$\pm$0.4}
\expandafter\def\csname tpn@sd15_g2\endcsname{3}
\expandafter\def\csname tpsec@sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@sd15_g2\endcsname{60}
\expandafter\def\csname tpfid@sd15_g2\endcsname{25.3}
\expandafter\def\csname tprec@sd15_g2\endcsname{0.31}
\expandafter\def\csname tp@sd21\endcsname{30.0}
\expandafter\def\csname tpsd@sd21\endcsname{30.0$\pm$0.1}
\expandafter\def\csname tpn@sd21\endcsname{3}
\expandafter\def\csname tpsec@sd21\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21\endcsname{60}
\expandafter\def\csname tpfid@sd21\endcsname{28.0}
\expandafter\def\csname tprec@sd21\endcsname{0.04}
\expandafter\def\csname tp@sd21_b2d10_g2\endcsname{24.4}
\expandafter\def\csname tpsd@sd21_b2d10_g2\endcsname{24.4$\pm$0.9}
\expandafter\def\csname tpn@sd21_b2d10_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_b2d10_g2\endcsname{0.14}
\expandafter\def\csname tpnfe@sd21_b2d10_g2\endcsname{40}
\expandafter\def\csname tpfid@sd21_b2d10_g2\endcsname{38.4}
\expandafter\def\csname tprec@sd21_b2d10_g2\endcsname{0.09}
\expandafter\def\csname tp@sd21_b2d15_g2\endcsname{37.4}
\expandafter\def\csname tpsd@sd21_b2d15_g2\endcsname{37.4$\pm$0.4}
\expandafter\def\csname tpn@sd21_b2d15_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_b2d15_g2\endcsname{0.15}
\expandafter\def\csname tpnfe@sd21_b2d15_g2\endcsname{45}
\expandafter\def\csname tpfid@sd21_b2d15_g2\endcsname{30.5}
\expandafter\def\csname tprec@sd21_b2d15_g2\endcsname{0.13}
\expandafter\def\csname tp@sd21_b2d20_g2\endcsname{46.5}
\expandafter\def\csname tpsd@sd21_b2d20_g2\endcsname{46.5$\pm$0.3}
\expandafter\def\csname tpn@sd21_b2d20_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_b2d20_g2\endcsname{0.17}
\expandafter\def\csname tpnfe@sd21_b2d20_g2\endcsname{50}
\expandafter\def\csname tpfid@sd21_b2d20_g2\endcsname{26.3}
\expandafter\def\csname tprec@sd21_b2d20_g2\endcsname{0.21}
\expandafter\def\csname tp@sd21_b2d25_g2\endcsname{48.9}
\expandafter\def\csname tpsd@sd21_b2d25_g2\endcsname{48.9$\pm$0.7}
\expandafter\def\csname tpn@sd21_b2d25_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_b2d25_g2\endcsname{0.18}
\expandafter\def\csname tpnfe@sd21_b2d25_g2\endcsname{55}
\expandafter\def\csname tpfid@sd21_b2d25_g2\endcsname{24.6}
\expandafter\def\csname tprec@sd21_b2d25_g2\endcsname{0.25}
\expandafter\def\csname tp@sd21_b2d5_g2\endcsname{17.2}
\expandafter\def\csname tpsd@sd21_b2d5_g2\endcsname{17.2$\pm$0.3}
\expandafter\def\csname tpn@sd21_b2d5_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_b2d5_g2\endcsname{0.13}
\expandafter\def\csname tpnfe@sd21_b2d5_g2\endcsname{35}
\expandafter\def\csname tpfid@sd21_b2d5_g2\endcsname{44.9}
\expandafter\def\csname tprec@sd21_b2d5_g2\endcsname{0.05}
\expandafter\def\csname tp@sd21_cads75_s01\endcsname{33.7}
\expandafter\def\csname tpsd@sd21_cads75_s01\endcsname{33.7$\pm$0.6}
\expandafter\def\csname tpn@sd21_cads75_s01\endcsname{3}
\expandafter\def\csname tpsec@sd21_cads75_s01\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_cads75_s01\endcsname{60}
\expandafter\def\csname tpfid@sd21_cads75_s01\endcsname{28.1}
\expandafter\def\csname tprec@sd21_cads75_s01\endcsname{0.06}
\expandafter\def\csname tp@sd21_cads75_s025\endcsname{34.5}
\expandafter\def\csname tpsd@sd21_cads75_s025\endcsname{34.5$\pm$0.4}
\expandafter\def\csname tpn@sd21_cads75_s025\endcsname{3}
\expandafter\def\csname tpsec@sd21_cads75_s025\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_cads75_s025\endcsname{60}
\expandafter\def\csname tpfid@sd21_cads75_s025\endcsname{28.4}
\expandafter\def\csname tprec@sd21_cads75_s025\endcsname{0.07}
\expandafter\def\csname tp@sd21_cfg_early\endcsname{48.6}
\expandafter\def\csname tpsd@sd21_cfg_early\endcsname{48.6$\pm$0.6}
\expandafter\def\csname tpn@sd21_cfg_early\endcsname{3}
\expandafter\def\csname tpsec@sd21_cfg_early\endcsname{0.15}
\expandafter\def\csname tpnfe@sd21_cfg_early\endcsname{45}
\expandafter\def\csname tpfid@sd21_cfg_early\endcsname{28.5}
\expandafter\def\csname tprec@sd21_cfg_early\endcsname{0.27}
\expandafter\def\csname tp@sd21_cfg_late\endcsname{53.7}
\expandafter\def\csname tpsd@sd21_cfg_late\endcsname{53.7$\pm$0.3}
\expandafter\def\csname tpn@sd21_cfg_late\endcsname{3}
\expandafter\def\csname tpsec@sd21_cfg_late\endcsname{0.15}
\expandafter\def\csname tpnfe@sd21_cfg_late\endcsname{45}
\expandafter\def\csname tpfid@sd21_cfg_late\endcsname{37.6}
\expandafter\def\csname tprec@sd21_cfg_late\endcsname{0.30}
\expandafter\def\csname tp@sd21_d2b10_g2\endcsname{27.4}
\expandafter\def\csname tpsd@sd21_d2b10_g2\endcsname{27.4$\pm$0.9}
\expandafter\def\csname tpn@sd21_d2b10_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_d2b10_g2\endcsname{0.17}
\expandafter\def\csname tpnfe@sd21_d2b10_g2\endcsname{50}
\expandafter\def\csname tpfid@sd21_d2b10_g2\endcsname{32.7}
\expandafter\def\csname tprec@sd21_d2b10_g2\endcsname{0.05}
\expandafter\def\csname tp@sd21_d2b15_g2\endcsname{19.1}
\expandafter\def\csname tpsd@sd21_d2b15_g2\endcsname{19.1$\pm$0.3}
\expandafter\def\csname tpn@sd21_d2b15_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_d2b15_g2\endcsname{0.15}
\expandafter\def\csname tpnfe@sd21_d2b15_g2\endcsname{45}
\expandafter\def\csname tpfid@sd21_d2b15_g2\endcsname{39.8}
\expandafter\def\csname tprec@sd21_d2b15_g2\endcsname{0.04}
\expandafter\def\csname tp@sd21_d2b20_g2\endcsname{15.1}
\expandafter\def\csname tpsd@sd21_d2b20_g2\endcsname{15.1$\pm$0.1}
\expandafter\def\csname tpn@sd21_d2b20_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_d2b20_g2\endcsname{0.14}
\expandafter\def\csname tpnfe@sd21_d2b20_g2\endcsname{40}
\expandafter\def\csname tpfid@sd21_d2b20_g2\endcsname{44.2}
\expandafter\def\csname tprec@sd21_d2b20_g2\endcsname{0.03}
\expandafter\def\csname tp@sd21_d2b25_g2\endcsname{13.9}
\expandafter\def\csname tpsd@sd21_d2b25_g2\endcsname{13.9$\pm$0.4}
\expandafter\def\csname tpn@sd21_d2b25_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_d2b25_g2\endcsname{0.13}
\expandafter\def\csname tpnfe@sd21_d2b25_g2\endcsname{35}
\expandafter\def\csname tpfid@sd21_d2b25_g2\endcsname{46.4}
\expandafter\def\csname tprec@sd21_d2b25_g2\endcsname{0.03}
\expandafter\def\csname tp@sd21_d2b5_g2\endcsname{38.9}
\expandafter\def\csname tpsd@sd21_d2b5_g2\endcsname{38.9$\pm$0.6}
\expandafter\def\csname tpn@sd21_d2b5_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_d2b5_g2\endcsname{0.18}
\expandafter\def\csname tpnfe@sd21_d2b5_g2\endcsname{55}
\expandafter\def\csname tpfid@sd21_d2b5_g2\endcsname{26.1}
\expandafter\def\csname tprec@sd21_d2b5_g2\endcsname{0.10}
\expandafter\def\csname tp@sd21_g1\endcsname{49.8}
\expandafter\def\csname tpsd@sd21_g1\endcsname{49.8$\pm$0.7}
\expandafter\def\csname tpn@sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@sd21_g1\endcsname{50.2}
\expandafter\def\csname tprec@sd21_g1\endcsname{0.33}
\expandafter\def\csname tp@sd21_g15\endcsname{51.3}
\expandafter\def\csname tpsd@sd21_g15\endcsname{51.3$\pm$0.2}
\expandafter\def\csname tpn@sd21_g15\endcsname{3}
\expandafter\def\csname tpsec@sd21_g15\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_g15\endcsname{60}
\expandafter\def\csname tpfid@sd21_g15\endcsname{30.9}
\expandafter\def\csname tprec@sd21_g15\endcsname{0.27}
\expandafter\def\csname tp@sd21_g1_s10\endcsname{46.7}
\expandafter\def\csname tpsd@sd21_g1_s10\endcsname{46.7$\pm$1.3}
\expandafter\def\csname tpn@sd21_g1_s10\endcsname{3}
\expandafter\def\csname tpsec@sd21_g1_s10\endcsname{0.05}
\expandafter\def\csname tpnfe@sd21_g1_s10\endcsname{10}
\expandafter\def\csname tpfid@sd21_g1_s10\endcsname{54.2}
\expandafter\def\csname tprec@sd21_g1_s10\endcsname{0.25}
\expandafter\def\csname tp@sd21_g2\endcsname{49.5}
\expandafter\def\csname tpsd@sd21_g2\endcsname{49.5$\pm$0.3}
\expandafter\def\csname tpn@sd21_g2\endcsname{3}
\expandafter\def\csname tpsec@sd21_g2\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_g2\endcsname{60}
\expandafter\def\csname tpfid@sd21_g2\endcsname{25.2}
\expandafter\def\csname tprec@sd21_g2\endcsname{0.22}
\expandafter\def\csname tp@sd21_g4\endcsname{40.8}
\expandafter\def\csname tpsd@sd21_g4\endcsname{40.8$\pm$0.3}
\expandafter\def\csname tpn@sd21_g4\endcsname{3}
\expandafter\def\csname tpsec@sd21_g4\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_g4\endcsname{60}
\expandafter\def\csname tpfid@sd21_g4\endcsname{24.3}
\expandafter\def\csname tprec@sd21_g4\endcsname{0.10}
\expandafter\def\csname tp@sd21_g75early\endcsname{31.2}
\expandafter\def\csname tpsd@sd21_g75early\endcsname{31.2$\pm$0.1}
\expandafter\def\csname tpn@sd21_g75early\endcsname{3}
\expandafter\def\csname tpsec@sd21_g75early\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_g75early\endcsname{60}
\expandafter\def\csname tpfid@sd21_g75early\endcsname{27.8}
\expandafter\def\csname tprec@sd21_g75early\endcsname{0.05}
\expandafter\def\csname tp@sd21_g75late\endcsname{47.6}
\expandafter\def\csname tpsd@sd21_g75late\endcsname{47.6$\pm$0.2}
\expandafter\def\csname tpn@sd21_g75late\endcsname{3}
\expandafter\def\csname tpsec@sd21_g75late\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_g75late\endcsname{60}
\expandafter\def\csname tpfid@sd21_g75late\endcsname{23.6}
\expandafter\def\csname tprec@sd21_g75late\endcsname{0.11}
\expandafter\def\csname tp@sd21_hi12\endcsname{31.9}
\expandafter\def\csname tpsd@sd21_hi12\endcsname{31.9$\pm$0.5}
\expandafter\def\csname tpn@sd21_hi12\endcsname{3}
\expandafter\def\csname tpsec@sd21_hi12\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_hi12\endcsname{60}
\expandafter\def\csname tpfid@sd21_hi12\endcsname{27.5}
\expandafter\def\csname tprec@sd21_hi12\endcsname{0.07}
\expandafter\def\csname tp@sd21_hi18\endcsname{30.9}
\expandafter\def\csname tpsd@sd21_hi18\endcsname{30.9$\pm$0.7}
\expandafter\def\csname tpn@sd21_hi18\endcsname{3}
\expandafter\def\csname tpsec@sd21_hi18\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_hi18\endcsname{60}
\expandafter\def\csname tpfid@sd21_hi18\endcsname{28.0}
\expandafter\def\csname tprec@sd21_hi18\endcsname{0.05}
\expandafter\def\csname tp@sd21_hi24\endcsname{30.6}
\expandafter\def\csname tpsd@sd21_hi24\endcsname{30.6$\pm$0.2}
\expandafter\def\csname tpn@sd21_hi24\endcsname{3}
\expandafter\def\csname tpsec@sd21_hi24\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_hi24\endcsname{60}
\expandafter\def\csname tpfid@sd21_hi24\endcsname{28.1}
\expandafter\def\csname tprec@sd21_hi24\endcsname{0.04}
\expandafter\def\csname tp@sd21_hi3\endcsname{43.2}
\expandafter\def\csname tpsd@sd21_hi3\endcsname{43.2$\pm$0.5}
\expandafter\def\csname tpn@sd21_hi3\endcsname{3}
\expandafter\def\csname tpsec@sd21_hi3\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_hi3\endcsname{60}
\expandafter\def\csname tpfid@sd21_hi3\endcsname{24.1}
\expandafter\def\csname tprec@sd21_hi3\endcsname{0.18}
\expandafter\def\csname tp@sd21_hi6\endcsname{36.5}
\expandafter\def\csname tpsd@sd21_hi6\endcsname{36.5$\pm$0.3}
\expandafter\def\csname tpn@sd21_hi6\endcsname{3}
\expandafter\def\csname tpsec@sd21_hi6\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_hi6\endcsname{60}
\expandafter\def\csname tpfid@sd21_hi6\endcsname{25.6}
\expandafter\def\csname tprec@sd21_hi6\endcsname{0.12}
\expandafter\def\csname tp@sd21_hi9\endcsname{33.0}
\expandafter\def\csname tpsd@sd21_hi9\endcsname{33.0$\pm$0.2}
\expandafter\def\csname tpn@sd21_hi9\endcsname{3}
\expandafter\def\csname tpsec@sd21_hi9\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_hi9\endcsname{60}
\expandafter\def\csname tpfid@sd21_hi9\endcsname{26.7}
\expandafter\def\csname tprec@sd21_hi9\endcsname{0.08}
\expandafter\def\csname tp@sd21_interval75\endcsname{40.7}
\expandafter\def\csname tpsd@sd21_interval75\endcsname{40.7$\pm$0.4}
\expandafter\def\csname tpn@sd21_interval75\endcsname{3}
\expandafter\def\csname tpsec@sd21_interval75\endcsname{0.17}
\expandafter\def\csname tpnfe@sd21_interval75\endcsname{52}
\expandafter\def\csname tpfid@sd21_interval75\endcsname{25.0}
\expandafter\def\csname tprec@sd21_interval75\endcsname{0.07}
\expandafter\def\csname tp@sd21_lo12\endcsname{45.6}
\expandafter\def\csname tpsd@sd21_lo12\endcsname{45.6$\pm$0.5}
\expandafter\def\csname tpn@sd21_lo12\endcsname{3}
\expandafter\def\csname tpsec@sd21_lo12\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_lo12\endcsname{60}
\expandafter\def\csname tpfid@sd21_lo12\endcsname{23.9}
\expandafter\def\csname tprec@sd21_lo12\endcsname{0.09}
\expandafter\def\csname tp@sd21_lo18\endcsname{48.4}
\expandafter\def\csname tpsd@sd21_lo18\endcsname{48.4$\pm$0.4}
\expandafter\def\csname tpn@sd21_lo18\endcsname{3}
\expandafter\def\csname tpsec@sd21_lo18\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_lo18\endcsname{60}
\expandafter\def\csname tpfid@sd21_lo18\endcsname{23.6}
\expandafter\def\csname tprec@sd21_lo18\endcsname{0.13}
\expandafter\def\csname tp@sd21_lo24\endcsname{49.9}
\expandafter\def\csname tpsd@sd21_lo24\endcsname{49.9$\pm$0.4}
\expandafter\def\csname tpn@sd21_lo24\endcsname{3}
\expandafter\def\csname tpsec@sd21_lo24\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_lo24\endcsname{60}
\expandafter\def\csname tpfid@sd21_lo24\endcsname{24.0}
\expandafter\def\csname tprec@sd21_lo24\endcsname{0.17}
\expandafter\def\csname tp@sd21_lo3\endcsname{35.0}
\expandafter\def\csname tpsd@sd21_lo3\endcsname{35.0$\pm$0.2}
\expandafter\def\csname tpn@sd21_lo3\endcsname{3}
\expandafter\def\csname tpsec@sd21_lo3\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_lo3\endcsname{60}
\expandafter\def\csname tpfid@sd21_lo3\endcsname{26.5}
\expandafter\def\csname tprec@sd21_lo3\endcsname{0.05}
\expandafter\def\csname tp@sd21_lo6\endcsname{39.5}
\expandafter\def\csname tpsd@sd21_lo6\endcsname{39.5$\pm$0.3}
\expandafter\def\csname tpn@sd21_lo6\endcsname{3}
\expandafter\def\csname tpsec@sd21_lo6\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_lo6\endcsname{60}
\expandafter\def\csname tpfid@sd21_lo6\endcsname{25.3}
\expandafter\def\csname tprec@sd21_lo6\endcsname{0.06}
\expandafter\def\csname tp@sd21_lo9\endcsname{42.6}
\expandafter\def\csname tpsd@sd21_lo9\endcsname{42.6$\pm$0.3}
\expandafter\def\csname tpn@sd21_lo9\endcsname{3}
\expandafter\def\csname tpsec@sd21_lo9\endcsname{0.20}
\expandafter\def\csname tpnfe@sd21_lo9\endcsname{60}
\expandafter\def\csname tpfid@sd21_lo9\endcsname{24.5}
\expandafter\def\csname tprec@sd21_lo9\endcsname{0.07}
\expandafter\def\csname tp@sd21_turbo_all30\endcsname{13.4}
\expandafter\def\csname tpsd@sd21_turbo_all30\endcsname{13.4$\pm$0.2}
\expandafter\def\csname tpn@sd21_turbo_all30\endcsname{3}
\expandafter\def\csname tpsec@sd21_turbo_all30\endcsname{0.11}
\expandafter\def\csname tpnfe@sd21_turbo_all30\endcsname{30}
\expandafter\def\csname tpfid@sd21_turbo_all30\endcsname{46.9}
\expandafter\def\csname tprec@sd21_turbo_all30\endcsname{0.03}
\expandafter\def\csname tp@sd35_large\endcsname{20.0}
\expandafter\def\csname tpsd@sd35_large\endcsname{20.0$\pm$0.3}
\expandafter\def\csname tpn@sd35_large\endcsname{3}
\expandafter\def\csname tpsec@sd35_large\endcsname{1.42}
\expandafter\def\csname tpnfe@sd35_large\endcsname{56}
\expandafter\def\csname tpfid@sd35_large\endcsname{33.0}
\expandafter\def\csname tprec@sd35_large\endcsname{0.05}
\expandafter\def\csname tp@sd35_large_g1\endcsname{33.1}
\expandafter\def\csname tpsd@sd35_large_g1\endcsname{33.1$\pm$0.8}
\expandafter\def\csname tpn@sd35_large_g1\endcsname{3}
\expandafter\def\csname tpsec@sd35_large_g1\endcsname{0.75}
\expandafter\def\csname tpnfe@sd35_large_g1\endcsname{28}
\expandafter\def\csname tpfid@sd35_large_g1\endcsname{98.2}
\expandafter\def\csname tprec@sd35_large_g1\endcsname{0.08}
\expandafter\def\csname tp@sd35_large_g1_s10\endcsname{29.8}
\expandafter\def\csname tpsd@sd35_large_g1_s10\endcsname{29.8$\pm$0.4}
\expandafter\def\csname tpn@sd35_large_g1_s10\endcsname{3}
\expandafter\def\csname tpsec@sd35_large_g1_s10\endcsname{0.28}
\expandafter\def\csname tpnfe@sd35_large_g1_s10\endcsname{10}
\expandafter\def\csname tpfid@sd35_large_g1_s10\endcsname{113.5}
\expandafter\def\csname tprec@sd35_large_g1_s10\endcsname{0.05}
\expandafter\def\csname tp@sd35_large_g2\endcsname{28.9}
\expandafter\def\csname tpsd@sd35_large_g2\endcsname{28.9$\pm$0.3}
\expandafter\def\csname tpn@sd35_large_g2\endcsname{3}
\expandafter\def\csname tpsec@sd35_large_g2\endcsname{1.42}
\expandafter\def\csname tpnfe@sd35_large_g2\endcsname{56}
\expandafter\def\csname tpfid@sd35_large_g2\endcsname{29.2}
\expandafter\def\csname tprec@sd35_large_g2\endcsname{0.08}
\expandafter\def\csname tp@sd35_turbo\endcsname{18.2}
\expandafter\def\csname tpsd@sd35_turbo\endcsname{18.2$\pm$0.2}
\expandafter\def\csname tpn@sd35_turbo\endcsname{3}
\expandafter\def\csname tpsec@sd35_turbo\endcsname{0.13}
\expandafter\def\csname tpnfe@sd35_turbo\endcsname{4}
\expandafter\def\csname tpfid@sd35_turbo\endcsname{37.9}
\expandafter\def\csname tprec@sd35_turbo\endcsname{0.04}
\expandafter\def\csname tp@sd35m\endcsname{21.1}
\expandafter\def\csname tpsd@sd35m\endcsname{21.1$\pm$0.5}
\expandafter\def\csname tpn@sd35m\endcsname{3}
\expandafter\def\csname tpsec@sd35m\endcsname{0.61}
\expandafter\def\csname tpnfe@sd35m\endcsname{56}
\expandafter\def\csname tpfid@sd35m\endcsname{34.5}
\expandafter\def\csname tprec@sd35m\endcsname{0.04}
\expandafter\def\csname tp@sd35m_g1\endcsname{44.9}
\expandafter\def\csname tpsd@sd35m_g1\endcsname{44.9$\pm$0.3}
\expandafter\def\csname tpn@sd35m_g1\endcsname{3}
\expandafter\def\csname tpsec@sd35m_g1\endcsname{0.33}
\expandafter\def\csname tpnfe@sd35m_g1\endcsname{28}
\expandafter\def\csname tpfid@sd35m_g1\endcsname{34.1}
\expandafter\def\csname tprec@sd35m_g1\endcsname{0.25}
\expandafter\def\csname tp@sd35t_ad0\endcsname{30.8}
\expandafter\def\csname tpsd@sd35t_ad0\endcsname{30.8$\pm$0.2}
\expandafter\def\csname tpn@sd35t_ad0\endcsname{3}
\expandafter\def\csname tpsec@sd35t_ad0\endcsname{0.14}
\expandafter\def\csname tpnfe@sd35t_ad0\endcsname{4}
\expandafter\def\csname tpfid@sd35t_ad0\endcsname{60.6}
\expandafter\def\csname tprec@sd35t_ad0\endcsname{0.08}
\expandafter\def\csname tp@sd35t_ad0_s1\endcsname{30.0}
\expandafter\def\csname tpsd@sd35t_ad0_s1\endcsname{30.0$\pm$0.2}
\expandafter\def\csname tpn@sd35t_ad0_s1\endcsname{3}
\expandafter\def\csname tpsec@sd35t_ad0_s1\endcsname{0.14}
\expandafter\def\csname tpnfe@sd35t_ad0_s1\endcsname{4}
\expandafter\def\csname tpfid@sd35t_ad0_s1\endcsname{59.9}
\expandafter\def\csname tprec@sd35t_ad0_s1\endcsname{0.08}
\expandafter\def\csname tp@sd35t_ad0_s2\endcsname{29.8}
\expandafter\def\csname tpsd@sd35t_ad0_s2\endcsname{29.8$\pm$0.9}
\expandafter\def\csname tpn@sd35t_ad0_s2\endcsname{3}
\expandafter\def\csname tpsec@sd35t_ad0_s2\endcsname{0.14}
\expandafter\def\csname tpnfe@sd35t_ad0_s2\endcsname{4}
\expandafter\def\csname tpfid@sd35t_ad0_s2\endcsname{60.4}
\expandafter\def\csname tprec@sd35t_ad0_s2\endcsname{0.08}
\expandafter\def\csname tp@sd35t_ad0_tg2\endcsname{21.5}
\expandafter\def\csname tpsd@sd35t_ad0_tg2\endcsname{21.5$\pm$0.1}
\expandafter\def\csname tpn@sd35t_ad0_tg2\endcsname{3}
\expandafter\def\csname tpsec@sd35t_ad0_tg2\endcsname{0.14}
\expandafter\def\csname tpnfe@sd35t_ad0_tg2\endcsname{4}
\expandafter\def\csname tpfid@sd35t_ad0_tg2\endcsname{36.5}
\expandafter\def\csname tprec@sd35t_ad0_tg2\endcsname{0.06}
\expandafter\def\csname tp@sd35t_ad0_tg35\endcsname{14.4}
\expandafter\def\csname tpsd@sd35t_ad0_tg35\endcsname{14.4$\pm$0.5}
\expandafter\def\csname tpn@sd35t_ad0_tg35\endcsname{3}
\expandafter\def\csname tpsec@sd35t_ad0_tg35\endcsname{0.14}
\expandafter\def\csname tpnfe@sd35t_ad0_tg35\endcsname{4}
\expandafter\def\csname tpfid@sd35t_ad0_tg35\endcsname{38.6}
\expandafter\def\csname tprec@sd35t_ad0_tg35\endcsname{0.04}
\expandafter\def\csname tp@sd35t_ad0_x3\endcsname{30.2}
\expandafter\def\csname tpsd@sd35t_ad0_x3\endcsname{30.2$\pm$0.7}
\expandafter\def\csname tpn@sd35t_ad0_x3\endcsname{9}
\expandafter\def\csname tpsec@sd35t_ad0_x3\endcsname{0.14}
\expandafter\def\csname tpnfe@sd35t_ad0_x3\endcsname{4}
\expandafter\def\csname tp@sd35t_ad1\endcsname{23.1}
\expandafter\def\csname tpsd@sd35t_ad1\endcsname{23.1$\pm$0.1}
\expandafter\def\csname tpn@sd35t_ad1\endcsname{3}
\expandafter\def\csname tpsec@sd35t_ad1\endcsname{0.12}
\expandafter\def\csname tpnfe@sd35t_ad1\endcsname{3}
\expandafter\def\csname tpfid@sd35t_ad1\endcsname{123.8}
\expandafter\def\csname tprec@sd35t_ad1\endcsname{0.05}
\expandafter\def\csname tp@sd35t_dd1_g1\endcsname{26.7}
\expandafter\def\csname tpsd@sd35t_dd1_g1\endcsname{26.7$\pm$0.0}
\expandafter\def\csname tpn@sd35t_dd1_g1\endcsname{3}
\expandafter\def\csname tpsec@sd35t_dd1_g1\endcsname{0.14}
\expandafter\def\csname tpnfe@sd35t_dd1_g1\endcsname{4}
\expandafter\def\csname tpfid@sd35t_dd1_g1\endcsname{48.1}
\expandafter\def\csname tprec@sd35t_dd1_g1\endcsname{0.05}
\expandafter\def\csname tp@sd35t_dd2_g1\endcsname{20.8}
\expandafter\def\csname tpsd@sd35t_dd2_g1\endcsname{20.8$\pm$0.4}
\expandafter\def\csname tpn@sd35t_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@sd35t_dd2_g1\endcsname{0.14}
\expandafter\def\csname tpnfe@sd35t_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@sd35t_dd2_g1\endcsname{92.6}
\expandafter\def\csname tprec@sd35t_dd2_g1\endcsname{0.04}
\expandafter\def\csname tp@sd35t_or18_d3\endcsname{29.5}
\expandafter\def\csname tpsd@sd35t_or18_d3\endcsname{29.5$\pm$0.5}
\expandafter\def\csname tpn@sd35t_or18_d3\endcsname{3}
\expandafter\def\csname tpsec@sd35t_or18_d3\endcsname{0.57}
\expandafter\def\csname tpnfe@sd35t_or18_d3\endcsname{21}
\expandafter\def\csname tpfid@sd35t_or18_d3\endcsname{56.0}
\expandafter\def\csname tprec@sd35t_or18_d3\endcsname{0.09}
\expandafter\def\csname tp@sd35t_or36_d2\endcsname{30.4}
\expandafter\def\csname tpsd@sd35t_or36_d2\endcsname{30.4$\pm$0.6}
\expandafter\def\csname tpn@sd35t_or36_d2\endcsname{3}
\expandafter\def\csname tpsec@sd35t_or36_d2\endcsname{1.01}
\expandafter\def\csname tpnfe@sd35t_or36_d2\endcsname{38}
\expandafter\def\csname tpfid@sd35t_or36_d2\endcsname{83.4}
\expandafter\def\csname tprec@sd35t_or36_d2\endcsname{0.07}
\expandafter\def\csname tp@sd35t_skip3\endcsname{14.2}
\expandafter\def\csname tpsd@sd35t_skip3\endcsname{14.2$\pm$0.3}
\expandafter\def\csname tpn@sd35t_skip3\endcsname{3}
\expandafter\def\csname tpsec@sd35t_skip3\endcsname{0.11}
\expandafter\def\csname tpnfe@sd35t_skip3\endcsname{3}
\expandafter\def\csname tpfid@sd35t_skip3\endcsname{39.2}
\expandafter\def\csname tprec@sd35t_skip3\endcsname{0.01}
\expandafter\def\csname tp@sd_turbo\endcsname{15.8}
\expandafter\def\csname tpsd@sd_turbo\endcsname{15.8$\pm$0.4}
\expandafter\def\csname tpn@sd_turbo\endcsname{3}
\expandafter\def\csname tpsec@sd_turbo\endcsname{0.02}
\expandafter\def\csname tpnfe@sd_turbo\endcsname{1}
\expandafter\def\csname tpfid@sd_turbo\endcsname{36.5}
\expandafter\def\csname tprec@sd_turbo\endcsname{0.00}
\expandafter\def\csname tp@sdt4\endcsname{18.3}
\expandafter\def\csname tpsd@sdt4\endcsname{18.3$\pm$0.3}
\expandafter\def\csname tpn@sdt4\endcsname{3}
\expandafter\def\csname tpsec@sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt4\endcsname{4}
\expandafter\def\csname tpfid@sdt4\endcsname{37.5}
\expandafter\def\csname tprec@sdt4\endcsname{0.02}
\expandafter\def\csname tp@sdt4_dd1_g2\endcsname{27.5}
\expandafter\def\csname tpsd@sdt4_dd1_g2\endcsname{27.5$\pm$0.7}
\expandafter\def\csname tpn@sdt4_dd1_g2\endcsname{3}
\expandafter\def\csname tpsec@sdt4_dd1_g2\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt4_dd1_g2\endcsname{5}
\expandafter\def\csname tpfid@sdt4_dd1_g2\endcsname{32.7}
\expandafter\def\csname tprec@sdt4_dd1_g2\endcsname{0.04}
\expandafter\def\csname tp@sdt4_dd2_g1\endcsname{36.4}
\expandafter\def\csname tpsd@sdt4_dd2_g1\endcsname{36.4$\pm$0.9}
\expandafter\def\csname tpn@sdt4_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@sdt4_dd2_g1\endcsname{32.1}
\expandafter\def\csname tprec@sdt4_dd2_g1\endcsname{0.12}
\expandafter\def\csname tp@sdt4_dd2_g2\endcsname{36.9}
\expandafter\def\csname tpsd@sdt4_dd2_g2\endcsname{36.9$\pm$0.1}
\expandafter\def\csname tpn@sdt4_dd2_g2\endcsname{3}
\expandafter\def\csname tpsec@sdt4_dd2_g2\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt4_dd2_g2\endcsname{6}
\expandafter\def\csname tpfid@sdt4_dd2_g2\endcsname{27.9}
\expandafter\def\csname tprec@sdt4_dd2_g2\endcsname{0.10}
\expandafter\def\csname tp@sdt4_ns1\endcsname{17.1}
\expandafter\def\csname tpsd@sdt4_ns1\endcsname{17.1$\pm$0.7}
\expandafter\def\csname tpn@sdt4_ns1\endcsname{3}
\expandafter\def\csname tpsec@sdt4_ns1\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt4_ns1\endcsname{4}
\expandafter\def\csname tpfid@sdt4_ns1\endcsname{37.6}
\expandafter\def\csname tprec@sdt4_ns1\endcsname{0.03}
\expandafter\def\csname tp@sdt_ad0\endcsname{32.2}
\expandafter\def\csname tpsd@sdt_ad0\endcsname{32.2$\pm$0.4}
\expandafter\def\csname tpn@sdt_ad0\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad0\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad0\endcsname{4}
\expandafter\def\csname tpfid@sdt_ad0\endcsname{31.2}
\expandafter\def\csname tprec@sdt_ad0\endcsname{0.06}
\expandafter\def\csname tp@sdt_ad1\endcsname{43.3}
\expandafter\def\csname tpsd@sdt_ad1\endcsname{43.3$\pm$0.2}
\expandafter\def\csname tpn@sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1\endcsname{30.2}
\expandafter\def\csname tprec@sdt_ad1\endcsname{0.16}
\expandafter\def\csname tp@sdt_ad1_all\endcsname{38.8}
\expandafter\def\csname tpsd@sdt_ad1_all\endcsname{38.8$\pm$0.8}
\expandafter\def\csname tpn@sdt_ad1_all\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_all\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_all\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_all\endcsname{65.9}
\expandafter\def\csname tprec@sdt_ad1_all\endcsname{0.18}
\expandafter\def\csname tp@sdt_ad1_full_lr1e5\endcsname{43.4}
\expandafter\def\csname tpsd@sdt_ad1_full_lr1e5\endcsname{43.4$\pm$0.3}
\expandafter\def\csname tpn@sdt_ad1_full_lr1e5\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_full_lr1e5\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_full_lr1e5\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_full_lr1e5\endcsname{30.3}
\expandafter\def\csname tprec@sdt_ad1_full_lr1e5\endcsname{0.17}
\expandafter\def\csname tp@sdt_ad1_full_lr3e6\endcsname{42.4}
\expandafter\def\csname tpsd@sdt_ad1_full_lr3e6\endcsname{42.4$\pm$1.0}
\expandafter\def\csname tpn@sdt_ad1_full_lr3e6\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_full_lr3e6\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_full_lr3e6\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_full_lr3e6\endcsname{30.6}
\expandafter\def\csname tprec@sdt_ad1_full_lr3e6\endcsname{0.17}
\expandafter\def\csname tp@sdt_ad1_ns1\endcsname{43.9}
\expandafter\def\csname tpsd@sdt_ad1_ns1\endcsname{43.9$\pm$0.1}
\expandafter\def\csname tpn@sdt_ad1_ns1\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_ns1\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_ns1\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_ns1\endcsname{30.0}
\expandafter\def\csname tprec@sdt_ad1_ns1\endcsname{0.18}
\expandafter\def\csname tp@sdt_ad1_r128\endcsname{44.5}
\expandafter\def\csname tpsd@sdt_ad1_r128\endcsname{44.5$\pm$0.5}
\expandafter\def\csname tpn@sdt_ad1_r128\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_r128\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_r128\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_r128\endcsname{30.0}
\expandafter\def\csname tprec@sdt_ad1_r128\endcsname{0.17}
\expandafter\def\csname tp@sdt_ad1_r128_s1\endcsname{44.4}
\expandafter\def\csname tpsd@sdt_ad1_r128_s1\endcsname{44.4$\pm$0.9}
\expandafter\def\csname tpn@sdt_ad1_r128_s1\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_r128_s1\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_r128_s1\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_r128_s1\endcsname{29.9}
\expandafter\def\csname tprec@sdt_ad1_r128_s1\endcsname{0.18}
\expandafter\def\csname tp@sdt_ad1_r128_s2\endcsname{44.3}
\expandafter\def\csname tpsd@sdt_ad1_r128_s2\endcsname{44.3$\pm$0.6}
\expandafter\def\csname tpn@sdt_ad1_r128_s2\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_r128_s2\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_r128_s2\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_r128_s2\endcsname{30.1}
\expandafter\def\csname tprec@sdt_ad1_r128_s2\endcsname{0.18}
\expandafter\def\csname tp@sdt_ad1_r128_x3\endcsname{44.4}
\expandafter\def\csname tpsd@sdt_ad1_r128_x3\endcsname{44.4$\pm$0.6}
\expandafter\def\csname tpn@sdt_ad1_r128_x3\endcsname{9}
\expandafter\def\csname tpsec@sdt_ad1_r128_x3\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_r128_x3\endcsname{3}
\expandafter\def\csname tp@sdt_ad1_r8\endcsname{43.3}
\expandafter\def\csname tpsd@sdt_ad1_r8\endcsname{43.3$\pm$0.3}
\expandafter\def\csname tpn@sdt_ad1_r8\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_r8\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_r8\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_r8\endcsname{30.6}
\expandafter\def\csname tprec@sdt_ad1_r8\endcsname{0.16}
\expandafter\def\csname tp@sdt_ad1_s1\endcsname{44.0}
\expandafter\def\csname tpsd@sdt_ad1_s1\endcsname{44.0$\pm$0.5}
\expandafter\def\csname tpn@sdt_ad1_s1\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_s1\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_s1\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_s1\endcsname{30.1}
\expandafter\def\csname tprec@sdt_ad1_s1\endcsname{0.17}
\expandafter\def\csname tp@sdt_ad1_s2\endcsname{43.8}
\expandafter\def\csname tpsd@sdt_ad1_s2\endcsname{43.8$\pm$0.7}
\expandafter\def\csname tpn@sdt_ad1_s2\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_s2\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_s2\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_s2\endcsname{30.3}
\expandafter\def\csname tprec@sdt_ad1_s2\endcsname{0.17}
\expandafter\def\csname tp@sdt_ad1_tg2\endcsname{41.2}
\expandafter\def\csname tpsd@sdt_ad1_tg2\endcsname{41.2$\pm$0.9}
\expandafter\def\csname tpn@sdt_ad1_tg2\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_tg2\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_tg2\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_tg2\endcsname{26.5}
\expandafter\def\csname tprec@sdt_ad1_tg2\endcsname{0.12}
\expandafter\def\csname tp@sdt_ad1_tg75\endcsname{30.4}
\expandafter\def\csname tpsd@sdt_ad1_tg75\endcsname{30.4$\pm$0.4}
\expandafter\def\csname tpn@sdt_ad1_tg75\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad1_tg75\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_tg75\endcsname{3}
\expandafter\def\csname tpfid@sdt_ad1_tg75\endcsname{28.1}
\expandafter\def\csname tprec@sdt_ad1_tg75\endcsname{0.05}
\expandafter\def\csname tp@sdt_ad1_x3\endcsname{43.7}
\expandafter\def\csname tpsd@sdt_ad1_x3\endcsname{43.7$\pm$0.6}
\expandafter\def\csname tpn@sdt_ad1_x3\endcsname{9}
\expandafter\def\csname tpsec@sdt_ad1_x3\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_ad1_x3\endcsname{3}
\expandafter\def\csname tp@sdt_ad2\endcsname{41.2}
\expandafter\def\csname tpsd@sdt_ad2\endcsname{41.2$\pm$0.7}
\expandafter\def\csname tpn@sdt_ad2\endcsname{3}
\expandafter\def\csname tpsec@sdt_ad2\endcsname{0.02}
\expandafter\def\csname tpnfe@sdt_ad2\endcsname{2}
\expandafter\def\csname tpfid@sdt_ad2\endcsname{50.9}
\expandafter\def\csname tprec@sdt_ad2\endcsname{0.19}
\expandafter\def\csname tp@sdt_coco\endcsname{42.4}
\expandafter\def\csname tpsd@sdt_coco\endcsname{42.4$\pm$1.3}
\expandafter\def\csname tpn@sdt_coco\endcsname{3}
\expandafter\def\csname tpsec@sdt_coco\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_coco\endcsname{3}
\expandafter\def\csname tpfid@sdt_coco\endcsname{30.0}
\expandafter\def\csname tprec@sdt_coco\endcsname{0.17}
\expandafter\def\csname tp@sdt_or15_d3\endcsname{32.5}
\expandafter\def\csname tpsd@sdt_or15_d3\endcsname{32.5$\pm$0.8}
\expandafter\def\csname tpn@sdt_or15_d3\endcsname{3}
\expandafter\def\csname tpsec@sdt_or15_d3\endcsname{0.07}
\expandafter\def\csname tpnfe@sdt_or15_d3\endcsname{18}
\expandafter\def\csname tpfid@sdt_or15_d3\endcsname{30.7}
\expandafter\def\csname tprec@sdt_or15_d3\endcsname{0.06}
\expandafter\def\csname tp@sdt_or30_d2\endcsname{47.1}
\expandafter\def\csname tpsd@sdt_or30_d2\endcsname{47.1$\pm$0.2}
\expandafter\def\csname tpn@sdt_or30_d2\endcsname{3}
\expandafter\def\csname tpsec@sdt_or30_d2\endcsname{0.11}
\expandafter\def\csname tpnfe@sdt_or30_d2\endcsname{32}
\expandafter\def\csname tpfid@sdt_or30_d2\endcsname{28.6}
\expandafter\def\csname tprec@sdt_or30_d2\endcsname{0.23}
\expandafter\def\csname tp@sdt_or30_d2_g2\endcsname{44.8}
\expandafter\def\csname tpsd@sdt_or30_d2_g2\endcsname{44.8$\pm$0.8}
\expandafter\def\csname tpn@sdt_or30_d2_g2\endcsname{3}
\expandafter\def\csname tpsec@sdt_or30_d2_g2\endcsname{0.20}
\expandafter\def\csname tpnfe@sdt_or30_d2_g2\endcsname{62}
\expandafter\def\csname tpfid@sdt_or30_d2_g2\endcsname{24.8}
\expandafter\def\csname tprec@sdt_or30_d2_g2\endcsname{0.17}
\expandafter\def\csname tp@sdt_or30_d2_g75\endcsname{30.5}
\expandafter\def\csname tpsd@sdt_or30_d2_g75\endcsname{30.5$\pm$0.3}
\expandafter\def\csname tpn@sdt_or30_d2_g75\endcsname{3}
\expandafter\def\csname tpsec@sdt_or30_d2_g75\endcsname{0.20}
\expandafter\def\csname tpnfe@sdt_or30_d2_g75\endcsname{62}
\expandafter\def\csname tpfid@sdt_or30_d2_g75\endcsname{29.1}
\expandafter\def\csname tprec@sdt_or30_d2_g75\endcsname{0.05}
\expandafter\def\csname tp@sdt_or45_d1\endcsname{49.7}
\expandafter\def\csname tpsd@sdt_or45_d1\endcsname{49.7$\pm$0.6}
\expandafter\def\csname tpn@sdt_or45_d1\endcsname{3}
\expandafter\def\csname tpsec@sdt_or45_d1\endcsname{0.15}
\expandafter\def\csname tpnfe@sdt_or45_d1\endcsname{46}
\expandafter\def\csname tpfid@sdt_or45_d1\endcsname{36.8}
\expandafter\def\csname tprec@sdt_or45_d1\endcsname{0.39}
\expandafter\def\csname tp@sdt_sft\endcsname{14.4}
\expandafter\def\csname tpsd@sdt_sft\endcsname{14.4$\pm$0.7}
\expandafter\def\csname tpn@sdt_sft\endcsname{3}
\expandafter\def\csname tpsec@sdt_sft\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_sft\endcsname{3}
\expandafter\def\csname tpfid@sdt_sft\endcsname{51.0}
\expandafter\def\csname tprec@sdt_sft\endcsname{0.02}
\expandafter\def\csname tp@sdt_skip2\endcsname{16.8}
\expandafter\def\csname tpsd@sdt_skip2\endcsname{16.8$\pm$0.5}
\expandafter\def\csname tpn@sdt_skip2\endcsname{3}
\expandafter\def\csname tpsec@sdt_skip2\endcsname{0.02}
\expandafter\def\csname tpnfe@sdt_skip2\endcsname{2}
\expandafter\def\csname tpfid@sdt_skip2\endcsname{37.3}
\expandafter\def\csname tprec@sdt_skip2\endcsname{0.00}
\expandafter\def\csname tp@sdt_skip3\endcsname{15.9}
\expandafter\def\csname tpsd@sdt_skip3\endcsname{15.9$\pm$0.6}
\expandafter\def\csname tpn@sdt_skip3\endcsname{3}
\expandafter\def\csname tpsec@sdt_skip3\endcsname{0.03}
\expandafter\def\csname tpnfe@sdt_skip3\endcsname{3}
\expandafter\def\csname tpfid@sdt_skip3\endcsname{38.7}
\expandafter\def\csname tprec@sdt_skip3\endcsname{0.01}
\expandafter\def\csname tp@sdxl\endcsname{27.2}
\expandafter\def\csname tpsd@sdxl\endcsname{27.2$\pm$0.6}
\expandafter\def\csname tpn@sdxl\endcsname{3}
\expandafter\def\csname tpsec@sdxl\endcsname{1.29}
\expandafter\def\csname tpnfe@sdxl\endcsname{60}
\expandafter\def\csname tpfid@sdxl\endcsname{27.4}
\expandafter\def\csname tprec@sdxl\endcsname{0.03}
\expandafter\def\csname tp@sdxl_dmd2\endcsname{18.1}
\expandafter\def\csname tpsd@sdxl_dmd2\endcsname{18.1$\pm$0.4}
\expandafter\def\csname tpn@sdxl_dmd2\endcsname{3}
\expandafter\def\csname tpsec@sdxl_dmd2\endcsname{0.17}
\expandafter\def\csname tpnfe@sdxl_dmd2\endcsname{4}
\expandafter\def\csname tpfid@sdxl_dmd2\endcsname{38.7}
\expandafter\def\csname tprec@sdxl_dmd2\endcsname{0.02}
\expandafter\def\csname tp@sdxl_dmd2_dd\endcsname{22.9}
\expandafter\def\csname tpsd@sdxl_dmd2_dd\endcsname{22.9$\pm$0.3}
\expandafter\def\csname tpn@sdxl_dmd2_dd\endcsname{3}
\expandafter\def\csname tpsec@sdxl_dmd2_dd\endcsname{0.17}
\expandafter\def\csname tpnfe@sdxl_dmd2_dd\endcsname{4}
\expandafter\def\csname tpfid@sdxl_dmd2_dd\endcsname{29.4}
\expandafter\def\csname tprec@sdxl_dmd2_dd\endcsname{0.02}
\expandafter\def\csname tp@sdxl_dmd2_dd1_g2\endcsname{23.7}
\expandafter\def\csname tpsd@sdxl_dmd2_dd1_g2\endcsname{23.7$\pm$0.4}
\expandafter\def\csname tpn@sdxl_dmd2_dd1_g2\endcsname{3}
\expandafter\def\csname tpsec@sdxl_dmd2_dd1_g2\endcsname{0.19}
\expandafter\def\csname tpnfe@sdxl_dmd2_dd1_g2\endcsname{5}
\expandafter\def\csname tpfid@sdxl_dmd2_dd1_g2\endcsname{30.4}
\expandafter\def\csname tprec@sdxl_dmd2_dd1_g2\endcsname{0.03}
\expandafter\def\csname tp@sdxl_dmd2_dd2\endcsname{13.8}
\expandafter\def\csname tpsd@sdxl_dmd2_dd2\endcsname{13.8$\pm$1.3}
\expandafter\def\csname tpn@sdxl_dmd2_dd2\endcsname{3}
\expandafter\def\csname tpsec@sdxl_dmd2_dd2\endcsname{0.17}
\expandafter\def\csname tpnfe@sdxl_dmd2_dd2\endcsname{4}
\expandafter\def\csname tpfid@sdxl_dmd2_dd2\endcsname{28.7}
\expandafter\def\csname tprec@sdxl_dmd2_dd2\endcsname{0.05}
\expandafter\def\csname tp@sdxl_dmd2_dd2_g2\endcsname{19.7}
\expandafter\def\csname tpsd@sdxl_dmd2_dd2_g2\endcsname{19.7$\pm$0.9}
\expandafter\def\csname tpn@sdxl_dmd2_dd2_g2\endcsname{3}
\expandafter\def\csname tpsec@sdxl_dmd2_dd2_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@sdxl_dmd2_dd2_g2\endcsname{6}
\expandafter\def\csname tpfid@sdxl_dmd2_dd2_g2\endcsname{27.4}
\expandafter\def\csname tprec@sdxl_dmd2_dd2_g2\endcsname{0.05}
\expandafter\def\csname tp@sdxl_g2\endcsname{32.0}
\expandafter\def\csname tpsd@sdxl_g2\endcsname{32.0$\pm$1.3}
\expandafter\def\csname tpn@sdxl_g2\endcsname{3}
\expandafter\def\csname tpsec@sdxl_g2\endcsname{1.28}
\expandafter\def\csname tpnfe@sdxl_g2\endcsname{60}
\expandafter\def\csname tpfid@sdxl_g2\endcsname{23.2}
\expandafter\def\csname tprec@sdxl_g2\endcsname{0.13}
\expandafter\def\csname tp@sdxl_g5\endcsname{28.6}
\expandafter\def\csname tpsd@sdxl_g5\endcsname{28.6$\pm$0.3}
\expandafter\def\csname tpn@sdxl_g5\endcsname{3}
\expandafter\def\csname tpsec@sdxl_g5\endcsname{1.26}
\expandafter\def\csname tpnfe@sdxl_g5\endcsname{60}
\expandafter\def\csname tpfid@sdxl_g5\endcsname{25.2}
\expandafter\def\csname tprec@sdxl_g5\endcsname{0.05}
\expandafter\def\csname tp@sdxl_lcm\endcsname{18.1}
\expandafter\def\csname tpsd@sdxl_lcm\endcsname{18.1$\pm$0.2}
\expandafter\def\csname tpn@sdxl_lcm\endcsname{3}
\expandafter\def\csname tpsec@sdxl_lcm\endcsname{0.17}
\expandafter\def\csname tpnfe@sdxl_lcm\endcsname{4}
\expandafter\def\csname tpfid@sdxl_lcm\endcsname{28.5}
\expandafter\def\csname tprec@sdxl_lcm\endcsname{0.04}
\expandafter\def\csname tp@sdxl_lcm_g1\endcsname{19.6}
\expandafter\def\csname tpsd@sdxl_lcm_g1\endcsname{19.6$\pm$0.4}
\expandafter\def\csname tpn@sdxl_lcm_g1\endcsname{3}
\expandafter\def\csname tpsec@sdxl_lcm_g1\endcsname{0.17}
\expandafter\def\csname tpnfe@sdxl_lcm_g1\endcsname{4}
\expandafter\def\csname tpfid@sdxl_lcm_g1\endcsname{27.7}
\expandafter\def\csname tprec@sdxl_lcm_g1\endcsname{0.04}
\expandafter\def\csname tp@sdxl_lcm_g3\endcsname{18.1}
\expandafter\def\csname tpsd@sdxl_lcm_g3\endcsname{18.1$\pm$0.7}
\expandafter\def\csname tpn@sdxl_lcm_g3\endcsname{3}
\expandafter\def\csname tpsec@sdxl_lcm_g3\endcsname{0.17}
\expandafter\def\csname tpnfe@sdxl_lcm_g3\endcsname{4}
\expandafter\def\csname tpfid@sdxl_lcm_g3\endcsname{28.6}
\expandafter\def\csname tprec@sdxl_lcm_g3\endcsname{0.04}
\expandafter\def\csname tp@sdxl_lightning\endcsname{20.2}
\expandafter\def\csname tpsd@sdxl_lightning\endcsname{20.2$\pm$0.2}
\expandafter\def\csname tpn@sdxl_lightning\endcsname{3}
\expandafter\def\csname tpsec@sdxl_lightning\endcsname{0.17}
\expandafter\def\csname tpnfe@sdxl_lightning\endcsname{4}
\expandafter\def\csname tpfid@sdxl_lightning\endcsname{32.7}
\expandafter\def\csname tprec@sdxl_lightning\endcsname{0.01}
\expandafter\def\csname tp@sdxl_turbo\endcsname{12.9}
\expandafter\def\csname tpsd@sdxl_turbo\endcsname{12.9$\pm$0.5}
\expandafter\def\csname tpn@sdxl_turbo\endcsname{3}
\expandafter\def\csname tpsec@sdxl_turbo\endcsname{0.03}
\expandafter\def\csname tpnfe@sdxl_turbo\endcsname{1}
\expandafter\def\csname tpfid@sdxl_turbo\endcsname{42.9}
\expandafter\def\csname tprec@sdxl_turbo\endcsname{0.00}
\expandafter\def\csname tp@srpo\endcsname{15.7}
\expandafter\def\csname tpsd@srpo\endcsname{15.7$\pm$0.3}
\expandafter\def\csname tpn@srpo\endcsname{3}
\expandafter\def\csname tpsec@srpo\endcsname{1.68}
\expandafter\def\csname tpnfe@srpo\endcsname{28}
\expandafter\def\csname tpfid@srpo\endcsname{40.4}
\expandafter\def\csname tprec@srpo\endcsname{0.04}
\expandafter\def\csname tp@srpo_g2\endcsname{19.9}
\expandafter\def\csname tpsd@srpo_g2\endcsname{19.9$\pm$0.6}
\expandafter\def\csname tpn@srpo_g2\endcsname{3}
\expandafter\def\csname tpsec@srpo_g2\endcsname{1.66}
\expandafter\def\csname tpnfe@srpo_g2\endcsname{28}
\expandafter\def\csname tpfid@srpo_g2\endcsname{36.0}
\expandafter\def\csname tprec@srpo_g2\endcsname{0.07}
\expandafter\def\csname tp@tin200_dpdmd\endcsname{15.3}
\expandafter\def\csname tpsd@tin200_dpdmd\endcsname{15.3$\pm$0.3}
\expandafter\def\csname tpn@tin200_dpdmd\endcsname{3}
\expandafter\def\csname tpsec@tin200_dpdmd\endcsname{0.07}
\expandafter\def\csname tpnfe@tin200_dpdmd\endcsname{4}
\expandafter\def\csname tp@tin200_dpdmd_ad0\endcsname{24.2}
\expandafter\def\csname tpsd@tin200_dpdmd_ad0\endcsname{24.2$\pm$0.1}
\expandafter\def\csname tpn@tin200_dpdmd_ad0\endcsname{3}
\expandafter\def\csname tpsec@tin200_dpdmd_ad0\endcsname{0.08}
\expandafter\def\csname tpnfe@tin200_dpdmd_ad0\endcsname{4}
\expandafter\def\csname tp@tin200_dpdmd_dd1_g1\endcsname{17.5}
\expandafter\def\csname tpsd@tin200_dpdmd_dd1_g1\endcsname{17.5$\pm$0.4}
\expandafter\def\csname tpn@tin200_dpdmd_dd1_g1\endcsname{3}
\expandafter\def\csname tpsec@tin200_dpdmd_dd1_g1\endcsname{0.08}
\expandafter\def\csname tpnfe@tin200_dpdmd_dd1_g1\endcsname{4}
\expandafter\def\csname tp@tin200_kb_dd2_g1\endcsname{43.7}
\expandafter\def\csname tpsd@tin200_kb_dd2_g1\endcsname{43.7$\pm$0.1}
\expandafter\def\csname tpn@tin200_kb_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@tin200_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@tin200_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tp@tin200_kb_g1\endcsname{48.2}
\expandafter\def\csname tpsd@tin200_kb_g1\endcsname{48.2$\pm$0.1}
\expandafter\def\csname tpn@tin200_kb_g1\endcsname{3}
\expandafter\def\csname tpsec@tin200_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@tin200_kb_g1\endcsname{50}
\expandafter\def\csname tp@tin200_kd_ad1\endcsname{47.9}
\expandafter\def\csname tpsd@tin200_kd_ad1\endcsname{47.9$\pm$0.4}
\expandafter\def\csname tpn@tin200_kd_ad1\endcsname{3}
\expandafter\def\csname tpsec@tin200_kd_ad1\endcsname{0.12}
\expandafter\def\csname tpnfe@tin200_kd_ad1\endcsname{3}
\expandafter\def\csname tp@tin200_kd_ad2\endcsname{48.6}
\expandafter\def\csname tpsd@tin200_kd_ad2\endcsname{48.6$\pm$0.3}
\expandafter\def\csname tpn@tin200_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@tin200_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@tin200_kd_ad2\endcsname{2}
\expandafter\def\csname tp@tin200_kd_ad2_tg4\endcsname{23.2}
\expandafter\def\csname tpsd@tin200_kd_ad2_tg4\endcsname{23.2$\pm$0.2}
\expandafter\def\csname tpn@tin200_kd_ad2_tg4\endcsname{3}
\expandafter\def\csname tpsec@tin200_kd_ad2_tg4\endcsname{0.10}
\expandafter\def\csname tpnfe@tin200_kd_ad2_tg4\endcsname{2}
\expandafter\def\csname tp@tin200_kd_coco\endcsname{48.5}
\expandafter\def\csname tpsd@tin200_kd_coco\endcsname{48.5$\pm$0.2}
\expandafter\def\csname tpn@tin200_kd_coco\endcsname{3}
\expandafter\def\csname tpsec@tin200_kd_coco\endcsname{0.10}
\expandafter\def\csname tpnfe@tin200_kd_coco\endcsname{2}
\expandafter\def\csname tp@tin200_kd_mono4_g32\endcsname{32.1}
\expandafter\def\csname tpsd@tin200_kd_mono4_g32\endcsname{32.1$\pm$0.3}
\expandafter\def\csname tpn@tin200_kd_mono4_g32\endcsname{3}
\expandafter\def\csname tpsec@tin200_kd_mono4_g32\endcsname{0.63}
\expandafter\def\csname tpnfe@tin200_kd_mono4_g32\endcsname{7.87}
\expandafter\def\csname tp@tin200_klein\endcsname{19.1}
\expandafter\def\csname tpsd@tin200_klein\endcsname{19.1$\pm$0.0}
\expandafter\def\csname tpn@tin200_klein\endcsname{3}
\expandafter\def\csname tpsec@tin200_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@tin200_klein\endcsname{4}
\expandafter\def\csname tp@tin200_klein_base\endcsname{27.0}
\expandafter\def\csname tpsd@tin200_klein_base\endcsname{27.0$\pm$0.2}
\expandafter\def\csname tpn@tin200_klein_base\endcsname{3}
\expandafter\def\csname tpsec@tin200_klein_base\endcsname{2.77}
\expandafter\def\csname tpnfe@tin200_klein_base\endcsname{100}
\expandafter\def\csname tp@tin200_real500\endcsname{75.5}
\expandafter\def\csname tpsd@tin200_real500\endcsname{75.5$\pm$0.1}
\expandafter\def\csname tpn@tin200_real500\endcsname{3}
\expandafter\def\csname tp@tin200_sd15\endcsname{34.9}
\expandafter\def\csname tpsd@tin200_sd15\endcsname{34.9$\pm$0.6}
\expandafter\def\csname tpn@tin200_sd15\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd15\endcsname{0.21}
\expandafter\def\csname tpnfe@tin200_sd15\endcsname{60}
\expandafter\def\csname tp@tin200_sd15_bare_g2\endcsname{48.5}
\expandafter\def\csname tpsd@tin200_sd15_bare_g2\endcsname{48.5$\pm$0.2}
\expandafter\def\csname tpn@tin200_sd15_bare_g2\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd15_bare_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@tin200_sd15_bare_g2\endcsname{60}
\expandafter\def\csname tp@tin200_sd15_g2\endcsname{52.0}
\expandafter\def\csname tpsd@tin200_sd15_g2\endcsname{52.0$\pm$0.4}
\expandafter\def\csname tpn@tin200_sd15_g2\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@tin200_sd15_g2\endcsname{60}
\expandafter\def\csname tp@tin200_sd21\endcsname{31.5}
\expandafter\def\csname tpsd@tin200_sd21\endcsname{31.5$\pm$0.3}
\expandafter\def\csname tpn@tin200_sd21\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd21\endcsname{0.20}
\expandafter\def\csname tpnfe@tin200_sd21\endcsname{60}
\expandafter\def\csname tp@tin200_sd21_cfg_late\endcsname{48.6}
\expandafter\def\csname tpsd@tin200_sd21_cfg_late\endcsname{48.6$\pm$1.8}
\expandafter\def\csname tpn@tin200_sd21_cfg_late\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd21_cfg_late\endcsname{0.16}
\expandafter\def\csname tpnfe@tin200_sd21_cfg_late\endcsname{45}
\expandafter\def\csname tp@tin200_sd21_g1\endcsname{45.7}
\expandafter\def\csname tpsd@tin200_sd21_g1\endcsname{45.7$\pm$0.9}
\expandafter\def\csname tpn@tin200_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@tin200_sd21_g1\endcsname{30}
\expandafter\def\csname tp@tin200_sd21_g2\endcsname{48.3}
\expandafter\def\csname tpsd@tin200_sd21_g2\endcsname{48.3$\pm$0.4}
\expandafter\def\csname tpn@tin200_sd21_g2\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd21_g2\endcsname{0.20}
\expandafter\def\csname tpnfe@tin200_sd21_g2\endcsname{60}
\expandafter\def\csname tp@tin200_sd35_large\endcsname{23.0}
\expandafter\def\csname tpsd@tin200_sd35_large\endcsname{23.0$\pm$0.3}
\expandafter\def\csname tpn@tin200_sd35_large\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35_large\endcsname{1.42}
\expandafter\def\csname tpnfe@tin200_sd35_large\endcsname{56}
\expandafter\def\csname tp@tin200_sd35_large_bare\endcsname{20.8}
\expandafter\def\csname tpsd@tin200_sd35_large_bare\endcsname{20.8$\pm$0.2}
\expandafter\def\csname tpn@tin200_sd35_large_bare\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35_large_bare\endcsname{1.42}
\expandafter\def\csname tpnfe@tin200_sd35_large_bare\endcsname{56}
\expandafter\def\csname tp@tin200_sd35_large_g1\endcsname{34.6}
\expandafter\def\csname tpsd@tin200_sd35_large_g1\endcsname{34.6$\pm$0.5}
\expandafter\def\csname tpn@tin200_sd35_large_g1\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35_large_g1\endcsname{0.74}
\expandafter\def\csname tpnfe@tin200_sd35_large_g1\endcsname{28}
\expandafter\def\csname tp@tin200_sd35_turbo\endcsname{19.4}
\expandafter\def\csname tpsd@tin200_sd35_turbo\endcsname{19.4$\pm$0.3}
\expandafter\def\csname tpn@tin200_sd35_turbo\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35_turbo\endcsname{0.13}
\expandafter\def\csname tpnfe@tin200_sd35_turbo\endcsname{4}
\expandafter\def\csname tp@tin200_sd35_turbo_bare\endcsname{16.3}
\expandafter\def\csname tpsd@tin200_sd35_turbo_bare\endcsname{16.3$\pm$0.4}
\expandafter\def\csname tpn@tin200_sd35_turbo_bare\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35_turbo_bare\endcsname{0.13}
\expandafter\def\csname tpnfe@tin200_sd35_turbo_bare\endcsname{4}
\expandafter\def\csname tp@tin200_sd35m\endcsname{25.1}
\expandafter\def\csname tpsd@tin200_sd35m\endcsname{25.1$\pm$0.4}
\expandafter\def\csname tpn@tin200_sd35m\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35m\endcsname{0.61}
\expandafter\def\csname tpnfe@tin200_sd35m\endcsname{56}
\expandafter\def\csname tp@tin200_sd35m_g1\endcsname{44.7}
\expandafter\def\csname tpsd@tin200_sd35m_g1\endcsname{44.7$\pm$0.4}
\expandafter\def\csname tpn@tin200_sd35m_g1\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35m_g1\endcsname{0.32}
\expandafter\def\csname tpnfe@tin200_sd35m_g1\endcsname{28}
\expandafter\def\csname tp@tin200_sd35t_ad0\endcsname{32.1}
\expandafter\def\csname tpsd@tin200_sd35t_ad0\endcsname{32.1$\pm$0.5}
\expandafter\def\csname tpn@tin200_sd35t_ad0\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35t_ad0\endcsname{0.14}
\expandafter\def\csname tpnfe@tin200_sd35t_ad0\endcsname{4}
\expandafter\def\csname tp@tin200_sd35t_ad0_tg35\endcsname{17.3}
\expandafter\def\csname tpsd@tin200_sd35t_ad0_tg35\endcsname{17.3$\pm$0.2}
\expandafter\def\csname tpn@tin200_sd35t_ad0_tg35\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35t_ad0_tg35\endcsname{0.14}
\expandafter\def\csname tpnfe@tin200_sd35t_ad0_tg35\endcsname{4}
\expandafter\def\csname tp@tin200_sd35t_ad1\endcsname{23.6}
\expandafter\def\csname tpsd@tin200_sd35t_ad1\endcsname{23.6$\pm$0.2}
\expandafter\def\csname tpn@tin200_sd35t_ad1\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35t_ad1\endcsname{0.12}
\expandafter\def\csname tpnfe@tin200_sd35t_ad1\endcsname{3}
\expandafter\def\csname tp@tin200_sd35t_dd1_g1\endcsname{26.9}
\expandafter\def\csname tpsd@tin200_sd35t_dd1_g1\endcsname{26.9$\pm$0.1}
\expandafter\def\csname tpn@tin200_sd35t_dd1_g1\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35t_dd1_g1\endcsname{0.14}
\expandafter\def\csname tpnfe@tin200_sd35t_dd1_g1\endcsname{4}
\expandafter\def\csname tp@tin200_sd35t_dd2_g1\endcsname{21.5}
\expandafter\def\csname tpsd@tin200_sd35t_dd2_g1\endcsname{21.5$\pm$0.8}
\expandafter\def\csname tpn@tin200_sd35t_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd35t_dd2_g1\endcsname{0.14}
\expandafter\def\csname tpnfe@tin200_sd35t_dd2_g1\endcsname{4}
\expandafter\def\csname tp@tin200_sd_turbo\endcsname{18.2}
\expandafter\def\csname tpsd@tin200_sd_turbo\endcsname{18.2$\pm$0.1}
\expandafter\def\csname tpn@tin200_sd_turbo\endcsname{3}
\expandafter\def\csname tpsec@tin200_sd_turbo\endcsname{0.02}
\expandafter\def\csname tpnfe@tin200_sd_turbo\endcsname{1}
\expandafter\def\csname tp@tin200_sdt4\endcsname{19.8}
\expandafter\def\csname tpsd@tin200_sdt4\endcsname{19.8$\pm$0.3}
\expandafter\def\csname tpn@tin200_sdt4\endcsname{3}
\expandafter\def\csname tpsec@tin200_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@tin200_sdt4\endcsname{4}
\expandafter\def\csname tp@tin200_sdt4_dd2_g1\endcsname{36.0}
\expandafter\def\csname tpsd@tin200_sdt4_dd2_g1\endcsname{36.0$\pm$0.2}
\expandafter\def\csname tpn@tin200_sdt4_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@tin200_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@tin200_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tp@tin200_sdt_ad1\endcsname{41.3}
\expandafter\def\csname tpsd@tin200_sdt_ad1\endcsname{41.3$\pm$0.8}
\expandafter\def\csname tpn@tin200_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@tin200_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@tin200_sdt_ad1\endcsname{3}
\expandafter\def\csname tp@tin200_sdt_ad1_tg75\endcsname{32.6}
\expandafter\def\csname tpsd@tin200_sdt_ad1_tg75\endcsname{32.6$\pm$0.3}
\expandafter\def\csname tpn@tin200_sdt_ad1_tg75\endcsname{3}
\expandafter\def\csname tpsec@tin200_sdt_ad1_tg75\endcsname{0.03}
\expandafter\def\csname tpnfe@tin200_sdt_ad1_tg75\endcsname{3}
\expandafter\def\csname tp@tin200_sdt_ad2\endcsname{36.3}
\expandafter\def\csname tpsd@tin200_sdt_ad2\endcsname{36.3$\pm$0.7}
\expandafter\def\csname tpn@tin200_sdt_ad2\endcsname{3}
\expandafter\def\csname tpsec@tin200_sdt_ad2\endcsname{0.03}
\expandafter\def\csname tpnfe@tin200_sdt_ad2\endcsname{2}
\expandafter\def\csname tp@tin200_sdt_coco\endcsname{41.0}
\expandafter\def\csname tpsd@tin200_sdt_coco\endcsname{41.0$\pm$1.0}
\expandafter\def\csname tpn@tin200_sdt_coco\endcsname{3}
\expandafter\def\csname tpsec@tin200_sdt_coco\endcsname{0.03}
\expandafter\def\csname tpnfe@tin200_sdt_coco\endcsname{3}
\expandafter\def\csname tp@tin200_sdxl\endcsname{28.8}
\expandafter\def\csname tpsd@tin200_sdxl\endcsname{28.8$\pm$0.4}
\expandafter\def\csname tpn@tin200_sdxl\endcsname{3}
\expandafter\def\csname tpsec@tin200_sdxl\endcsname{1.27}
\expandafter\def\csname tpnfe@tin200_sdxl\endcsname{60}
\expandafter\def\csname tp@tin200_sdxl_g5\endcsname{29.7}
\expandafter\def\csname tpsd@tin200_sdxl_g5\endcsname{29.7$\pm$0.3}
\expandafter\def\csname tpn@tin200_sdxl_g5\endcsname{3}
\expandafter\def\csname tpsec@tin200_sdxl_g5\endcsname{1.27}
\expandafter\def\csname tpnfe@tin200_sdxl_g5\endcsname{60}
\expandafter\def\csname tp@tin200_sdxl_turbo\endcsname{15.0}
\expandafter\def\csname tpsd@tin200_sdxl_turbo\endcsname{15.0$\pm$0.3}
\expandafter\def\csname tpn@tin200_sdxl_turbo\endcsname{3}
\expandafter\def\csname tpsec@tin200_sdxl_turbo\endcsname{0.03}
\expandafter\def\csname tpnfe@tin200_sdxl_turbo\endcsname{1}
\expandafter\def\csname tp@tin200_zimage_turbo\endcsname{13.9}
\expandafter\def\csname tpsd@tin200_zimage_turbo\endcsname{13.9$\pm$0.4}
\expandafter\def\csname tpn@tin200_zimage_turbo\endcsname{3}
\expandafter\def\csname tpsec@tin200_zimage_turbo\endcsname{0.37}
\expandafter\def\csname tpnfe@tin200_zimage_turbo\endcsname{9}
\expandafter\def\csname tp@tin200_zt_ad1\endcsname{34.2}
\expandafter\def\csname tpsd@tin200_zt_ad1\endcsname{34.2$\pm$0.6}
\expandafter\def\csname tpn@tin200_zt_ad1\endcsname{3}
\expandafter\def\csname tpsec@tin200_zt_ad1\endcsname{0.33}
\expandafter\def\csname tpnfe@tin200_zt_ad1\endcsname{8}
\expandafter\def\csname tp@tin200_zt_ad2\endcsname{38.2}
\expandafter\def\csname tpsd@tin200_zt_ad2\endcsname{38.2$\pm$0.3}
\expandafter\def\csname tpn@tin200_zt_ad2\endcsname{3}
\expandafter\def\csname tpsec@tin200_zt_ad2\endcsname{0.29}
\expandafter\def\csname tpnfe@tin200_zt_ad2\endcsname{7}
\expandafter\def\csname tp@tin200_zt_ad2_tg5\endcsname{20.1}
\expandafter\def\csname tpsd@tin200_zt_ad2_tg5\endcsname{20.1$\pm$0.1}
\expandafter\def\csname tpn@tin200_zt_ad2_tg5\endcsname{3}
\expandafter\def\csname tpsec@tin200_zt_ad2_tg5\endcsname{0.30}
\expandafter\def\csname tpnfe@tin200_zt_ad2_tg5\endcsname{7}
\expandafter\def\csname tp@tin200_zt_dd3_g1\endcsname{35.3}
\expandafter\def\csname tpsd@tin200_zt_dd3_g1\endcsname{35.3$\pm$0.3}
\expandafter\def\csname tpn@tin200_zt_dd3_g1\endcsname{3}
\expandafter\def\csname tpsec@tin200_zt_dd3_g1\endcsname{0.37}
\expandafter\def\csname tpnfe@tin200_zt_dd3_g1\endcsname{9}
\expandafter\def\csname tp@vits_kb_dd2_g1\endcsname{26.6}
\expandafter\def\csname tpsd@vits_kb_dd2_g1\endcsname{26.6$\pm$0.1}
\expandafter\def\csname tpn@vits_kb_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@vits_kb_dd2_g1\endcsname{0.15}
\expandafter\def\csname tpnfe@vits_kb_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@vits_kb_dd2_g1\endcsname{29.9}
\expandafter\def\csname tprec@vits_kb_dd2_g1\endcsname{0.17}
\expandafter\def\csname tp@vits_kb_g1\endcsname{25.4}
\expandafter\def\csname tpsd@vits_kb_g1\endcsname{25.4$\pm$0.2}
\expandafter\def\csname tpn@vits_kb_g1\endcsname{3}
\expandafter\def\csname tpsec@vits_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@vits_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@vits_kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@vits_kb_g1\endcsname{0.49}
\expandafter\def\csname tp@vits_kd_ad2\endcsname{26.9}
\expandafter\def\csname tpsd@vits_kd_ad2\endcsname{26.9$\pm$0.5}
\expandafter\def\csname tpn@vits_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@vits_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@vits_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@vits_kd_ad2\endcsname{34.8}
\expandafter\def\csname tprec@vits_kd_ad2\endcsname{0.28}
\expandafter\def\csname tp@vits_klein\endcsname{15.6}
\expandafter\def\csname tpsd@vits_klein\endcsname{15.6$\pm$0.1}
\expandafter\def\csname tpn@vits_klein\endcsname{3}
\expandafter\def\csname tpsec@vits_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@vits_klein\endcsname{4}
\expandafter\def\csname tpfid@vits_klein\endcsname{47.6}
\expandafter\def\csname tprec@vits_klein\endcsname{0.01}
\expandafter\def\csname tp@vits_klein_base\endcsname{21.1}
\expandafter\def\csname tpsd@vits_klein_base\endcsname{21.1$\pm$0.7}
\expandafter\def\csname tpn@vits_klein_base\endcsname{3}
\expandafter\def\csname tpsec@vits_klein_base\endcsname{2.82}
\expandafter\def\csname tpnfe@vits_klein_base\endcsname{100}
\expandafter\def\csname tpfid@vits_klein_base\endcsname{42.6}
\expandafter\def\csname tprec@vits_klein_base\endcsname{0.04}
\expandafter\def\csname tp@vits_real500\endcsname{53.8}
\expandafter\def\csname tpsd@vits_real500\endcsname{53.8$\pm$0.4}
\expandafter\def\csname tpn@vits_real500\endcsname{3}
\expandafter\def\csname tp@vits_sd15\endcsname{23.1}
\expandafter\def\csname tpsd@vits_sd15\endcsname{23.1$\pm$0.2}
\expandafter\def\csname tpn@vits_sd15\endcsname{3}
\expandafter\def\csname tpsec@vits_sd15\endcsname{0.21}
\expandafter\def\csname tpnfe@vits_sd15\endcsname{60}
\expandafter\def\csname tpfid@vits_sd15\endcsname{26.6}
\expandafter\def\csname tprec@vits_sd15\endcsname{0.06}
\expandafter\def\csname tp@vits_sd15_g2\endcsname{31.6}
\expandafter\def\csname tpsd@vits_sd15_g2\endcsname{31.6$\pm$0.6}
\expandafter\def\csname tpn@vits_sd15_g2\endcsname{3}
\expandafter\def\csname tpsec@vits_sd15_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@vits_sd15_g2\endcsname{60}
\expandafter\def\csname tpfid@vits_sd15_g2\endcsname{25.3}
\expandafter\def\csname tprec@vits_sd15_g2\endcsname{0.31}
\expandafter\def\csname tp@vits_sd21_g1\endcsname{22.9}
\expandafter\def\csname tpsd@vits_sd21_g1\endcsname{22.9$\pm$0.2}
\expandafter\def\csname tpn@vits_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@vits_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@vits_sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@vits_sd21_g1\endcsname{50.2}
\expandafter\def\csname tprec@vits_sd21_g1\endcsname{0.33}
\expandafter\def\csname tp@vits_sdt4\endcsname{13.8}
\expandafter\def\csname tpsd@vits_sdt4\endcsname{13.8$\pm$0.4}
\expandafter\def\csname tpn@vits_sdt4\endcsname{3}
\expandafter\def\csname tpsec@vits_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@vits_sdt4\endcsname{4}
\expandafter\def\csname tpfid@vits_sdt4\endcsname{37.5}
\expandafter\def\csname tprec@vits_sdt4\endcsname{0.02}
\expandafter\def\csname tp@vits_sdt4_dd2_g1\endcsname{24.5}
\expandafter\def\csname tpsd@vits_sdt4_dd2_g1\endcsname{24.5$\pm$0.9}
\expandafter\def\csname tpn@vits_sdt4_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@vits_sdt4_dd2_g1\endcsname{0.03}
\expandafter\def\csname tpnfe@vits_sdt4_dd2_g1\endcsname{4}
\expandafter\def\csname tpfid@vits_sdt4_dd2_g1\endcsname{32.1}
\expandafter\def\csname tprec@vits_sdt4_dd2_g1\endcsname{0.12}
\expandafter\def\csname tp@vits_sdt_ad1\endcsname{26.8}
\expandafter\def\csname tpsd@vits_sdt_ad1\endcsname{26.8$\pm$0.3}
\expandafter\def\csname tpn@vits_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@vits_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@vits_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@vits_sdt_ad1\endcsname{30.2}
\expandafter\def\csname tprec@vits_sdt_ad1\endcsname{0.16}
\expandafter\def\csname tp@wp_kb_g1\endcsname{41.1}
\expandafter\def\csname tpsd@wp_kb_g1\endcsname{41.1$\pm$0.5}
\expandafter\def\csname tpn@wp_kb_g1\endcsname{3}
\expandafter\def\csname tpsec@wp_kb_g1\endcsname{1.38}
\expandafter\def\csname tpnfe@wp_kb_g1\endcsname{50}
\expandafter\def\csname tpfid@wp_kb_g1\endcsname{33.0}
\expandafter\def\csname tprec@wp_kb_g1\endcsname{0.49}
\expandafter\def\csname tp@wp_kd_ad2\endcsname{39.0}
\expandafter\def\csname tpsd@wp_kd_ad2\endcsname{39.0$\pm$0.3}
\expandafter\def\csname tpn@wp_kd_ad2\endcsname{3}
\expandafter\def\csname tpsec@wp_kd_ad2\endcsname{0.10}
\expandafter\def\csname tpnfe@wp_kd_ad2\endcsname{2}
\expandafter\def\csname tpfid@wp_kd_ad2\endcsname{34.8}
\expandafter\def\csname tprec@wp_kd_ad2\endcsname{0.28}
\expandafter\def\csname tp@wp_klein\endcsname{17.9}
\expandafter\def\csname tpsd@wp_klein\endcsname{17.9$\pm$1.0}
\expandafter\def\csname tpn@wp_klein\endcsname{3}
\expandafter\def\csname tpsec@wp_klein\endcsname{0.14}
\expandafter\def\csname tpnfe@wp_klein\endcsname{4}
\expandafter\def\csname tpfid@wp_klein\endcsname{47.6}
\expandafter\def\csname tprec@wp_klein\endcsname{0.01}
\expandafter\def\csname tp@wp_real500\endcsname{68.1}
\expandafter\def\csname tpsd@wp_real500\endcsname{68.1$\pm$0.9}
\expandafter\def\csname tpn@wp_real500\endcsname{3}
\expandafter\def\csname tp@wp_sd21_g1\endcsname{39.7}
\expandafter\def\csname tpsd@wp_sd21_g1\endcsname{39.7$\pm$0.3}
\expandafter\def\csname tpn@wp_sd21_g1\endcsname{3}
\expandafter\def\csname tpsec@wp_sd21_g1\endcsname{0.11}
\expandafter\def\csname tpnfe@wp_sd21_g1\endcsname{30}
\expandafter\def\csname tpfid@wp_sd21_g1\endcsname{50.2}
\expandafter\def\csname tprec@wp_sd21_g1\endcsname{0.33}
\expandafter\def\csname tp@wp_sdt4\endcsname{21.7}
\expandafter\def\csname tpsd@wp_sdt4\endcsname{21.7$\pm$1.2}
\expandafter\def\csname tpn@wp_sdt4\endcsname{3}
\expandafter\def\csname tpsec@wp_sdt4\endcsname{0.03}
\expandafter\def\csname tpnfe@wp_sdt4\endcsname{4}
\expandafter\def\csname tpfid@wp_sdt4\endcsname{37.5}
\expandafter\def\csname tprec@wp_sdt4\endcsname{0.02}
\expandafter\def\csname tp@wp_sdt_ad1\endcsname{38.6}
\expandafter\def\csname tpsd@wp_sdt_ad1\endcsname{38.6$\pm$0.5}
\expandafter\def\csname tpn@wp_sdt_ad1\endcsname{3}
\expandafter\def\csname tpsec@wp_sdt_ad1\endcsname{0.03}
\expandafter\def\csname tpnfe@wp_sdt_ad1\endcsname{3}
\expandafter\def\csname tpfid@wp_sdt_ad1\endcsname{30.2}
\expandafter\def\csname tprec@wp_sdt_ad1\endcsname{0.16}
\expandafter\def\csname tp@wp_tin200_real500\endcsname{70.0}
\expandafter\def\csname tpsd@wp_tin200_real500\endcsname{70.0$\pm$0.7}
\expandafter\def\csname tpn@wp_tin200_real500\endcsname{3}
\expandafter\def\csname tp@wp_tin200_sd15_bare_g2\endcsname{46.1}
\expandafter\def\csname tpsd@wp_tin200_sd15_bare_g2\endcsname{46.1$\pm$0.4}
\expandafter\def\csname tpn@wp_tin200_sd15_bare_g2\endcsname{3}
\expandafter\def\csname tpsec@wp_tin200_sd15_bare_g2\endcsname{0.21}
\expandafter\def\csname tpnfe@wp_tin200_sd15_bare_g2\endcsname{60}
\expandafter\def\csname tp@wp_tin200_sd35_large_bare\endcsname{19.8}
\expandafter\def\csname tpsd@wp_tin200_sd35_large_bare\endcsname{19.8$\pm$2.9}
\expandafter\def\csname tpn@wp_tin200_sd35_large_bare\endcsname{3}
\expandafter\def\csname tpsec@wp_tin200_sd35_large_bare\endcsname{1.42}
\expandafter\def\csname tpnfe@wp_tin200_sd35_large_bare\endcsname{56}
\expandafter\def\csname tp@wp_tin200_sd35_turbo_bare\endcsname{14.9}
\expandafter\def\csname tpsd@wp_tin200_sd35_turbo_bare\endcsname{14.9$\pm$1.7}
\expandafter\def\csname tpn@wp_tin200_sd35_turbo_bare\endcsname{3}
\expandafter\def\csname tpsec@wp_tin200_sd35_turbo_bare\endcsname{0.13}
\expandafter\def\csname tpnfe@wp_tin200_sd35_turbo_bare\endcsname{4}
\expandafter\def\csname tp@wp_tin200_sdxl\endcsname{31.5}
\expandafter\def\csname tpsd@wp_tin200_sdxl\endcsname{31.5$\pm$3.0}
\expandafter\def\csname tpn@wp_tin200_sdxl\endcsname{3}
\expandafter\def\csname tpsec@wp_tin200_sdxl\endcsname{1.27}
\expandafter\def\csname tpnfe@wp_tin200_sdxl\endcsname{60}
\expandafter\def\csname tp@wp_tin200_sdxl_g5\endcsname{35.3}
\expandafter\def\csname tpsd@wp_tin200_sdxl_g5\endcsname{35.3$\pm$0.4}
\expandafter\def\csname tpn@wp_tin200_sdxl_g5\endcsname{3}
\expandafter\def\csname tpsec@wp_tin200_sdxl_g5\endcsname{1.27}
\expandafter\def\csname tpnfe@wp_tin200_sdxl_g5\endcsname{60}
\expandafter\def\csname tp@wp_tin200_sdxl_turbo\endcsname{13.1}
\expandafter\def\csname tpsd@wp_tin200_sdxl_turbo\endcsname{13.1$\pm$0.3}
\expandafter\def\csname tpn@wp_tin200_sdxl_turbo\endcsname{3}
\expandafter\def\csname tpsec@wp_tin200_sdxl_turbo\endcsname{0.03}
\expandafter\def\csname tpnfe@wp_tin200_sdxl_turbo\endcsname{1}
\expandafter\def\csname tp@zimage\endcsname{17.6}
\expandafter\def\csname tpsd@zimage\endcsname{17.6$\pm$0.3}
\expandafter\def\csname tpn@zimage\endcsname{3}
\expandafter\def\csname tpsec@zimage\endcsname{3.78}
\expandafter\def\csname tpnfe@zimage\endcsname{100}
\expandafter\def\csname tpfid@zimage\endcsname{34.6}
\expandafter\def\csname tprec@zimage\endcsname{0.03}
\expandafter\def\csname tp@zimage_g1\endcsname{45.6}
\expandafter\def\csname tpsd@zimage_g1\endcsname{45.6$\pm$0.7}
\expandafter\def\csname tpn@zimage_g1\endcsname{3}
\expandafter\def\csname tpsec@zimage_g1\endcsname{1.92}
\expandafter\def\csname tpnfe@zimage_g1\endcsname{50}
\expandafter\def\csname tpfid@zimage_g1\endcsname{29.4}
\expandafter\def\csname tprec@zimage_g1\endcsname{0.39}
\expandafter\def\csname tp@zimage_g2\endcsname{35.4}
\expandafter\def\csname tpsd@zimage_g2\endcsname{35.4$\pm$0.2}
\expandafter\def\csname tpn@zimage_g2\endcsname{3}
\expandafter\def\csname tpsec@zimage_g2\endcsname{3.76}
\expandafter\def\csname tpnfe@zimage_g2\endcsname{100}
\expandafter\def\csname tpfid@zimage_g2\endcsname{23.1}
\expandafter\def\csname tprec@zimage_g2\endcsname{0.14}
\expandafter\def\csname tp@zimage_turbo\endcsname{14.0}
\expandafter\def\csname tpsd@zimage_turbo\endcsname{14.0$\pm$0.0}
\expandafter\def\csname tpn@zimage_turbo\endcsname{3}
\expandafter\def\csname tpsec@zimage_turbo\endcsname{0.37}
\expandafter\def\csname tpnfe@zimage_turbo\endcsname{9}
\expandafter\def\csname tpfid@zimage_turbo\endcsname{56.2}
\expandafter\def\csname tprec@zimage_turbo\endcsname{0.00}
\expandafter\def\csname tp@zimage_turbo_s8\endcsname{13.8}
\expandafter\def\csname tpsd@zimage_turbo_s8\endcsname{13.8$\pm$0.4}
\expandafter\def\csname tpn@zimage_turbo_s8\endcsname{3}
\expandafter\def\csname tpsec@zimage_turbo_s8\endcsname{0.33}
\expandafter\def\csname tpnfe@zimage_turbo_s8\endcsname{8}
\expandafter\def\csname tpfid@zimage_turbo_s8\endcsname{56.6}
\expandafter\def\csname tprec@zimage_turbo_s8\endcsname{0.00}
\expandafter\def\csname tp@zt_ad1\endcsname{31.1}
\expandafter\def\csname tpsd@zt_ad1\endcsname{31.1$\pm$0.4}
\expandafter\def\csname tpn@zt_ad1\endcsname{3}
\expandafter\def\csname tpsec@zt_ad1\endcsname{0.33}
\expandafter\def\csname tpnfe@zt_ad1\endcsname{8}
\expandafter\def\csname tpfid@zt_ad1\endcsname{30.8}
\expandafter\def\csname tprec@zt_ad1\endcsname{0.05}
\expandafter\def\csname tp@zt_ad2\endcsname{35.2}
\expandafter\def\csname tpsd@zt_ad2\endcsname{35.2$\pm$0.6}
\expandafter\def\csname tpn@zt_ad2\endcsname{3}
\expandafter\def\csname tpsec@zt_ad2\endcsname{0.30}
\expandafter\def\csname tpnfe@zt_ad2\endcsname{7}
\expandafter\def\csname tpfid@zt_ad2\endcsname{24.9}
\expandafter\def\csname tprec@zt_ad2\endcsname{0.08}
\expandafter\def\csname tp@zt_ad2_s1\endcsname{35.2}
\expandafter\def\csname tpsd@zt_ad2_s1\endcsname{35.2$\pm$0.6}
\expandafter\def\csname tpn@zt_ad2_s1\endcsname{3}
\expandafter\def\csname tpsec@zt_ad2_s1\endcsname{0.29}
\expandafter\def\csname tpnfe@zt_ad2_s1\endcsname{7}
\expandafter\def\csname tpfid@zt_ad2_s1\endcsname{24.9}
\expandafter\def\csname tprec@zt_ad2_s1\endcsname{0.08}
\expandafter\def\csname tp@zt_ad2_s2\endcsname{35.1}
\expandafter\def\csname tpsd@zt_ad2_s2\endcsname{35.1$\pm$0.4}
\expandafter\def\csname tpn@zt_ad2_s2\endcsname{3}
\expandafter\def\csname tpsec@zt_ad2_s2\endcsname{0.30}
\expandafter\def\csname tpnfe@zt_ad2_s2\endcsname{7}
\expandafter\def\csname tpfid@zt_ad2_s2\endcsname{24.8}
\expandafter\def\csname tprec@zt_ad2_s2\endcsname{0.08}
\expandafter\def\csname tp@zt_ad2_tg2\endcsname{26.0}
\expandafter\def\csname tpsd@zt_ad2_tg2\endcsname{26.0$\pm$0.2}
\expandafter\def\csname tpn@zt_ad2_tg2\endcsname{3}
\expandafter\def\csname tpsec@zt_ad2_tg2\endcsname{0.29}
\expandafter\def\csname tpnfe@zt_ad2_tg2\endcsname{7}
\expandafter\def\csname tpfid@zt_ad2_tg2\endcsname{30.6}
\expandafter\def\csname tprec@zt_ad2_tg2\endcsname{0.04}
\expandafter\def\csname tp@zt_ad2_tg5\endcsname{16.3}
\expandafter\def\csname tpsd@zt_ad2_tg5\endcsname{16.3$\pm$0.5}
\expandafter\def\csname tpn@zt_ad2_tg5\endcsname{3}
\expandafter\def\csname tpsec@zt_ad2_tg5\endcsname{0.29}
\expandafter\def\csname tpnfe@zt_ad2_tg5\endcsname{7}
\expandafter\def\csname tpfid@zt_ad2_tg5\endcsname{38.0}
\expandafter\def\csname tprec@zt_ad2_tg5\endcsname{0.02}
\expandafter\def\csname tp@zt_ad2_x3\endcsname{35.1}
\expandafter\def\csname tpsd@zt_ad2_x3\endcsname{35.1$\pm$0.5}
\expandafter\def\csname tpn@zt_ad2_x3\endcsname{9}
\expandafter\def\csname tpsec@zt_ad2_x3\endcsname{0.30}
\expandafter\def\csname tpnfe@zt_ad2_x3\endcsname{7}
\expandafter\def\csname tp@zt_ad3\endcsname{36.0}
\expandafter\def\csname tpsd@zt_ad3\endcsname{36.0$\pm$1.1}
\expandafter\def\csname tpn@zt_ad3\endcsname{3}
\expandafter\def\csname tpsec@zt_ad3\endcsname{0.26}
\expandafter\def\csname tpnfe@zt_ad3\endcsname{6}
\expandafter\def\csname tpfid@zt_ad3\endcsname{26.4}
\expandafter\def\csname tprec@zt_ad3\endcsname{0.12}
\expandafter\def\csname tp@zt_ad4\endcsname{36.0}
\expandafter\def\csname tpsd@zt_ad4\endcsname{36.0$\pm$0.3}
\expandafter\def\csname tpn@zt_ad4\endcsname{3}
\expandafter\def\csname tpsec@zt_ad4\endcsname{0.22}
\expandafter\def\csname tpnfe@zt_ad4\endcsname{5}
\expandafter\def\csname tpfid@zt_ad4\endcsname{38.7}
\expandafter\def\csname tprec@zt_ad4\endcsname{0.11}
\expandafter\def\csname tp@zt_dd1_g1\endcsname{20.9}
\expandafter\def\csname tpsd@zt_dd1_g1\endcsname{20.9$\pm$0.3}
\expandafter\def\csname tpn@zt_dd1_g1\endcsname{3}
\expandafter\def\csname tpsec@zt_dd1_g1\endcsname{0.38}
\expandafter\def\csname tpnfe@zt_dd1_g1\endcsname{9}
\expandafter\def\csname tpfid@zt_dd1_g1\endcsname{44.9}
\expandafter\def\csname tprec@zt_dd1_g1\endcsname{0.01}
\expandafter\def\csname tp@zt_dd2_g1\endcsname{27.1}
\expandafter\def\csname tpsd@zt_dd2_g1\endcsname{27.1$\pm$0.4}
\expandafter\def\csname tpn@zt_dd2_g1\endcsname{3}
\expandafter\def\csname tpsec@zt_dd2_g1\endcsname{0.37}
\expandafter\def\csname tpnfe@zt_dd2_g1\endcsname{9}
\expandafter\def\csname tpfid@zt_dd2_g1\endcsname{34.1}
\expandafter\def\csname tprec@zt_dd2_g1\endcsname{0.04}
\expandafter\def\csname tp@zt_dd3_g1\endcsname{32.8}
\expandafter\def\csname tpsd@zt_dd3_g1\endcsname{32.8$\pm$0.9}
\expandafter\def\csname tpn@zt_dd3_g1\endcsname{3}
\expandafter\def\csname tpsec@zt_dd3_g1\endcsname{0.37}
\expandafter\def\csname tpnfe@zt_dd3_g1\endcsname{9}
\expandafter\def\csname tpfid@zt_dd3_g1\endcsname{26.4}
\expandafter\def\csname tprec@zt_dd3_g1\endcsname{0.08}
\expandafter\def\csname tp@zt_dd4_g1\endcsname{36.4}
\expandafter\def\csname tpsd@zt_dd4_g1\endcsname{36.4$\pm$0.6}
\expandafter\def\csname tpn@zt_dd4_g1\endcsname{3}
\expandafter\def\csname tpsec@zt_dd4_g1\endcsname{0.37}
\expandafter\def\csname tpnfe@zt_dd4_g1\endcsname{9}
\expandafter\def\csname tpfid@zt_dd4_g1\endcsname{24.7}
\expandafter\def\csname tprec@zt_dd4_g1\endcsname{0.12}
\expandafter\def\csname tp@zt_dd5_g1\endcsname{38.5}
\expandafter\def\csname tpsd@zt_dd5_g1\endcsname{38.5$\pm$0.7}
\expandafter\def\csname tpn@zt_dd5_g1\endcsname{3}
\expandafter\def\csname tpsec@zt_dd5_g1\endcsname{0.37}
\expandafter\def\csname tpnfe@zt_dd5_g1\endcsname{9}
\expandafter\def\csname tpfid@zt_dd5_g1\endcsname{28.9}
\expandafter\def\csname tprec@zt_dd5_g1\endcsname{0.15}
\expandafter\def\csname tp@zt_or19_d7\endcsname{32.5}
\expandafter\def\csname tpsd@zt_or19_d7\endcsname{32.5$\pm$0.3}
\expandafter\def\csname tpn@zt_or19_d7\endcsname{3}
\expandafter\def\csname tpsec@zt_or19_d7\endcsname{1.01}
\expandafter\def\csname tpnfe@zt_or19_d7\endcsname{26}
\expandafter\def\csname tpfid@zt_or19_d7\endcsname{28.8}
\expandafter\def\csname tprec@zt_or19_d7\endcsname{0.07}
\expandafter\def\csname tp@zt_or26_d6\endcsname{38.3}
\expandafter\def\csname tpsd@zt_or26_d6\endcsname{38.3$\pm$0.6}
\expandafter\def\csname tpn@zt_or26_d6\endcsname{3}
\expandafter\def\csname tpsec@zt_or26_d6\endcsname{1.24}
\expandafter\def\csname tpnfe@zt_or26_d6\endcsname{32}
\expandafter\def\csname tpfid@zt_or26_d6\endcsname{22.5}
\expandafter\def\csname tprec@zt_or26_d6\endcsname{0.13}
\expandafter\def\csname tp@zt_sda_all\endcsname{25.1}
\expandafter\def\csname tpsd@zt_sda_all\endcsname{25.1$\pm$0.1}
\expandafter\def\csname tpn@zt_sda_all\endcsname{3}
\expandafter\def\csname tpsec@zt_sda_all\endcsname{0.71}
\expandafter\def\csname tpnfe@zt_sda_all\endcsname{8}
\expandafter\def\csname tpfid@zt_sda_all\endcsname{37.2}
\expandafter\def\csname tprec@zt_sda_all\endcsname{0.05}
\expandafter\def\csname tp@zt_sda_first2\endcsname{20.9}
\expandafter\def\csname tpsd@zt_sda_first2\endcsname{20.9$\pm$0.2}
\expandafter\def\csname tpn@zt_sda_first2\endcsname{3}
\expandafter\def\csname tpsec@zt_sda_first2\endcsname{0.43}
\expandafter\def\csname tpnfe@zt_sda_first2\endcsname{8}
\expandafter\def\csname tpfid@zt_sda_first2\endcsname{42.2}
\expandafter\def\csname tprec@zt_sda_first2\endcsname{0.03}
\expandafter\def\csname tp@zt_skip7\endcsname{12.4}
\expandafter\def\csname tpsd@zt_skip7\endcsname{12.4$\pm$0.3}
\expandafter\def\csname tpn@zt_skip7\endcsname{3}
\expandafter\def\csname tpsec@zt_skip7\endcsname{0.29}
\expandafter\def\csname tpnfe@zt_skip7\endcsname{7}
\expandafter\def\csname tpfid@zt_skip7\endcsname{57.5}
\expandafter\def\csname tprec@zt_skip7\endcsname{0.00}
\expandafter\def\csname tp@zt_skip8\endcsname{12.9}
\expandafter\def\csname tpsd@zt_skip8\endcsname{12.9$\pm$0.1}
\expandafter\def\csname tpn@zt_skip8\endcsname{3}
\expandafter\def\csname tpsec@zt_skip8\endcsname{0.33}
\expandafter\def\csname tpnfe@zt_skip8\endcsname{8}
\expandafter\def\csname tpfid@zt_skip8\endcsname{57.0}
\expandafter\def\csname tprec@zt_skip8\endcsname{0.00}
\expandafter\def\csname gp@capGuideSD\endcsname{+13.8}
\expandafter\def\csname gpci@capGuideSD\endcsname{[+11.3, +16.3]}
\expandafter\def\csname gpa@capGuideSD\endcsname{13.8}
\expandafter\def\csname gpcia@capGuideSD\endcsname{[11.3, 16.3]}
\expandafter\def\csname gp@capDistKlein\endcsname{+8.0}
\expandafter\def\csname gpci@capDistKlein\endcsname{[+5.6, +10.3]}
\expandafter\def\csname gpa@capDistKlein\endcsname{8.0}
\expandafter\def\csname gpcia@capDistKlein\endcsname{[5.6, 10.3]}
\expandafter\def\csname gp@distKleinUnguided\endcsname{+27.9}
\expandafter\def\csname gpci@distKleinUnguided\endcsname{[+24.3, +31.5]}
\expandafter\def\csname gpa@distKleinUnguided\endcsname{27.9}
\expandafter\def\csname gpcia@distKleinUnguided\endcsname{[24.3, 31.5]}
\expandafter\def\csname gp@capDistSDXL\endcsname{$-$2.2}
\expandafter\def\csname gpci@capDistSDXL\endcsname{[$-$4.9, +0.6]}
\expandafter\def\csname gpa@capDistSDXL\endcsname{2.2}
\expandafter\def\csname gpcia@capDistSDXL\endcsname{[$-$0.6, 4.9]}
\expandafter\def\csname gp@mixKlein\endcsname{+2.0}
\expandafter\def\csname gpci@mixKlein\endcsname{[+1.4, +2.7]}
\expandafter\def\csname gpa@mixKlein\endcsname{2.0}
\expandafter\def\csname gpcia@mixKlein\endcsname{[1.4, 2.7]}
\expandafter\def\csname gp@mixSDOne\endcsname{+0.6}
\expandafter\def\csname gpci@mixSDOne\endcsname{[+0.1, +1.2]}
\expandafter\def\csname gpa@mixSDOne\endcsname{0.6}
\expandafter\def\csname gpcia@mixSDOne\endcsname{[0.1, 1.2]}
\expandafter\def\csname gp@mixBase\endcsname{+0.8}
\expandafter\def\csname gpci@mixBase\endcsname{[0.0, +1.5]}
\expandafter\def\csname gpa@mixBase\endcsname{0.8}
\expandafter\def\csname gpcia@mixBase\endcsname{[0.0, 1.5]}
\expandafter\def\csname gp@mixKleinOverReal\endcsname{$-$0.1}
\expandafter\def\csname gpci@mixKleinOverReal\endcsname{[$-$0.7, +0.5]}
\expandafter\def\csname gpa@mixKleinOverReal\endcsname{0.1}
\expandafter\def\csname gpcia@mixKleinOverReal\endcsname{[$-$0.5, 0.7]}
\expandafter\def\csname gp@mixBfOverReal\endcsname{+1.9}
\expandafter\def\csname gpci@mixBfOverReal\endcsname{[+1.2, +2.7]}
\expandafter\def\csname gpa@mixBfOverReal\endcsname{1.9}
\expandafter\def\csname gpcia@mixBfOverReal\endcsname{[1.2, 2.7]}
\expandafter\def\csname gp@mixSDOneOverReal\endcsname{+2.3}
\expandafter\def\csname gpci@mixSDOneOverReal\endcsname{[+1.6, +3.0]}
\expandafter\def\csname gpa@mixSDOneOverReal\endcsname{2.3}
\expandafter\def\csname gpcia@mixSDOneOverReal\endcsname{[1.6, 3.0]}
\expandafter\def\csname gp@tgFourKlein\endcsname{$-$23.1}
\expandafter\def\csname gpci@tgFourKlein\endcsname{[$-$26.2, $-$20.2]}
\expandafter\def\csname gpa@tgFourKlein\endcsname{23.1}
\expandafter\def\csname gpcia@tgFourKlein\endcsname{[20.2, 26.2]}
\expandafter\def\csname gp@tgTwoKlein\endcsname{$-$11.7}
\expandafter\def\csname gpci@tgTwoKlein\endcsname{[$-$13.9, $-$9.5]}
\expandafter\def\csname gpa@tgTwoKlein\endcsname{11.7}
\expandafter\def\csname gpcia@tgTwoKlein\endcsname{[9.5, 13.9]}
\expandafter\def\csname gp@tgSevenSD\endcsname{$-$13.2}
\expandafter\def\csname gpci@tgSevenSD\endcsname{[$-$16.1, $-$10.5]}
\expandafter\def\csname gpa@tgSevenSD\endcsname{13.2}
\expandafter\def\csname gpcia@tgSevenSD\endcsname{[10.5, 16.1]}
\expandafter\def\csname gp@tgTwoSD\endcsname{$-$2.5}
\expandafter\def\csname gpci@tgTwoSD\endcsname{[$-$4.0, $-$1.1]}
\expandafter\def\csname gpa@tgTwoSD\endcsname{2.5}
\expandafter\def\csname gpcia@tgTwoSD\endcsname{[1.1, 4.0]}
\expandafter\def\csname gp@tgFourKleinTin\endcsname{$-$25.4}
\expandafter\def\csname gpci@tgFourKleinTin\endcsname{[$-$27.5, $-$23.4]}
\expandafter\def\csname gpa@tgFourKleinTin\endcsname{25.4}
\expandafter\def\csname gpcia@tgFourKleinTin\endcsname{[23.4, 27.5]}
\expandafter\def\csname gp@tgSevenSDTin\endcsname{$-$8.7}
\expandafter\def\csname gpci@tgSevenSDTin\endcsname{[$-$10.5, $-$6.9]}
\expandafter\def\csname gpa@tgSevenSDTin\endcsname{8.7}
\expandafter\def\csname gpcia@tgSevenSDTin\endcsname{[6.9, 10.5]}
\expandafter\def\csname gp@allKlein\endcsname{$-$2.5}
\expandafter\def\csname gpci@allKlein\endcsname{[$-$3.5, $-$1.4]}
\expandafter\def\csname gpa@allKlein\endcsname{2.5}
\expandafter\def\csname gpcia@allKlein\endcsname{[1.4, 3.5]}
\expandafter\def\csname gp@allSD\endcsname{$-$4.9}
\expandafter\def\csname gpci@allSD\endcsname{[$-$7.6, $-$2.3]}
\expandafter\def\csname gpa@allSD\endcsname{4.9}
\expandafter\def\csname gpcia@allSD\endcsname{[2.3, 7.6]}
\expandafter\def\csname gp@monoKlein\endcsname{$-$13.9}
\expandafter\def\csname gpci@monoKlein\endcsname{[$-$16.9, $-$11.0]}
\expandafter\def\csname gpa@monoKlein\endcsname{13.9}
\expandafter\def\csname gpcia@monoKlein\endcsname{[11.0, 16.9]}
\expandafter\def\csname gp@fsgKlein\endcsname{$-$23.1}
\expandafter\def\csname gpci@fsgKlein\endcsname{[$-$26.5, $-$19.8]}
\expandafter\def\csname gpa@fsgKlein\endcsname{23.1}
\expandafter\def\csname gpcia@fsgKlein\endcsname{[19.8, 26.5]}
\expandafter\def\csname gp@monoPubKlein\endcsname{$-$17.0}
\expandafter\def\csname gpci@monoPubKlein\endcsname{[$-$20.2, $-$13.8]}
\expandafter\def\csname gpa@monoPubKlein\endcsname{17.0}
\expandafter\def\csname gpcia@monoPubKlein\endcsname{[13.8, 20.2]}
\expandafter\def\csname gp@monoKleinTin\endcsname{$-$16.5}
\expandafter\def\csname gpci@monoKleinTin\endcsname{[$-$18.5, $-$14.5]}
\expandafter\def\csname gpa@monoKleinTin\endcsname{16.5}
\expandafter\def\csname gpcia@monoKleinTin\endcsname{[14.5, 18.5]}
\expandafter\def\csname gp@adKlein\endcsname{+26.7}
\expandafter\def\csname gpci@adKlein\endcsname{[+23.3, +30.1]}
\expandafter\def\csname gpa@adKlein\endcsname{26.7}
\expandafter\def\csname gpcia@adKlein\endcsname{[23.3, 30.1]}
\expandafter\def\csname gp@adSD\endcsname{+25.4}
\expandafter\def\csname gpci@adSD\endcsname{[+22.4, +28.4]}
\expandafter\def\csname gpa@adSD\endcsname{25.4}
\expandafter\def\csname gpcia@adSD\endcsname{[22.4, 28.4]}
\expandafter\def\csname gp@adZ\endcsname{+21.1}
\expandafter\def\csname gpci@adZ\endcsname{[+18.0, +24.2]}
\expandafter\def\csname gpa@adZ\endcsname{21.1}
\expandafter\def\csname gpcia@adZ\endcsname{[18.0, 24.2]}
\expandafter\def\csname gp@adVsBfKlein\endcsname{+3.9}
\expandafter\def\csname gpci@adVsBfKlein\endcsname{[+2.2, +5.7]}
\expandafter\def\csname gpa@adVsBfKlein\endcsname{3.9}
\expandafter\def\csname gpcia@adVsBfKlein\endcsname{[2.2, 5.7]}
\expandafter\def\csname gp@adVsBfSD\endcsname{+7.3}
\expandafter\def\csname gpci@adVsBfSD\endcsname{[+5.3, +9.3]}
\expandafter\def\csname gpa@adVsBfSD\endcsname{7.3}
\expandafter\def\csname gpcia@adVsBfSD\endcsname{[5.3, 9.3]}
\expandafter\def\csname gp@adVsBfZ\endcsname{+2.4}
\expandafter\def\csname gpci@adVsBfZ\endcsname{[+1.4, +3.4]}
\expandafter\def\csname gpa@adVsBfZ\endcsname{2.4}
\expandafter\def\csname gpcia@adVsBfZ\endcsname{[1.4, 3.4]}
\expandafter\def\csname gp@adVsBfZTin\endcsname{+2.9}
\expandafter\def\csname gpci@adVsBfZTin\endcsname{[+2.0, +3.9]}
\expandafter\def\csname gpa@adVsBfZTin\endcsname{2.9}
\expandafter\def\csname gpcia@adVsBfZTin\endcsname{[2.0, 3.9]}
\expandafter\def\csname gp@distSD\endcsname{$-$14.2}
\expandafter\def\csname gpci@distSD\endcsname{[$-$17.3, $-$11.2]}
\expandafter\def\csname gpa@distSD\endcsname{14.2}
\expandafter\def\csname gpcia@distSD\endcsname{[11.2, 17.3]}
\expandafter\def\csname gp@distSDXL\endcsname{$-$15.6}
\expandafter\def\csname gpci@distSDXL\endcsname{[$-$17.9, $-$13.3]}
\expandafter\def\csname gpa@distSDXL\endcsname{15.6}
\expandafter\def\csname gpcia@distSDXL\endcsname{[13.3, 17.9]}
\expandafter\def\csname gp@distKlein\endcsname{$-$6.5}
\expandafter\def\csname gpci@distKlein\endcsname{[$-$8.6, $-$4.4]}
\expandafter\def\csname gpa@distKlein\endcsname{6.5}
\expandafter\def\csname gpcia@distKlein\endcsname{[4.4, 8.6]}
\expandafter\def\csname gp@distZ\endcsname{$-$3.6}
\expandafter\def\csname gpci@distZ\endcsname{[$-$5.7, $-$1.5]}
\expandafter\def\csname gpa@distZ\endcsname{3.6}
\expandafter\def\csname gpcia@distZ\endcsname{[1.5, 5.7]}
\expandafter\def\csname gp@srpo\endcsname{+3.1}
\expandafter\def\csname gpci@srpo\endcsname{[+1.6, +4.7]}
\expandafter\def\csname gpa@srpo\endcsname{3.1}
\expandafter\def\csname gpcia@srpo\endcsname{[1.6, 4.7]}
\expandafter\def\csname gp@guideKlein\endcsname{+21.4}
\expandafter\def\csname gpci@guideKlein\endcsname{[+18.4, +24.8]}
\expandafter\def\csname gpa@guideKlein\endcsname{21.4}
\expandafter\def\csname gpcia@guideKlein\endcsname{[18.4, 24.8]}
\expandafter\def\csname gp@guideSD\endcsname{+19.8}
\expandafter\def\csname gpci@guideSD\endcsname{[+16.1, +23.3]}
\expandafter\def\csname gpa@guideSD\endcsname{19.8}
\expandafter\def\csname gpcia@guideSD\endcsname{[16.1, 23.3]}
\expandafter\def\csname gp@guideZ\endcsname{+28.1}
\expandafter\def\csname gpci@guideZ\endcsname{[+24.3, +31.7]}
\expandafter\def\csname gpa@guideZ\endcsname{28.1}
\expandafter\def\csname gpcia@guideZ\endcsname{[24.3, 31.7]}
\expandafter\def\csname gp@guideSDXL\endcsname{+3.5}
\expandafter\def\csname gpci@guideSDXL\endcsname{[+1.7, +5.3]}
\expandafter\def\csname gpa@guideSDXL\endcsname{3.5}
\expandafter\def\csname gpcia@guideSDXL\endcsname{[1.7, 5.3]}
\expandafter\def\csname gp@guideFlux\endcsname{+18.0}
\expandafter\def\csname gpci@guideFlux\endcsname{[+15.4, +20.5]}
\expandafter\def\csname gpa@guideFlux\endcsname{18.0}
\expandafter\def\csname gpcia@guideFlux\endcsname{[15.4, 20.5]}
\expandafter\def\csname gp@bfKlein\endcsname{+22.8}
\expandafter\def\csname gpci@bfKlein\endcsname{[+19.7, +25.9]}
\expandafter\def\csname gpa@bfKlein\endcsname{22.8}
\expandafter\def\csname gpcia@bfKlein\endcsname{[19.7, 25.9]}
\expandafter\def\csname gp@bfSD\endcsname{+18.1}
\expandafter\def\csname gpci@bfSD\endcsname{[+14.6, +21.7]}
\expandafter\def\csname gpa@bfSD\endcsname{18.1}
\expandafter\def\csname gpcia@bfSD\endcsname{[14.6, 21.7]}
\expandafter\def\csname gp@hiTenKlein\endcsname{$-$17.5}
\expandafter\def\csname gpci@hiTenKlein\endcsname{[$-$20.3, $-$14.7]}
\expandafter\def\csname gpa@hiTenKlein\endcsname{17.5}
\expandafter\def\csname gpcia@hiTenKlein\endcsname{[14.7, 20.3]}
\expandafter\def\csname gp@loTwentyKlein\endcsname{+0.3}
\expandafter\def\csname gpci@loTwentyKlein\endcsname{[$-$1.1, +1.6]}
\expandafter\def\csname gpa@loTwentyKlein\endcsname{0.3}
\expandafter\def\csname gpcia@loTwentyKlein\endcsname{[$-$1.1, 1.6]}
\expandafter\def\csname gp@loTenKlein\endcsname{$-$7.9}
\expandafter\def\csname gpci@loTenKlein\endcsname{[$-$10.2, $-$5.6]}
\expandafter\def\csname gpa@loTenKlein\endcsname{7.9}
\expandafter\def\csname gpcia@loTenKlein\endcsname{[5.6, 10.2]}
\expandafter\def\csname gp@hiNineSD\endcsname{$-$16.5}
\expandafter\def\csname gpci@hiNineSD\endcsname{[$-$18.8, $-$14.3]}
\expandafter\def\csname gpa@hiNineSD\endcsname{16.5}
\expandafter\def\csname gpcia@hiNineSD\endcsname{[14.3, 18.8]}
\expandafter\def\csname gp@hiThreeSD\endcsname{$-$6.3}
\expandafter\def\csname gpci@hiThreeSD\endcsname{[$-$7.5, $-$5.1]}
\expandafter\def\csname gpa@hiThreeSD\endcsname{6.3}
\expandafter\def\csname gpcia@hiThreeSD\endcsname{[5.1, 7.5]}
\expandafter\def\csname gp@loNineSD\endcsname{$-$6.9}
\expandafter\def\csname gpci@loNineSD\endcsname{[$-$9.0, $-$4.8]}
\expandafter\def\csname gpa@loNineSD\endcsname{6.9}
\expandafter\def\csname gpcia@loNineSD\endcsname{[4.8, 9.0]}
\expandafter\def\csname gp@guideSDTwo\endcsname{+19.5}
\expandafter\def\csname gpci@guideSDTwo\endcsname{[+17.0, +21.9]}
\expandafter\def\csname gpa@guideSDTwo\endcsname{19.5}
\expandafter\def\csname gpcia@guideSDTwo\endcsname{[17.0, 21.9]}
\expandafter\def\csname gp@dfKlein\endcsname{$-$0.2}
\expandafter\def\csname gpci@dfKlein\endcsname{[$-$0.9, +0.5]}
\expandafter\def\csname gpa@dfKlein\endcsname{0.2}
\expandafter\def\csname gpcia@dfKlein\endcsname{[$-$0.5, 0.9]}
\expandafter\def\csname gp@intervalKlein\endcsname{+0.8}
\expandafter\def\csname gpci@intervalKlein\endcsname{[$-$0.3, +1.8]}
\expandafter\def\csname gpa@intervalKlein\endcsname{0.8}
\expandafter\def\csname gpcia@intervalKlein\endcsname{[$-$0.3, 1.8]}
\expandafter\def\csname gp@intervalSD\endcsname{$-$9.0}
\expandafter\def\csname gpci@intervalSD\endcsname{[$-$12.2, $-$5.7]}
\expandafter\def\csname gpa@intervalSD\endcsname{9.0}
\expandafter\def\csname gpcia@intervalSD\endcsname{[5.7, 12.2]}
\expandafter\def\csname gp@cadsKlein\endcsname{+1.2}
\expandafter\def\csname gpci@cadsKlein\endcsname{[$-$2.8, +5.1]}
\expandafter\def\csname gpa@cadsKlein\endcsname{1.2}
\expandafter\def\csname gpcia@cadsKlein\endcsname{[$-$2.8, 5.1]}
\expandafter\def\csname gp@cadsSD\endcsname{+3.7}
\expandafter\def\csname gpci@cadsSD\endcsname{[+1.7, +5.6]}
\expandafter\def\csname gpa@cadsSD\endcsname{3.7}
\expandafter\def\csname gpcia@cadsSD\endcsname{[1.7, 5.6]}
\expandafter\def\csname gp@guideSDOne\endcsname{+19.2}
\expandafter\def\csname gpci@guideSDOne\endcsname{[+16.5, +21.8]}
\expandafter\def\csname gpa@guideSDOne\endcsname{19.2}
\expandafter\def\csname gpcia@guideSDOne\endcsname{[16.5, 21.8]}
\expandafter\def\csname gp@vitsBfKlein\endcsname{+11.0}
\expandafter\def\csname gpci@vitsBfKlein\endcsname{[+8.9, +13.1]}
\expandafter\def\csname gpa@vitsBfKlein\endcsname{11.0}
\expandafter\def\csname gpcia@vitsBfKlein\endcsname{[8.9, 13.1]}
\expandafter\def\csname gp@vitsGuideKlein\endcsname{+4.3}
\expandafter\def\csname gpci@vitsGuideKlein\endcsname{[+2.1, +6.5]}
\expandafter\def\csname gpa@vitsGuideKlein\endcsname{4.3}
\expandafter\def\csname gpcia@vitsGuideKlein\endcsname{[2.1, 6.5]}
\expandafter\def\csname gp@vitsGuideSDOne\endcsname{+8.6}
\expandafter\def\csname gpci@vitsGuideSDOne\endcsname{[+6.4, +10.8]}
\expandafter\def\csname gpa@vitsGuideSDOne\endcsname{8.6}
\expandafter\def\csname gpcia@vitsGuideSDOne\endcsname{[6.4, 10.8]}
\expandafter\def\csname gp@wpSDXL\endcsname{$-$22.1}
\expandafter\def\csname gpci@wpSDXL\endcsname{[$-$24.1, $-$20.2]}
\expandafter\def\csname gpa@wpSDXL\endcsname{22.1}
\expandafter\def\csname gpcia@wpSDXL\endcsname{[20.2, 24.1]}
\expandafter\def\csname gp@fixedSDXL\endcsname{$-$14.8}
\expandafter\def\csname gpci@fixedSDXL\endcsname{[$-$16.6, $-$12.9]}
\expandafter\def\csname gpa@fixedSDXL\endcsname{14.8}
\expandafter\def\csname gpcia@fixedSDXL\endcsname{[12.9, 16.6]}
\expandafter\def\csname gp@vitsAdKlein\endcsname{+11.3}
\expandafter\def\csname gpci@vitsAdKlein\endcsname{[+9.0, +13.8]}
\expandafter\def\csname gpa@vitsAdKlein\endcsname{11.3}
\expandafter\def\csname gpcia@vitsAdKlein\endcsname{[9.0, 13.8]}
\expandafter\def\csname gp@vitsAdSD\endcsname{+13.0}
\expandafter\def\csname gpci@vitsAdSD\endcsname{[+10.8, +15.4]}
\expandafter\def\csname gpa@vitsAdSD\endcsname{13.0}
\expandafter\def\csname gpcia@vitsAdSD\endcsname{[10.8, 15.4]}
\expandafter\def\csname gp@vitsAdVsBfKlein\endcsname{+0.3}
\expandafter\def\csname gpci@vitsAdVsBfKlein\endcsname{[$-$0.9, +1.6]}
\expandafter\def\csname gpa@vitsAdVsBfKlein\endcsname{0.3}
\expandafter\def\csname gpcia@vitsAdVsBfKlein\endcsname{[$-$0.9, 1.6]}
\expandafter\def\csname gp@vitsAdVsBfSD\endcsname{+2.3}
\expandafter\def\csname gpci@vitsAdVsBfSD\endcsname{[+1.2, +3.4]}
\expandafter\def\csname gpa@vitsAdVsBfSD\endcsname{2.3}
\expandafter\def\csname gpcia@vitsAdVsBfSD\endcsname{[1.2, 3.4]}
\expandafter\def\csname gp@mixAdKlein\endcsname{+1.8}
\expandafter\def\csname gpci@mixAdKlein\endcsname{[+1.1, +2.5]}
\expandafter\def\csname gpa@mixAdKlein\endcsname{1.8}
\expandafter\def\csname gpcia@mixAdKlein\endcsname{[1.1, 2.5]}
\expandafter\def\csname gp@mixAdSD\endcsname{+2.9}
\expandafter\def\csname gpci@mixAdSD\endcsname{[+2.1, +3.6]}
\expandafter\def\csname gpa@mixAdSD\endcsname{2.9}
\expandafter\def\csname gpcia@mixAdSD\endcsname{[2.1, 3.6]}
\expandafter\def\csname gp@mixAdKleinOverReal\endcsname{+1.7}
\expandafter\def\csname gpci@mixAdKleinOverReal\endcsname{[+0.9, +2.5]}
\expandafter\def\csname gpa@mixAdKleinOverReal\endcsname{1.7}
\expandafter\def\csname gpcia@mixAdKleinOverReal\endcsname{[0.9, 2.5]}
\expandafter\def\csname gp@mixAdSDOverReal\endcsname{+3.4}
\expandafter\def\csname gpci@mixAdSDOverReal\endcsname{[+2.6, +4.2]}
\expandafter\def\csname gpa@mixAdSDOverReal\endcsname{3.4}
\expandafter\def\csname gpcia@mixAdSDOverReal\endcsname{[2.6, 4.2]}
\expandafter\def\csname gp@sftKlein\endcsname{+14.7}
\expandafter\def\csname gpci@sftKlein\endcsname{[+12.1, +17.3]}
\expandafter\def\csname gpa@sftKlein\endcsname{14.7}
\expandafter\def\csname gpcia@sftKlein\endcsname{[12.1, 17.3]}
\expandafter\def\csname gp@sftSD\endcsname{$-$3.9}
\expandafter\def\csname gpci@sftSD\endcsname{[$-$6.4, $-$1.4]}
\expandafter\def\csname gpa@sftSD\endcsname{3.9}
\expandafter\def\csname gpcia@sftSD\endcsname{[1.4, 6.4]}
\expandafter\def\csname gp@sftVsAdKlein\endcsname{$-$12.0}
\expandafter\def\csname gpci@sftVsAdKlein\endcsname{[$-$15.2, $-$8.9]}
\expandafter\def\csname gpa@sftVsAdKlein\endcsname{12.0}
\expandafter\def\csname gpcia@sftVsAdKlein\endcsname{[8.9, 15.2]}
\expandafter\def\csname gp@sftVsAdSD\endcsname{$-$29.3}
\expandafter\def\csname gpci@sftVsAdSD\endcsname{[$-$32.2, $-$26.5]}
\expandafter\def\csname gpa@sftVsAdSD\endcsname{29.3}
\expandafter\def\csname gpcia@sftVsAdSD\endcsname{[26.5, 32.2]}
\expandafter\def\csname gp@scaleDistThreeK\endcsname{$-$24.6}
\expandafter\def\csname gpci@scaleDistThreeK\endcsname{[$-$28.2, $-$20.9]}
\expandafter\def\csname gpa@scaleDistThreeK\endcsname{24.6}
\expandafter\def\csname gpcia@scaleDistThreeK\endcsname{[20.9, 28.2]}
\expandafter\def\csname gp@scaleAdHundredVsDistThreeK\endcsname{+4.9}
\expandafter\def\csname gpci@scaleAdHundredVsDistThreeK\endcsname{[+2.2, +7.6]}
\expandafter\def\csname gpa@scaleAdHundredVsDistThreeK\endcsname{4.9}
\expandafter\def\csname gpcia@scaleAdHundredVsDistThreeK\endcsname{[2.2, 7.6]}
\expandafter\def\csname gp@cocoKlein\endcsname{+27.8}
\expandafter\def\csname gpci@cocoKlein\endcsname{[+24.6, +31.2]}
\expandafter\def\csname gpa@cocoKlein\endcsname{27.8}
\expandafter\def\csname gpcia@cocoKlein\endcsname{[24.6, 31.2]}
\expandafter\def\csname gp@cocoSD\endcsname{+24.1}
\expandafter\def\csname gpci@cocoSD\endcsname{[+21.1, +27.2]}
\expandafter\def\csname gpa@cocoSD\endcsname{24.1}
\expandafter\def\csname gpcia@cocoSD\endcsname{[21.1, 27.2]}
\expandafter\def\csname gp@cocoVsAdKlein\endcsname{+1.1}
\expandafter\def\csname gpci@cocoVsAdKlein\endcsname{[$-$0.1, +2.4]}
\expandafter\def\csname gpa@cocoVsAdKlein\endcsname{1.1}
\expandafter\def\csname gpcia@cocoVsAdKlein\endcsname{[$-$0.1, 2.4]}
\expandafter\def\csname gp@cocoVsAdSD\endcsname{$-$1.3}
\expandafter\def\csname gpci@cocoVsAdSD\endcsname{[$-$2.3, $-$0.3]}
\expandafter\def\csname gpa@cocoVsAdSD\endcsname{1.3}
\expandafter\def\csname gpcia@cocoVsAdSD\endcsname{[0.3, 2.3]}
\expandafter\def\csname gp@cocoKleinTin\endcsname{+29.4}
\expandafter\def\csname gpci@cocoKleinTin\endcsname{[+27.0, +31.9]}
\expandafter\def\csname gpa@cocoKleinTin\endcsname{29.4}
\expandafter\def\csname gpcia@cocoKleinTin\endcsname{[27.0, 31.9]}
\expandafter\def\csname gp@cocoSDTin\endcsname{+21.3}
\expandafter\def\csname gpci@cocoSDTin\endcsname{[+19.2, +23.4]}
\expandafter\def\csname gpa@cocoSDTin\endcsname{21.3}
\expandafter\def\csname gpcia@cocoSDTin\endcsname{[19.2, 23.4]}
\expandafter\def\csname gp@cocoVsAdKleinTin\endcsname{0.0}
\expandafter\def\csname gpci@cocoVsAdKleinTin\endcsname{[$-$0.8, +0.7]}
\expandafter\def\csname gpa@cocoVsAdKleinTin\endcsname{0.0}
\expandafter\def\csname gpcia@cocoVsAdKleinTin\endcsname{[$-$0.7, 0.8]}
\expandafter\def\csname gp@cocoVsAdSDTin\endcsname{$-$0.3}
\expandafter\def\csname gpci@cocoVsAdSDTin\endcsname{[$-$0.9, +0.4]}
\expandafter\def\csname gpa@cocoVsAdSDTin\endcsname{0.3}
\expandafter\def\csname gpcia@cocoVsAdSDTin\endcsname{[$-$0.4, 0.9]}
\expandafter\def\csname gp@foodAdKlein\endcsname{+20.4}
\expandafter\def\csname gpci@foodAdKlein\endcsname{[+17.3, +23.5]}
\expandafter\def\csname gpa@foodAdKlein\endcsname{20.4}
\expandafter\def\csname gpcia@foodAdKlein\endcsname{[17.3, 23.5]}
\expandafter\def\csname gp@foodAdSD\endcsname{+21.8}
\expandafter\def\csname gpci@foodAdSD\endcsname{[+19.4, +24.3]}
\expandafter\def\csname gpa@foodAdSD\endcsname{21.8}
\expandafter\def\csname gpcia@foodAdSD\endcsname{[19.4, 24.3]}
\expandafter\def\csname gp@foodBaseKlein\endcsname{+19.4}
\expandafter\def\csname gpci@foodBaseKlein\endcsname{[+15.8, +23.0]}
\expandafter\def\csname gpa@foodBaseKlein\endcsname{19.4}
\expandafter\def\csname gpcia@foodBaseKlein\endcsname{[15.8, 23.0]}
\expandafter\def\csname gp@foodBaseSD\endcsname{+27.3}
\expandafter\def\csname gpci@foodBaseSD\endcsname{[+24.3, +30.2]}
\expandafter\def\csname gpa@foodBaseSD\endcsname{27.3}
\expandafter\def\csname gpcia@foodBaseSD\endcsname{[24.3, 30.2]}
\expandafter\def\csname gp@foodAdVsBfKlein\endcsname{+5.0}
\expandafter\def\csname gpci@foodAdVsBfKlein\endcsname{[+3.0, +6.9]}
\expandafter\def\csname gpa@foodAdVsBfKlein\endcsname{5.0}
\expandafter\def\csname gpcia@foodAdVsBfKlein\endcsname{[3.0, 6.9]}
\expandafter\def\csname gp@foodAdVsBfSD\endcsname{+4.4}
\expandafter\def\csname gpci@foodAdVsBfSD\endcsname{[+3.0, +5.8]}
\expandafter\def\csname gpa@foodAdVsBfSD\endcsname{4.4}
\expandafter\def\csname gpcia@foodAdVsBfSD\endcsname{[3.0, 5.8]}
\expandafter\def\csname gp@lowAdKlein\endcsname{+12.1}
\expandafter\def\csname gpci@lowAdKlein\endcsname{[+10.3, +14.1]}
\expandafter\def\csname gpa@lowAdKlein\endcsname{12.1}
\expandafter\def\csname gpcia@lowAdKlein\endcsname{[10.3, 14.1]}
\expandafter\def\csname gp@lowAdSD\endcsname{+13.1}
\expandafter\def\csname gpci@lowAdSD\endcsname{[+11.7, +14.6]}
\expandafter\def\csname gpa@lowAdSD\endcsname{13.1}
\expandafter\def\csname gpcia@lowAdSD\endcsname{[11.7, 14.6]}
\expandafter\def\csname gp@lowAdVsBaseKlein\endcsname{+1.9}
\expandafter\def\csname gpci@lowAdVsBaseKlein\endcsname{[+0.8, +3.1]}
\expandafter\def\csname gpa@lowAdVsBaseKlein\endcsname{1.9}
\expandafter\def\csname gpcia@lowAdVsBaseKlein\endcsname{[0.8, 3.1]}
\expandafter\def\csname gp@lowAdVsBaseSD\endcsname{+3.0}
\expandafter\def\csname gpci@lowAdVsBaseSD\endcsname{[+1.8, +4.2]}
\expandafter\def\csname gpa@lowAdVsBaseSD\endcsname{3.0}
\expandafter\def\csname gpcia@lowAdVsBaseSD\endcsname{[1.8, 4.2]}
\expandafter\def\csname gp@lowKleinOverReal\endcsname{+14.1}
\expandafter\def\csname gpci@lowKleinOverReal\endcsname{[+12.6, +15.7]}
\expandafter\def\csname gpa@lowKleinOverReal\endcsname{14.1}
\expandafter\def\csname gpcia@lowKleinOverReal\endcsname{[12.6, 15.7]}
\expandafter\def\csname gp@lowAdKleinOverReal\endcsname{+26.3}
\expandafter\def\csname gpci@lowAdKleinOverReal\endcsname{[+23.8, +28.9]}
\expandafter\def\csname gpa@lowAdKleinOverReal\endcsname{26.3}
\expandafter\def\csname gpcia@lowAdKleinOverReal\endcsname{[23.8, 28.9]}
\expandafter\def\csname gp@tgZ\endcsname{$-$18.8}
\expandafter\def\csname gpci@tgZ\endcsname{[$-$21.3, $-$16.4]}
\expandafter\def\csname gpa@tgZ\endcsname{18.8}
\expandafter\def\csname gpcia@tgZ\endcsname{[16.4, 21.3]}
\expandafter\def\csname gp@tgZTin\endcsname{$-$18.1}
\expandafter\def\csname gpci@tgZTin\endcsname{[$-$19.9, $-$16.4]}
\expandafter\def\csname gpa@tgZTin\endcsname{18.1}
\expandafter\def\csname gpcia@tgZTin\endcsname{[16.4, 19.9]}
\expandafter\def\csname gp@tgZVsDist\endcsname{+2.3}
\expandafter\def\csname gpci@tgZVsDist\endcsname{[+0.1, +4.6]}
\expandafter\def\csname gpa@tgZVsDist\endcsname{2.3}
\expandafter\def\csname gpcia@tgZVsDist\endcsname{[0.1, 4.6]}
\expandafter\def\csname gp@carsAdVsBfKlein\endcsname{$-$2.6}
\expandafter\def\csname gpci@carsAdVsBfKlein\endcsname{[$-$4.5, $-$0.7]}
\expandafter\def\csname gpa@carsAdVsBfKlein\endcsname{2.6}
\expandafter\def\csname gpcia@carsAdVsBfKlein\endcsname{[0.7, 4.5]}
\expandafter\def\csname gp@carsAdVsBfSD\endcsname{+3.4}
\expandafter\def\csname gpci@carsAdVsBfSD\endcsname{[+2.2, +4.7]}
\expandafter\def\csname gpa@carsAdVsBfSD\endcsname{3.4}
\expandafter\def\csname gpcia@carsAdVsBfSD\endcsname{[2.2, 4.7]}
\expandafter\def\csname gp@petsAdVsBfKlein\endcsname{+0.8}
\expandafter\def\csname gpci@petsAdVsBfKlein\endcsname{[$-$2.5, +4.2]}
\expandafter\def\csname gpa@petsAdVsBfKlein\endcsname{0.8}
\expandafter\def\csname gpcia@petsAdVsBfKlein\endcsname{[$-$2.5, 4.2]}
\expandafter\def\csname gp@petsAdVsBfSD\endcsname{+3.9}
\expandafter\def\csname gpci@petsAdVsBfSD\endcsname{[+2.0, +6.0]}
\expandafter\def\csname gpa@petsAdVsBfSD\endcsname{3.9}
\expandafter\def\csname gpcia@petsAdVsBfSD\endcsname{[2.0, 6.0]}
\expandafter\def\csname gp@carsAdKlein\endcsname{+17.5}
\expandafter\def\csname gpci@carsAdKlein\endcsname{[+15.2, +19.9]}
\expandafter\def\csname gpa@carsAdKlein\endcsname{17.5}
\expandafter\def\csname gpcia@carsAdKlein\endcsname{[15.2, 19.9]}
\expandafter\def\csname gp@carsAdSD\endcsname{+21.5}
\expandafter\def\csname gpci@carsAdSD\endcsname{[+19.4, +23.6]}
\expandafter\def\csname gpa@carsAdSD\endcsname{21.5}
\expandafter\def\csname gpcia@carsAdSD\endcsname{[19.4, 23.6]}
\expandafter\def\csname gp@petsAdKlein\endcsname{+25.6}
\expandafter\def\csname gpci@petsAdKlein\endcsname{[+18.7, +32.6]}
\expandafter\def\csname gpa@petsAdKlein\endcsname{25.6}
\expandafter\def\csname gpcia@petsAdKlein\endcsname{[18.7, 32.6]}
\expandafter\def\csname gp@petsAdSD\endcsname{+35.0}
\expandafter\def\csname gpci@petsAdSD\endcsname{[+29.9, +39.9]}
\expandafter\def\csname gpa@petsAdSD\endcsname{35.0}
\expandafter\def\csname gpcia@petsAdSD\endcsname{[29.9, 39.9]}
\expandafter\def\csname gp@inkAdKlein\endcsname{+25.8}
\expandafter\def\csname gpci@inkAdKlein\endcsname{[+24.6, +27.0]}
\expandafter\def\csname gpa@inkAdKlein\endcsname{25.8}
\expandafter\def\csname gpcia@inkAdKlein\endcsname{[24.6, 27.0]}
\expandafter\def\csname gp@inkAdSD\endcsname{+19.4}
\expandafter\def\csname gpci@inkAdSD\endcsname{[+18.4, +20.3]}
\expandafter\def\csname gpa@inkAdSD\endcsname{19.4}
\expandafter\def\csname gpcia@inkAdSD\endcsname{[18.4, 20.3]}
\expandafter\def\csname gp@inkDistFullVsPilot\endcsname{0.0}
\expandafter\def\csname gpci@inkDistFullVsPilot\endcsname{[$-$0.3, +0.3]}
\expandafter\def\csname gpa@inkDistFullVsPilot\endcsname{0.0}
\expandafter\def\csname gpcia@inkDistFullVsPilot\endcsname{[$-$0.3, 0.3]}
\expandafter\def\csname gp@capAdKlein\endcsname{+6.4}
\expandafter\def\csname gpci@capAdKlein\endcsname{[+4.3, +8.6]}
\expandafter\def\csname gpa@capAdKlein\endcsname{6.4}
\expandafter\def\csname gpcia@capAdKlein\endcsname{[4.3, 8.6]}
\expandafter\def\csname gp@capAdSD\endcsname{+20.7}
\expandafter\def\csname gpci@capAdSD\endcsname{[+17.7, +23.8]}
\expandafter\def\csname gpa@capAdSD\endcsname{20.7}
\expandafter\def\csname gpcia@capAdSD\endcsname{[17.7, 23.8]}
\expandafter\def\csname gp@capAdVsBfKlein\endcsname{+0.6}
\expandafter\def\csname gpci@capAdVsBfKlein\endcsname{[$-$0.7, +2.0]}
\expandafter\def\csname gpa@capAdVsBfKlein\endcsname{0.6}
\expandafter\def\csname gpcia@capAdVsBfKlein\endcsname{[$-$0.7, 2.0]}
\expandafter\def\csname gp@capAdVsBfSD\endcsname{+10.4}
\expandafter\def\csname gpci@capAdVsBfSD\endcsname{[+8.2, +12.6]}
\expandafter\def\csname gpa@capAdVsBfSD\endcsname{10.4}
\expandafter\def\csname gpcia@capAdVsBfSD\endcsname{[8.2, 12.6]}
\expandafter\def\csname gp@regenKlein\endcsname{+0.4}
\expandafter\def\csname gpci@regenKlein\endcsname{[$-$0.2, +1.1]}
\expandafter\def\csname gpa@regenKlein\endcsname{0.4}
\expandafter\def\csname gpcia@regenKlein\endcsname{[$-$0.2, 1.1]}
\expandafter\def\csname gp@regenKd\endcsname{+0.4}
\expandafter\def\csname gpci@regenKd\endcsname{[$-$0.6, +1.4]}
\expandafter\def\csname gpa@regenKd\endcsname{0.4}
\expandafter\def\csname gpcia@regenKd\endcsname{[$-$0.6, 1.4]}
\expandafter\def\csname gp@regenSdt\endcsname{$-$1.2}
\expandafter\def\csname gpci@regenSdt\endcsname{[$-$1.9, $-$0.4]}
\expandafter\def\csname gpa@regenSdt\endcsname{1.2}
\expandafter\def\csname gpcia@regenSdt\endcsname{[0.4, 1.9]}
\expandafter\def\csname gp@regenSdtAd\endcsname{+0.6}
\expandafter\def\csname gpci@regenSdtAd\endcsname{[$-$0.6, +1.7]}
\expandafter\def\csname gpa@regenSdtAd\endcsname{0.6}
\expandafter\def\csname gpcia@regenSdtAd\endcsname{[$-$0.6, 1.7]}
\expandafter\def\csname gp@regenGainKlein\endcsname{+27.2}
\expandafter\def\csname gpci@regenGainKlein\endcsname{[+23.7, +30.7]}
\expandafter\def\csname gpa@regenGainKlein\endcsname{27.2}
\expandafter\def\csname gpcia@regenGainKlein\endcsname{[23.7, 30.7]}
\expandafter\def\csname gp@regenGainSD\endcsname{+26.7}
\expandafter\def\csname gpci@regenGainSD\endcsname{[+24.0, +29.4]}
\expandafter\def\csname gpa@regenGainSD\endcsname{26.7}
\expandafter\def\csname gpcia@regenGainSD\endcsname{[24.0, 29.4]}
\expandafter\def\csname gp@inkAdFullVsPilot\endcsname{+15.6}
\expandafter\def\csname gpci@inkAdFullVsPilot\endcsname{[+14.8, +16.4]}
\expandafter\def\csname gpa@inkAdFullVsPilot\endcsname{15.6}
\expandafter\def\csname gpcia@inkAdFullVsPilot\endcsname{[14.8, 16.4]}
\expandafter\def\csname gp@inkAdVsBaseHundred\endcsname{+1.1}
\expandafter\def\csname gpci@inkAdVsBaseHundred\endcsname{[+0.7, +1.4]}
\expandafter\def\csname gpa@inkAdVsBaseHundred\endcsname{1.1}
\expandafter\def\csname gpcia@inkAdVsBaseHundred\endcsname{[0.7, 1.4]}
\expandafter\def\csname gp@inkSdtAdVsBase\endcsname{+0.4}
\expandafter\def\csname gpci@inkSdtAdVsBase\endcsname{[$-$0.2, +0.9]}
\expandafter\def\csname gpa@inkSdtAdVsBase\endcsname{0.4}
\expandafter\def\csname gpcia@inkSdtAdVsBase\endcsname{[$-$0.2, 0.9]}
\expandafter\def\csname gp@llmAdKlein\endcsname{+1.7}
\expandafter\def\csname gpci@llmAdKlein\endcsname{[$-$0.4, +4.0]}
\expandafter\def\csname gpa@llmAdKlein\endcsname{1.7}
\expandafter\def\csname gpcia@llmAdKlein\endcsname{[$-$0.4, 4.0]}
\expandafter\def\csname gp@llmAdSD\endcsname{+16.2}
\expandafter\def\csname gpci@llmAdSD\endcsname{[+13.6, +18.9]}
\expandafter\def\csname gpa@llmAdSD\endcsname{16.2}
\expandafter\def\csname gpcia@llmAdSD\endcsname{[13.6, 18.9]}
\expandafter\def\csname gp@llmGapKlein\endcsname{+5.0}
\expandafter\def\csname gpci@llmGapKlein\endcsname{[+2.6, +7.5]}
\expandafter\def\csname gpa@llmGapKlein\endcsname{5.0}
\expandafter\def\csname gpcia@llmGapKlein\endcsname{[2.6, 7.5]}
\expandafter\def\csname gp@oursVsSda\endcsname{+10.0}
\expandafter\def\csname gpci@oursVsSda\endcsname{[+7.5, +12.6]}
\expandafter\def\csname gpa@oursVsSda\endcsname{10.0}
\expandafter\def\csname gpcia@oursVsSda\endcsname{[7.5, 12.6]}
\expandafter\def\csname gp@inkMixAdOverReal\endcsname{$-$0.2}
\expandafter\def\csname gpci@inkMixAdOverReal\endcsname{[$-$0.4, 0.0]}
\expandafter\def\csname gpa@inkMixAdOverReal\endcsname{0.2}
\expandafter\def\csname gpcia@inkMixAdOverReal\endcsname{[0.0, 0.4]}
\expandafter\def\csname gp@inkMixDistOverReal\endcsname{$-$0.7}
\expandafter\def\csname gpci@inkMixDistOverReal\endcsname{[$-$0.9, $-$0.5]}
\expandafter\def\csname gpa@inkMixDistOverReal\endcsname{0.7}
\expandafter\def\csname gpcia@inkMixDistOverReal\endcsname{[0.5, 0.9]}
\expandafter\def\csname gp@inkMixAdOverDist\endcsname{+0.5}
\expandafter\def\csname gpci@inkMixAdOverDist\endcsname{[+0.3, +0.7]}
\expandafter\def\csname gpa@inkMixAdOverDist\endcsname{0.5}
\expandafter\def\csname gpcia@inkMixAdOverDist\endcsname{[0.3, 0.7]}
\expandafter\def\csname gp@inkBaseVsAdFull\endcsname{+3.0}
\expandafter\def\csname gpci@inkBaseVsAdFull\endcsname{[+2.4, +3.6]}
\expandafter\def\csname gpa@inkBaseVsAdFull\endcsname{3.0}
\expandafter\def\csname gpcia@inkBaseVsAdFull\endcsname{[2.4, 3.6]}
\expandafter\def\csname gp@dpdmdVsTeacher\endcsname{$-$7.2}
\expandafter\def\csname gpci@dpdmdVsTeacher\endcsname{[$-$8.9, $-$5.5]}
\expandafter\def\csname gpa@dpdmdVsTeacher\endcsname{7.2}
\expandafter\def\csname gpcia@dpdmdVsTeacher\endcsname{[5.5, 8.9]}
\expandafter\def\csname gp@dpdmdGuide\endcsname{+23.8}
\expandafter\def\csname gpci@dpdmdGuide\endcsname{[+20.6, +27.0]}
\expandafter\def\csname gpa@dpdmdGuide\endcsname{23.8}
\expandafter\def\csname gpcia@dpdmdGuide\endcsname{[20.6, 27.0]}
\expandafter\def\csname gp@dpdmdBf\endcsname{+1.8}
\expandafter\def\csname gpci@dpdmdBf\endcsname{[+0.2, +3.6]}
\expandafter\def\csname gpa@dpdmdBf\endcsname{1.8}
\expandafter\def\csname gpcia@dpdmdBf\endcsname{[0.2, 3.6]}
\expandafter\def\csname gp@dpdmdAd\endcsname{+7.7}
\expandafter\def\csname gpci@dpdmdAd\endcsname{[+6.2, +9.3]}
\expandafter\def\csname gpa@dpdmdAd\endcsname{7.7}
\expandafter\def\csname gpcia@dpdmdAd\endcsname{[6.2, 9.3]}
\expandafter\def\csname gp@dpdmdAdDeep\endcsname{+13.4}
\expandafter\def\csname gpci@dpdmdAdDeep\endcsname{[+11.1, +15.7]}
\expandafter\def\csname gpa@dpdmdAdDeep\endcsname{13.4}
\expandafter\def\csname gpcia@dpdmdAdDeep\endcsname{[11.1, 15.7]}
\expandafter\def\csname gp@dpdmdAdVsBf\endcsname{+5.9}
\expandafter\def\csname gpci@dpdmdAdVsBf\endcsname{[+4.4, +7.4]}
\expandafter\def\csname gpa@dpdmdAdVsBf\endcsname{5.9}
\expandafter\def\csname gpcia@dpdmdAdVsBf\endcsname{[4.4, 7.4]}
\expandafter\def\csname gp@dpdmdDeepVsFirst\endcsname{+5.7}
\expandafter\def\csname gpci@dpdmdDeepVsFirst\endcsname{[+3.9, +7.3]}
\expandafter\def\csname gpa@dpdmdDeepVsFirst\endcsname{5.7}
\expandafter\def\csname gpcia@dpdmdDeepVsFirst\endcsname{[3.9, 7.3]}
\expandafter\def\csname gp@dpdmdAdTin\endcsname{+8.9}
\expandafter\def\csname gpci@dpdmdAdTin\endcsname{[+7.7, +10.1]}
\expandafter\def\csname gpa@dpdmdAdTin\endcsname{8.9}
\expandafter\def\csname gpcia@dpdmdAdTin\endcsname{[7.7, 10.1]}
\expandafter\def\csname gp@dpdmdAdVsBfTin\endcsname{+6.7}
\expandafter\def\csname gpci@dpdmdAdVsBfTin\endcsname{[+5.5, +7.9]}
\expandafter\def\csname gpa@dpdmdAdVsBfTin\endcsname{6.7}
\expandafter\def\csname gpcia@dpdmdAdVsBfTin\endcsname{[5.5, 7.9]}
\expandafter\def\csname nm@tgShareKlein\endcsname{11}
\expandafter\def\csname nm@tgShareSD\endcsname{48}
\expandafter\def\csname nm@anchorShareKlein\endcsname{57}
\expandafter\def\csname nm@anchorShareSD\endcsname{55}
\expandafter\def\csname nm@tgVendiKlein\endcsname{8}
\expandafter\def\csname nm@tgVendiSD\endcsname{20}
\expandafter\def\csname nm@anchorVendiKlein\endcsname{22}
\expandafter\def\csname nm@anchorVendiSD\endcsname{39}
\expandafter\def\csname nm@llmShareKlein\endcsname{35}
\expandafter\def\csname nm@llmShareSD\endcsname{78}
\expandafter\def\csname nm@inkShareKlein\endcsname{112}
\expandafter\def\csname nm@inkShareSD\endcsname{104}
\expandafter\def\csname nm@sdaShare\endcsname{36}
\expandafter\def\csname nm@inkFullShareKlein\endcsname{90}
\expandafter\def\csname nm@cocoShareKlein\endcsname{104}
\expandafter\def\csname nm@cocoShareSD\endcsname{95}
\expandafter\def\csname nm@cocoShareKleinTin\endcsname{100}
\expandafter\def\csname nm@cocoShareSDTin\endcsname{99}
\expandafter\def\csname nm@foodShareKlein\endcsname{105}
\expandafter\def\csname nm@foodShareSD\endcsname{80}
\expandafter\def\csname nm@tgShareZ\endcsname{11}
\expandafter\def\csname nm@tgShareZTin\endcsname{25}
\expandafter\def\csname nm@tgVendiZ\endcsname{32}
\expandafter\def\csname nm@tgRecallKlein\endcsname{2}
\expandafter\def\csname nm@tgRecallSD\endcsname{25}
\expandafter\def\csname nm@tgRecallZ\endcsname{23}
\expandafter\def\csname nm@dpdmdRetained\endcsname{$-$30}
\expandafter\def\csname nm@dpdmdAdShare\endcsname{25}
\expandafter\def\csname nm@dpdmdAdDeepShare\endcsname{43}
\expandafter\def\csname nm@carsShareKlein\endcsname{117}
\expandafter\def\csname nm@carsShareSD\endcsname{94}
\expandafter\def\csname nm@petsShareKlein\endcsname{96}
\expandafter\def\csname nm@petsShareSD\endcsname{76}
\expandafter\def\csname nm@cocoFoodShareKlein\endcsname{105}
\expandafter\def\csname nm@cocoFoodShareSD\endcsname{98}
\expandafter\def\csname nm@cocoCarsShareKlein\endcsname{81}
\expandafter\def\csname nm@cocoCarsShareSD\endcsname{98}
\expandafter\def\csname nm@capShareKlein\endcsname{81}
\expandafter\def\csname nm@capShareSD\endcsname{98}
\expandafter\def\csname nm@tgShareMax\endcsname{48}
\expandafter\def\csname nm@tgVendiMax\endcsname{32}
\expandafter\def\csname nm@tgRecallMax\endcsname{25}
\expandafter\def\csname nm@regenMax\endcsname{1.2}
\expandafter\def\csname nm@tTwoRecallKlein\endcsname{+0.91}
\expandafter\def\csname nm@tTwoRecallSD\endcsname{+0.60}
\expandafter\def\csname nm@guideMin\endcsname{3.5}
\expandafter\def\csname nm@guideMax\endcsname{28.1}
\expandafter\def\csname nm@cpuCalMax\endcsname{0.32}
\expandafter\def\csname nm@wpEpochSDXLTurbo\endcsname{19--26}
\expandafter\def\csname nm@wpEpochSDXL\endcsname{62--71}
\expandafter\def\csname nm@sdxlRecallMax\endcsname{0.13}
\expandafter\def\csname nm@wpReproMax\endcsname{3.0}
\expandafter\def\csname nm@inkGainShareKlein\endcsname{88}
\expandafter\def\csname nm@inkGainShareSD\endcsname{90}
\expandafter\def\csname nm@adKleinMean\endcsname{43.8}
\expandafter\def\csname nm@adKleinRange\endcsname{43.6--44.1}
\expandafter\def\csname nm@adKleinOneMean\endcsname{43.5}
\expandafter\def\csname nm@adKleinOneRange\endcsname{43.2--43.9}
\expandafter\def\csname nm@adSDMean\endcsname{43.7}
\expandafter\def\csname nm@adSDRange\endcsname{43.3--44.0}
\expandafter\def\csname nm@adZMean\endcsname{35.1}
\expandafter\def\csname nm@adZRange\endcsname{35.1--35.2}
\expandafter\def\csname nm@eNSets\endcsname{186}
\expandafter\def\csname nm@rhoRecall\endcsname{+0.87}
\expandafter\def\csname nm@rhoRecallCI\endcsname{[+0.81, +0.93]}
\expandafter\def\csname nm@rhoRecallPooled\endcsname{+0.91}
\expandafter\def\csname nm@rhoRecallInKlein\endcsname{+0.95}
\expandafter\def\csname nm@rhoRecallInKleinCI\endcsname{[+0.91, +0.98]}
\expandafter\def\csname nm@rhoRecallInSd21\endcsname{+0.91}
\expandafter\def\csname nm@rhoRecallInSd21CI\endcsname{[+0.84, +0.95]}
\expandafter\def\csname nm@rhoRecallInSdxl\endcsname{+0.20}
\expandafter\def\csname nm@rhoRecallInSdxlCI\endcsname{[$-$0.59, +0.81]}
\expandafter\def\csname nm@rhoRecallInZimage\endcsname{+0.97}
\expandafter\def\csname nm@rhoRecallInZimageCI\endcsname{[+0.85, +1.00]}
\expandafter\def\csname nm@rhoRecallClip\endcsname{+0.86}
\expandafter\def\csname nm@rhoRecallClipCI\endcsname{[+0.79, +0.91]}
\expandafter\def\csname nm@rhoRecallClipPooled\endcsname{+0.89}
\expandafter\def\csname nm@rhoRecallClipInKlein\endcsname{+0.94}
\expandafter\def\csname nm@rhoRecallClipInKleinCI\endcsname{[+0.87, +0.98]}
\expandafter\def\csname nm@rhoRecallClipInSd21\endcsname{+0.86}
\expandafter\def\csname nm@rhoRecallClipInSd21CI\endcsname{[+0.77, +0.91]}
\expandafter\def\csname nm@rhoRecallClipInSdxl\endcsname{+0.24}
\expandafter\def\csname nm@rhoRecallClipInSdxlCI\endcsname{[$-$0.55, +0.83]}
\expandafter\def\csname nm@rhoRecallClipInZimage\endcsname{+0.98}
\expandafter\def\csname nm@rhoRecallClipInZimageCI\endcsname{[+0.85, +1.00]}
\expandafter\def\csname nm@rhoFdClip\endcsname{$-$0.86}
\expandafter\def\csname nm@rhoFdClipCI\endcsname{[$-$0.91, $-$0.79]}
\expandafter\def\csname nm@rhoFdClipPooled\endcsname{$-$0.88}
\expandafter\def\csname nm@rhoFdClipInKlein\endcsname{$-$0.92}
\expandafter\def\csname nm@rhoFdClipInKleinCI\endcsname{[$-$0.96, $-$0.85]}
\expandafter\def\csname nm@rhoFdClipInSd21\endcsname{$-$0.85}
\expandafter\def\csname nm@rhoFdClipInSd21CI\endcsname{[$-$0.93, $-$0.73]}
\expandafter\def\csname nm@rhoFdClipInSdxl\endcsname{$-$0.44}
\expandafter\def\csname nm@rhoFdClipInSdxlCI\endcsname{[$-$0.89, +0.26]}
\expandafter\def\csname nm@rhoFdClipInZimage\endcsname{$-$0.98}
\expandafter\def\csname nm@rhoFdClipInZimageCI\endcsname{[$-$1.00, $-$0.82]}
\expandafter\def\csname nm@rhoCoverage\endcsname{+0.30}
\expandafter\def\csname nm@rhoCoverageCI\endcsname{[+0.15, +0.45]}
\expandafter\def\csname nm@rhoCoveragePooled\endcsname{+0.03}
\expandafter\def\csname nm@rhoCoverageInKlein\endcsname{+0.34}
\expandafter\def\csname nm@rhoCoverageInKleinCI\endcsname{[+0.11, +0.54]}
\expandafter\def\csname nm@rhoCoverageInSd21\endcsname{+0.22}
\expandafter\def\csname nm@rhoCoverageInSd21CI\endcsname{[$-$0.06, +0.50]}
\expandafter\def\csname nm@rhoCoverageInSdxl\endcsname{+0.21}
\expandafter\def\csname nm@rhoCoverageInSdxlCI\endcsname{[$-$0.39, +0.93]}
\expandafter\def\csname nm@rhoCoverageInZimage\endcsname{+0.76}
\expandafter\def\csname nm@rhoCoverageInZimageCI\endcsname{[+0.22, +0.99]}
\expandafter\def\csname nm@rhoCoverageClip\endcsname{+0.63}
\expandafter\def\csname nm@rhoCoverageClipCI\endcsname{[+0.52, +0.72]}
\expandafter\def\csname nm@rhoCoverageClipPooled\endcsname{+0.60}
\expandafter\def\csname nm@rhoCoverageClipInKlein\endcsname{+0.75}
\expandafter\def\csname nm@rhoCoverageClipInKleinCI\endcsname{[+0.62, +0.83]}
\expandafter\def\csname nm@rhoCoverageClipInSd21\endcsname{+0.51}
\expandafter\def\csname nm@rhoCoverageClipInSd21CI\endcsname{[+0.28, +0.70]}
\expandafter\def\csname nm@rhoCoverageClipInSdxl\endcsname{+0.22}
\expandafter\def\csname nm@rhoCoverageClipInSdxlCI\endcsname{[$-$0.39, +0.70]}
\expandafter\def\csname nm@rhoCoverageClipInZimage\endcsname{+0.82}
\expandafter\def\csname nm@rhoCoverageClipInZimageCI\endcsname{[+0.36, +1.00]}
\expandafter\def\csname nm@rhoFid\endcsname{$-$0.66}
\expandafter\def\csname nm@rhoFidCI\endcsname{[$-$0.76, $-$0.55]}
\expandafter\def\csname nm@rhoFidPooled\endcsname{$-$0.60}
\expandafter\def\csname nm@rhoFidInKlein\endcsname{$-$0.83}
\expandafter\def\csname nm@rhoFidInKleinCI\endcsname{[$-$0.89, $-$0.73]}
\expandafter\def\csname nm@rhoFidInSd21\endcsname{$-$0.38}
\expandafter\def\csname nm@rhoFidInSd21CI\endcsname{[$-$0.62, $-$0.12]}
\expandafter\def\csname nm@rhoFidInSdxl\endcsname{$-$0.54}
\expandafter\def\csname nm@rhoFidInSdxlCI\endcsname{[$-$0.97, +0.19]}
\expandafter\def\csname nm@rhoFidInZimage\endcsname{$-$0.91}
\expandafter\def\csname nm@rhoFidInZimageCI\endcsname{[$-$1.00, $-$0.63]}
\expandafter\def\csname nm@rhoIs\endcsname{$-$0.34}
\expandafter\def\csname nm@rhoIsCI\endcsname{[$-$0.48, $-$0.17]}
\expandafter\def\csname nm@rhoIsPooled\endcsname{$-$0.48}
\expandafter\def\csname nm@rhoIsInKlein\endcsname{$-$0.44}
\expandafter\def\csname nm@rhoIsInKleinCI\endcsname{[$-$0.63, $-$0.22]}
\expandafter\def\csname nm@rhoIsInSd21\endcsname{$-$0.25}
\expandafter\def\csname nm@rhoIsInSd21CI\endcsname{[$-$0.50, +0.01]}
\expandafter\def\csname nm@rhoIsInSdxl\endcsname{+0.17}
\expandafter\def\csname nm@rhoIsInSdxlCI\endcsname{[$-$0.59, +0.89]}
\expandafter\def\csname nm@rhoIsInZimage\endcsname{$-$0.36}
\expandafter\def\csname nm@rhoIsInZimageCI\endcsname{[$-$0.85, +0.43]}
\expandafter\def\csname nm@rhoRecog\endcsname{$-$0.54}
\expandafter\def\csname nm@rhoRecogCI\endcsname{[$-$0.66, $-$0.39]}
\expandafter\def\csname nm@rhoRecogPooled\endcsname{$-$0.43}
\expandafter\def\csname nm@rhoRecogInKlein\endcsname{$-$0.65}
\expandafter\def\csname nm@rhoRecogInKleinCI\endcsname{[$-$0.83, $-$0.43]}
\expandafter\def\csname nm@rhoRecogInSd21\endcsname{$-$0.41}
\expandafter\def\csname nm@rhoRecogInSd21CI\endcsname{[$-$0.63, $-$0.17]}
\expandafter\def\csname nm@rhoRecogInSdxl\endcsname{$-$0.01}
\expandafter\def\csname nm@rhoRecogInSdxlCI\endcsname{[$-$0.66, +0.72]}
\expandafter\def\csname nm@rhoRecogInZimage\endcsname{$-$0.87}
\expandafter\def\csname nm@rhoRecogInZimageCI\endcsname{[$-$1.00, $-$0.48]}
\expandafter\def\csname nm@rhoVendi\endcsname{+0.78}
\expandafter\def\csname nm@rhoVendiCI\endcsname{[+0.68, +0.86]}
\expandafter\def\csname nm@rhoVendiPooled\endcsname{+0.82}
\expandafter\def\csname nm@rhoVendiInKlein\endcsname{+0.83}
\expandafter\def\csname nm@rhoVendiInKleinCI\endcsname{[+0.69, +0.94]}
\expandafter\def\csname nm@rhoVendiInSd21\endcsname{+0.78}
\expandafter\def\csname nm@rhoVendiInSd21CI\endcsname{[+0.67, +0.86]}
\expandafter\def\csname nm@rhoVendiInSdxl\endcsname{+0.21}
\expandafter\def\csname nm@rhoVendiInSdxlCI\endcsname{[$-$0.65, +0.81]}
\expandafter\def\csname nm@rhoVendiInZimage\endcsname{+0.99}
\expandafter\def\csname nm@rhoVendiInZimageCI\endcsname{[+0.92, +1.00]}
\expandafter\def\csname nm@rhoAesthetic\endcsname{$-$0.46}
\expandafter\def\csname nm@rhoAestheticCI\endcsname{[$-$0.58, $-$0.31]}
\expandafter\def\csname nm@rhoAestheticPooled\endcsname{$-$0.32}
\expandafter\def\csname nm@rhoAestheticInKlein\endcsname{$-$0.56}
\expandafter\def\csname nm@rhoAestheticInKleinCI\endcsname{[$-$0.73, $-$0.34]}
\expandafter\def\csname nm@rhoAestheticInSd21\endcsname{$-$0.35}
\expandafter\def\csname nm@rhoAestheticInSd21CI\endcsname{[$-$0.59, $-$0.09]}
\expandafter\def\csname nm@rhoAestheticInSdxl\endcsname{+0.26}
\expandafter\def\csname nm@rhoAestheticInSdxlCI\endcsname{[$-$0.42, +0.79]}
\expandafter\def\csname nm@rhoAestheticInZimage\endcsname{$-$0.90}
\expandafter\def\csname nm@rhoAestheticInZimageCI\endcsname{[$-$1.00, $-$0.61]}
\expandafter\def\csname nm@rhoPick\endcsname{$-$0.55}
\expandafter\def\csname nm@rhoPickCI\endcsname{[$-$0.69, $-$0.39]}
\expandafter\def\csname nm@rhoPickPooled\endcsname{$-$0.59}
\expandafter\def\csname nm@rhoPickInKlein\endcsname{$-$0.67}
\expandafter\def\csname nm@rhoPickInKleinCI\endcsname{[$-$0.85, $-$0.44]}
\expandafter\def\csname nm@rhoPickInSd21\endcsname{$-$0.43}
\expandafter\def\csname nm@rhoPickInSd21CI\endcsname{[$-$0.68, $-$0.15]}
\expandafter\def\csname nm@rhoPickInSdxl\endcsname{$-$0.21}
\expandafter\def\csname nm@rhoPickInSdxlCI\endcsname{[$-$0.82, +0.63]}
\expandafter\def\csname nm@rhoPickInZimage\endcsname{$-$0.49}
\expandafter\def\csname nm@rhoPickInZimageCI\endcsname{[$-$0.87, +0.20]}
\expandafter\def\csname nm@rhoLinear\endcsname{+0.69}
\expandafter\def\csname nm@rhoLinearCI\endcsname{[+0.58, +0.76]}
\expandafter\def\csname nm@rhoLinearPooled\endcsname{+0.41}
\expandafter\def\csname nm@rhoLinearInKlein\endcsname{+0.65}
\expandafter\def\csname nm@rhoLinearInKleinCI\endcsname{[+0.49, +0.77]}
\expandafter\def\csname nm@rhoLinearInSd21\endcsname{+0.77}
\expandafter\def\csname nm@rhoLinearInSd21CI\endcsname{[+0.63, +0.86]}
\expandafter\def\csname nm@rhoLinearInSdxl\endcsname{+0.59}
\expandafter\def\csname nm@rhoLinearInSdxlCI\endcsname{[$-$0.07, +0.89]}
\expandafter\def\csname nm@rhoLinearInZimage\endcsname{+0.73}
\expandafter\def\csname nm@rhoLinearInZimageCI\endcsname{[+0.25, +0.92]}
\expandafter\def\csname nm@rhoContrast\endcsname{$-$0.49}
\expandafter\def\csname nm@rhoContrastCI\endcsname{[$-$0.59, $-$0.36]}
\expandafter\def\csname nm@rhoContrastPooled\endcsname{$-$0.40}
\expandafter\def\csname nm@rhoContrastInKlein\endcsname{$-$0.48}
\expandafter\def\csname nm@rhoContrastInKleinCI\endcsname{[$-$0.61, $-$0.30]}
\expandafter\def\csname nm@rhoContrastInSd21\endcsname{$-$0.63}
\expandafter\def\csname nm@rhoContrastInSd21CI\endcsname{[$-$0.77, $-$0.44]}
\expandafter\def\csname nm@rhoContrastInSdxl\endcsname{$-$0.14}
\expandafter\def\csname nm@rhoContrastInSdxlCI\endcsname{[$-$0.81, +0.52]}
\expandafter\def\csname nm@rhoContrastInZimage\endcsname{$-$0.18}
\expandafter\def\csname nm@rhoContrastInZimageCI\endcsname{[$-$0.64, +0.54]}
\expandafter\def\csname nm@rhoFd\endcsname{$-$0.74}
\expandafter\def\csname nm@rhoFdCI\endcsname{[$-$0.82, $-$0.63]}
\expandafter\def\csname nm@rhoFdPooled\endcsname{$-$0.72}
\expandafter\def\csname nm@rhoFdInKlein\endcsname{$-$0.90}
\expandafter\def\csname nm@rhoFdInKleinCI\endcsname{[$-$0.96, $-$0.82]}
\expandafter\def\csname nm@rhoFdInSd21\endcsname{$-$0.60}
\expandafter\def\csname nm@rhoFdInSd21CI\endcsname{[$-$0.78, $-$0.37]}
\expandafter\def\csname nm@rhoFdInSdxl\endcsname{$-$0.05}
\expandafter\def\csname nm@rhoFdInSdxlCI\endcsname{[$-$0.72, +0.63]}
\expandafter\def\csname nm@rhoFdInZimage\endcsname{$-$0.98}
\expandafter\def\csname nm@rhoFdInZimageCI\endcsname{[$-$1.00, $-$0.89]}
\expandafter\def\csname nm@vsRecallClip\endcsname{$-$0.01 [$-$0.04, +0.01]}
\expandafter\def\csname nm@vsFdClip\endcsname{$-$0.01 [$-$0.08, +0.05]}
\expandafter\def\csname nm@vsCoverage\endcsname{$-$0.57 [$-$0.73, $-$0.41]}
\expandafter\def\csname nm@vsCoverageClip\endcsname{$-$0.24 [$-$0.37, $-$0.13]}
\expandafter\def\csname nm@vsFid\endcsname{$-$0.21 [$-$0.33, $-$0.11]}
\expandafter\def\csname nm@vsIs\endcsname{$-$0.54 [$-$0.69, $-$0.40]}
\expandafter\def\csname nm@vsRecog\endcsname{$-$0.33 [$-$0.47, $-$0.22]}
\expandafter\def\csname nm@vsVendi\endcsname{$-$0.09 [$-$0.16, $-$0.04]}
\expandafter\def\csname nm@vsAesthetic\endcsname{$-$0.41 [$-$0.55, $-$0.29]}
\expandafter\def\csname nm@vsPick\endcsname{$-$0.32 [$-$0.47, $-$0.19]}
\expandafter\def\csname nm@vsLinear\endcsname{$-$0.19 [$-$0.29, $-$0.11]}
\expandafter\def\csname nm@vsContrast\endcsname{$-$0.38 [$-$0.51, $-$0.28]}
\expandafter\def\csname nm@vsFd\endcsname{$-$0.14 [$-$0.23, $-$0.06]}
\expandafter\def\csname nm@rhoRecallLofo\endcsname{+0.85}
\expandafter\def\csname nm@partAesthetic\endcsname{+0.26}
\expandafter\def\csname nm@partAestheticCI\endcsname{[+0.08, +0.39]}
\expandafter\def\csname nm@rawAesthetic\endcsname{$-$0.46}
\expandafter\def\csname nm@partPick\endcsname{+0.11}
\expandafter\def\csname nm@partPickCI\endcsname{[$-$0.10, +0.30]}
\expandafter\def\csname nm@rawPick\endcsname{$-$0.55}
\expandafter\def\csname nm@eSixteenMin\endcsname{61}
\expandafter\def\csname nm@eSixteenMax\endcsname{95}
\expandafter\def\csname nm@eSixteenCount\endcsname{10}
\expandafter\def\csname nm@eSixteenPairs\endcsname{10}
\expandafter\def\csname nm@frozenSDResnet\endcsname{$-$14.2}
\expandafter\def\csname nm@frozenSDDinoThree\endcsname{$-$1.8}
\expandafter\def\csname nm@frozenSDDinoTwo\endcsname{$-$3.7}
\expandafter\def\csname nm@frozenSDXLResnet\endcsname{$-$15.6}
\expandafter\def\csname nm@frozenSDXLDinoThree\endcsname{$-$1.1}
\expandafter\def\csname nm@frozenSDXLDinoTwo\endcsname{$-$1.8}
\expandafter\def\csname nm@frozenKleinResnet\endcsname{$-$6.5}
\expandafter\def\csname nm@frozenKleinDinoThree\endcsname{+1.1}
\expandafter\def\csname nm@frozenKleinDinoTwo\endcsname{$-$0.7}
\expandafter\def\csname nm@relayAdKlein\endcsname{0.32}
\expandafter\def\csname nm@relayDistKlein\endcsname{0.05}
\expandafter\def\csname nm@relayBfKlein\endcsname{0.27}
\expandafter\def\csname nm@relayAdSD\endcsname{0.33}
\expandafter\def\csname nm@relayDistSD\endcsname{0.08}
\expandafter\def\csname nm@relayBfSD\endcsname{0.27}
\expandafter\def\csname nm@pcGainKlein\endcsname{96}
\expandafter\def\csname nm@pcLoseKlein\endcsname{4}
\expandafter\def\csname nm@pcGainSD\endcsname{96}
\expandafter\def\csname nm@pcLoseSD\endcsname{4}
\expandafter\def\csname nm@pcRealTopKlein\endcsname{+0.48 [+0.31, +0.63]}
\expandafter\def\csname nm@pcVendiGivenTopKlein\endcsname{$-$0.17 [$-$0.37, +0.03]}
\expandafter\def\csname nm@pcRecallChangeKlein\endcsname{+0.21 [0.00, +0.40]}
\expandafter\def\csname nm@pcRealTopSD\endcsname{+0.39 [+0.21, +0.55]}
\expandafter\def\csname nm@pcVendiGivenTopSD\endcsname{$-$0.18 [$-$0.37, +0.01]}
\expandafter\def\csname nm@pcRecallChangeSD\endcsname{$-$0.21 [$-$0.39, $-$0.01]}
\expandafter\def\csname nm@pcAgree\endcsname{+0.49 [+0.31, +0.64]}
\makeatother
\expandafter\def\csname oo@real500:v2\endcsname{66.1}
\expandafter\def\csname oo@real500:sketch\endcsname{21.1}
\expandafter\def\csname oo@real500:r\endcsname{30.8}
\expandafter\def\csname oo@real500:a\endcsname{4.3}
\expandafter\def\csname oo@klein:v2\endcsname{15.4}
\expandafter\def\csname oo@klein:sketch\endcsname{5.0}
\expandafter\def\csname oo@klein:r\endcsname{6.8}
\expandafter\def\csname oo@klein:a\endcsname{0.5}
\expandafter\def\csname oo@kb_dd2_g1:v2\endcsname{34.9}
\expandafter\def\csname oo@kb_dd2_g1:sketch\endcsname{16.3}
\expandafter\def\csname oo@kb_dd2_g1:r\endcsname{22.6}
\expandafter\def\csname oo@kb_dd2_g1:a\endcsname{2.8}
\expandafter\def\csname oo@kd_ad2_x3:v2\endcsname{37.4}
\expandafter\def\csname oo@kd_ad2_x3:sketch\endcsname{22.5}
\expandafter\def\csname oo@kd_ad2_x3:r\endcsname{27.9}
\expandafter\def\csname oo@kd_ad2_x3:a\endcsname{3.6}
\expandafter\def\csname oo@kb_g1:v2\endcsname{37.4}
\expandafter\def\csname oo@kb_g1:sketch\endcsname{23.0}
\expandafter\def\csname oo@kb_g1:r\endcsname{30.3}
\expandafter\def\csname oo@kb_g1:a\endcsname{3.7}
\expandafter\def\csname oo@sdt4:v2\endcsname{14.9}
\expandafter\def\csname oo@sdt4:sketch\endcsname{4.9}
\expandafter\def\csname oo@sdt4:r\endcsname{4.6}
\expandafter\def\csname oo@sdt4:a\endcsname{2.2}
\expandafter\def\csname oo@sdt4_dd2_g1:v2\endcsname{28.8}
\expandafter\def\csname oo@sdt4_dd2_g1:sketch\endcsname{11.1}
\expandafter\def\csname oo@sdt4_dd2_g1:r\endcsname{13.7}
\expandafter\def\csname oo@sdt4_dd2_g1:a\endcsname{3.8}
\expandafter\def\csname oo@sdt_ad1_x3:v2\endcsname{36.8}
\expandafter\def\csname oo@sdt_ad1_x3:sketch\endcsname{12.7}
\expandafter\def\csname oo@sdt_ad1_x3:r\endcsname{16.4}
\expandafter\def\csname oo@sdt_ad1_x3:a\endcsname{2.6}
\expandafter\def\csname oo@sd21_g1:v2\endcsname{41.0}
\expandafter\def\csname oo@sd21_g1:sketch\endcsname{18.6}
\expandafter\def\csname oo@sd21_g1:r\endcsname{26.4}
\expandafter\def\csname oo@sd21_g1:a\endcsname{2.8}
\expandafter\def\csname oo@zimage_turbo:v2\endcsname{12.0}
\expandafter\def\csname oo@zimage_turbo:sketch\endcsname{5.7}
\expandafter\def\csname oo@zimage_turbo:r\endcsname{6.0}
\expandafter\def\csname oo@zimage_turbo:a\endcsname{0.9}
\expandafter\def\csname oo@zt_ad2_x3:v2\endcsname{30.0}
\expandafter\def\csname oo@zt_ad2_x3:sketch\endcsname{12.9}
\expandafter\def\csname oo@zt_ad2_x3:r\endcsname{13.2}
\expandafter\def\csname oo@zt_ad2_x3:a\endcsname{2.1}
\expandafter\def\csname oo@real500_e200:v2\endcsname{67.0}
\expandafter\def\csname oo@real500_e200:sketch\endcsname{21.6}
\expandafter\def\csname oo@real500_e200:r\endcsname{31.0}
\expandafter\def\csname oo@real500_e200:a\endcsname{3.8}
\expandafter\def\csname oo@mix_klein:v2\endcsname{67.8}
\expandafter\def\csname oo@mix_klein:sketch\endcsname{23.7}
\expandafter\def\csname oo@mix_klein:r\endcsname{33.3}
\expandafter\def\csname oo@mix_klein:a\endcsname{5.1}
\expandafter\def\csname oo@mix_kd_ad2:v2\endcsname{70.1}
\expandafter\def\csname oo@mix_kd_ad2:sketch\endcsname{31.8}
\expandafter\def\csname oo@mix_kd_ad2:r\endcsname{38.6}
\expandafter\def\csname oo@mix_kd_ad2:a\endcsname{5.1}
\expandafter\def\csname oo@mix_sdt4:v2\endcsname{69.0}
\expandafter\def\csname oo@mix_sdt4:sketch\endcsname{25.9}
\expandafter\def\csname oo@mix_sdt4:r\endcsname{33.9}
\expandafter\def\csname oo@mix_sdt4:a\endcsname{5.1}
\expandafter\def\csname oo@mix_sdt_ad1:v2\endcsname{70.1}
\expandafter\def\csname oo@mix_sdt_ad1:sketch\endcsname{29.0}
\expandafter\def\csname oo@mix_sdt_ad1:r\endcsname{36.9}
\expandafter\def\csname oo@mix_sdt_ad1:a\endcsname{4.9}
\expandafter\def\csname oo@in1k_klein_full:v2\endcsname{7.1}
\expandafter\def\csname oo@in1k_klein_full:sketch\endcsname{2.2}
\expandafter\def\csname oo@in1k_klein_full:r\endcsname{1.8}
\expandafter\def\csname oo@in1k_klein_full:a\endcsname{0.1}
\expandafter\def\csname oo@in1k_kd_ad2_full:v2\endcsname{29.0}
\expandafter\def\csname oo@in1k_kd_ad2_full:sketch\endcsname{13.6}
\expandafter\def\csname oo@in1k_kd_ad2_full:r\endcsname{15.0}
\expandafter\def\csname oo@in1k_kd_ad2_full:a\endcsname{1.3}
\expandafter\def\csname oo@in1k_sdt4_full:v2\endcsname{10.5}
\expandafter\def\csname oo@in1k_sdt4_full:sketch\endcsname{2.9}
\expandafter\def\csname oo@in1k_sdt4_full:r\endcsname{4.2}
\expandafter\def\csname oo@in1k_sdt4_full:a\endcsname{0.5}
\expandafter\def\csname oo@in1k_sdt_ad1_full:v2\endcsname{27.1}
\expandafter\def\csname oo@in1k_sdt_ad1_full:sketch\endcsname{7.4}
\expandafter\def\csname oo@in1k_sdt_ad1_full:r\endcsname{10.1}
\expandafter\def\csname oo@in1k_sdt_ad1_full:a\endcsname{1.2}
\expandafter\def\csname oo@in1k_real_e200:v2\endcsname{65.2}
\expandafter\def\csname oo@in1k_real_e200:sketch\endcsname{24.4}
\expandafter\def\csname oo@in1k_real_e200:r\endcsname{25.4}
\expandafter\def\csname oo@in1k_real_e200:a\endcsname{2.5}
\expandafter\def\csname oo@in1k_mix_klein:v2\endcsname{64.5}
\expandafter\def\csname oo@in1k_mix_klein:sketch\endcsname{24.0}
\expandafter\def\csname oo@in1k_mix_klein:r\endcsname{24.8}
\expandafter\def\csname oo@in1k_mix_klein:a\endcsname{1.7}
\expandafter\def\csname oo@in1k_mix_kd_ad2:v2\endcsname{65.0}
\expandafter\def\csname oo@in1k_mix_kd_ad2:sketch\endcsname{27.7}
\expandafter\def\csname oo@in1k_mix_kd_ad2:r\endcsname{27.9}
\expandafter\def\csname oo@in1k_mix_kd_ad2:a\endcsname{2.6}
\expandafter\def\csname gp@oodVTwoKlein\endcsname{+22.1}
\expandafter\def\csname gpci@oodVTwoKlein\endcsname{[+18.8, +25.4]}
\expandafter\def\csname gpa@oodVTwoKlein\endcsname{22.1}
\expandafter\def\csname gp@oodSketchKlein\endcsname{+17.5}
\expandafter\def\csname gpci@oodSketchKlein\endcsname{[+13.8, +21.4]}
\expandafter\def\csname gpa@oodSketchKlein\endcsname{17.5}
\expandafter\def\csname gp@oodVTwoSD\endcsname{+21.9}
\expandafter\def\csname gpci@oodVTwoSD\endcsname{[+18.4, +25.4]}
\expandafter\def\csname gpa@oodVTwoSD\endcsname{21.9}
\expandafter\def\csname gp@oodSketchSD\endcsname{+7.8}
\expandafter\def\csname gpci@oodSketchSD\endcsname{[+5.3, +10.5]}
\expandafter\def\csname gpa@oodSketchSD\endcsname{7.8}
\expandafter\def\csname gp@oodVTwoZ\endcsname{+18.0}
\expandafter\def\csname gpci@oodVTwoZ\endcsname{[+15.0, +21.1]}
\expandafter\def\csname gpa@oodVTwoZ\endcsname{18.0}
\expandafter\def\csname gp@oodSketchZ\endcsname{+7.3}
\expandafter\def\csname gpci@oodSketchZ\endcsname{[+5.1, +9.6]}
\expandafter\def\csname gpa@oodSketchZ\endcsname{7.3}
\expandafter\def\csname gp@inkOodVTwoKlein\endcsname{+21.9}
\expandafter\def\csname gpci@inkOodVTwoKlein\endcsname{[+20.7, +23.1]}
\expandafter\def\csname gpa@inkOodVTwoKlein\endcsname{21.9}
\expandafter\def\csname gp@inkOodSketchKlein\endcsname{+11.5}
\expandafter\def\csname gpci@inkOodSketchKlein\endcsname{[+10.6, +12.4]}
\expandafter\def\csname gpa@inkOodSketchKlein\endcsname{11.5}
\expandafter\def\csname gp@inkOodRKlein\endcsname{+12.8}
\expandafter\def\csname gpci@inkOodRKlein\endcsname{[+11.4, +14.1]}
\expandafter\def\csname gpa@inkOodRKlein\endcsname{12.8}
\expandafter\def\csname gp@inkOodAKlein\endcsname{+1.3}
\expandafter\def\csname gpci@inkOodAKlein\endcsname{[+0.9, +1.8]}
\expandafter\def\csname gpa@inkOodAKlein\endcsname{1.3}
\expandafter\def\csname gp@inkOodVTwoSD\endcsname{+16.6}
\expandafter\def\csname gpci@inkOodVTwoSD\endcsname{[+15.5, +17.7]}
\expandafter\def\csname gpa@inkOodVTwoSD\endcsname{16.6}
\expandafter\def\csname gp@inkOodSketchSD\endcsname{+4.6}
\expandafter\def\csname gpci@inkOodSketchSD\endcsname{[+4.0, +5.1]}
\expandafter\def\csname gpa@inkOodSketchSD\endcsname{4.6}
\expandafter\def\csname gp@inkOodRSD\endcsname{+5.8}
\expandafter\def\csname gpci@inkOodRSD\endcsname{[+4.9, +6.8]}
\expandafter\def\csname gpa@inkOodRSD\endcsname{5.8}
\expandafter\def\csname gp@inkOodASD\endcsname{+0.8}
\expandafter\def\csname gpci@inkOodASD\endcsname{[+0.3, +1.3]}
\expandafter\def\csname gpa@inkOodASD\endcsname{0.8}
\expandafter\def\csname gp@mixOodSketchKleinOverReal\endcsname{+10.2}
\expandafter\def\csname gpci@mixOodSketchKleinOverReal\endcsname{[+7.9, +12.6]}
\expandafter\def\csname gpa@mixOodSketchKleinOverReal\endcsname{10.2}
\expandafter\def\csname gp@mixOodSketchSDOverReal\endcsname{+7.4}
\expandafter\def\csname gpci@mixOodSketchSDOverReal\endcsname{[+5.5, +9.3]}
\expandafter\def\csname gpa@mixOodSketchSDOverReal\endcsname{7.4}
\expandafter\def\csname gp@mixOodSketchDistKleinOverReal\endcsname{+2.1}
\expandafter\def\csname gpci@mixOodSketchDistKleinOverReal\endcsname{[+0.9, +3.3]}
\expandafter\def\csname gpa@mixOodSketchDistKleinOverReal\endcsname{2.1}
\expandafter\def\csname gp@mixOodSketchDistSDOverReal\endcsname{+4.3}
\expandafter\def\csname gpci@mixOodSketchDistSDOverReal\endcsname{[+2.6, +5.9]}
\expandafter\def\csname gpa@mixOodSketchDistSDOverReal\endcsname{4.3}
\expandafter\def\csname gp@inkMixOodSketchAdOverReal\endcsname{+3.3}
\expandafter\def\csname gpci@inkMixOodSketchAdOverReal\endcsname{[+2.9, +3.7]}
\expandafter\def\csname gpa@inkMixOodSketchAdOverReal\endcsname{3.3}
\expandafter\def\csname gp@inkMixOodRAdOverReal\endcsname{+2.5}
\expandafter\def\csname gpci@inkMixOodRAdOverReal\endcsname{[+2.0, +3.0]}
\expandafter\def\csname gpa@inkMixOodRAdOverReal\endcsname{2.5}
\expandafter\def\csname gp@inkMixOodSketchDistOverReal\endcsname{$-$0.4}
\expandafter\def\csname gpci@inkMixOodSketchDistOverReal\endcsname{[$-$0.7, $-$0.1]}
\expandafter\def\csname gpa@inkMixOodSketchDistOverReal\endcsname{0.4}
\expandafter\def\csname gp@inkMixOodRDistOverReal\endcsname{$-$0.5}
\expandafter\def\csname gpci@inkMixOodRDistOverReal\endcsname{[$-$0.9, $-$0.2]}
\expandafter\def\csname gpa@inkMixOodRDistOverReal\endcsname{0.5}
\expandafter\def\csname nm@qAestLower\endcsname{all three}
\expandafter\def\csname nm@qPickLower\endcsname{two}
\expandafter\def\csname nm@qRecogLower\endcsname{all three}
\expandafter\def\csname nm@qFidBetter\endcsname{all three}
\expandafter\def\csname nm@lrnShareRAKlein\endcsname{92}
\expandafter\def\csname nm@lrnShareRASD\endcsname{98}
\expandafter\def\csname nm@lrnShareWPKlein\endcsname{78}
\expandafter\def\csname nm@lrnShareWPSD\endcsname{68}
\expandafter\def\csname nm@lrnShareCNXKlein\endcsname{71}
\expandafter\def\csname nm@lrnShareCNXSD\endcsname{85}
\expandafter\def\csname nm@lrnShareMin\endcsname{68}
\expandafter\def\csname nm@lrnShareMax\endcsname{98}
\expandafter\def\csname nm@trGainMin\endcsname{10.7}
\expandafter\def\csname nm@trGainMax\endcsname{28.5}

